Sum-of-Squares meets Nash: Optimal Lower Bounds for Finding any Equilibrium

Several works have shown unconditional hardness (via integrality gaps) of computing equilibria using strong hierarchies of convex relaxations. Such results however only apply to the problem of computing equilibria that optimize a certain objective function and not to the (arguably more fundamental) task of finding \emph{any} equilibrium. We present an algorithmic model based on the sum-of-squares (SoS) hierarchy that allows escaping this inherent limitation of integrality gaps. In this model, algorithms access the input game only through a relaxed solution to the natural SoS relaxation for computing equilibria. They can then adaptively construct a list of candidate solutions and invoke a verification oracle to check if any candidate on the list is a solution. This model captures most well-studied approximation algorithms such as those for Max-Cut, Sparsest Cut, and Unique-Games. The state-of-the-art algorithms for computing exact and approximate equilibria in two-player, n-strategy games are captured in this model and require that at least one of i) size (~ running time) of the SoS relaxation or ii) the size of the list of candidates, be at least $2^{\Omega(n)}$ and $n^{\Omega(\log{(n)})}$ respectively. Our main result shows a lower bound that matches these upper bound up to constant factors in the exponent. This can be interpreted as an unconditional confirmation, in our restricted algorithmic framework, of Rubinstein's recent conditional hardness \cite{Rub} for computing approximate equilibria. Our proof strategy involves constructing a family of games that all share a common sum-of-squares solution but every (approximate) equilibrium of one game is far from every (approximate) equilibrium of any other game in the family.

==> content/Old/Gilbow-Zemel.tex <==
%!TEX root=../main.tex
\section{Gilbow-Zemel Construction: Clique to Game}
Given an undirected graph $G$ on $n$ vertices represented by an adjacency matrix $E$ (abuse of notation), we wish to check if it has a clique of size $k\le n$. We will reduce this problem to checking if a two player game has more than one equilibrium. 

For $\delta \in (0, 1)$, $M>1$ , and $A=E + (1+\delta) I_{n\times n}$, $B=-M* I_{n\times n}$ and $B'=k*I_{n\times n}$, consider the following $2n+1 \times 2n+1$ block matrices:
\[
R=\left[\begin{array}{cc}
\begin{array}{cc}
A & B\\
B' & \zeros_{n\times n}\\
\end{array}
& -M \ones_{2n \times 1}\\
(1+\frac{\delta}{k}) \ones_{1\times 2n} & 1+\frac{\delta}{k}
\end{array}\right]
\ \ \ \ \ \ 
C=\left[\begin{array}{cc}
\begin{array}{cc}
A & B'\\
B & \zeros_{n\times n}\\
\end{array}
& (1+\frac{\delta}{k}) \ones_{2n\times 1}\\
-M \ones_{2n\times 1}& 1+\frac{\delta}{k}
\end{array}\right]
\]


Note that game $(R,C)$ is symmetric, i.e., $C=R^T$. For ease of notation let $m=2n+1$. For any given mixed strategy $\xx \in \Delta_{m}$, we will denote its support by $S(\xx)=\{i \ |\ x_i>0\}$. 


\begin{lemma}\label{lem:gz1}
$(\xx,\yy)$ is a NE of game $(R,C)$ where $S(\xx),S(\yy) \subseteq \{1,\dots,n\}$ iff graph $G$ has a clique of size $k$. 
\end{lemma}
\begin{proof}
From clique to NE is easy to see. Let $K\subset \{1,\dots,n\}$ be the vertices on the $k$-clique. Then setting $x_u=y_u=1/k,\ \forall u \in K$, and $x_u=y_u=0$ otherwise is a Nash equilibrium. This is because payoff from each non-zero strategy is $(1+\delta/k)$, and from strategies with zero probability it is at most $(1+\delta/k)$. 

To map NE supported on first $n$ strategies to clique in graph $G$, first observe that no matter what the column player is playing, row player gets $(1+\delta/k)$ from the last strategy $m$, and vice-versa. Therefore, all the non-zero strategies of both the players has to give at least $(1+\delta/k)$ payoff. This is possible for the row player only if $S(\yy)$ forms a clique, and for each $j \in S(\yy),\ y_j\ge \frac{1}{k}$. This implies $|S(\yy)|\le k$.

Now it suffices to argue that $|S(\yy)|=k$. To the contrary suppose $|S(\yy)|<k$. Let $j^* = \argmax_{j \le m} y_j$, then clearly $y_{j^*} \ge \frac{1}{k-1}$. 
Row player's payoff from any $i\in \{1,\dots, n\}$ is at most $1+\delta y_{j^*}<1+y_{j^*}$, where the inequality is due to $\delta<1$. While from strategy $n+j$ it is $k * y_{j^*} = (k-1) y_{j^*} + y_{j^*} \ge 1+y_{j^*}$, where the last inequality is due to $y_{j^*}\ge \frac{1}{(k-1)}$. A contradiction to $S(\xx)\subseteq \{1,\dots,n\}$. 

Since the game is symmetric, we can similarly argue that vertices corresponding strategies in $S(\xx)$ forms a $k$-clique in graph $G$. 
\end{proof}

\begin{lemma}\label{lem:gz2}
If $(\xx,\yy)$ is a Nash equilibrium of game $(R,C)$ then either $S(\xx),S(\yy) \in \{1,\dots,n\}$ or $S(\xx)=S(\yy) = 2n+1$. 
\end{lemma}
\begin{proof}
To the contrary suppose neither holds $S(\yy)$. If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$ then $S(\xx)=\{m\}$, and vice-versa. This is because any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of $(1+\delta/k)$. Therefore, we have that $y_L =  \sum_{i=1}^n y_i \in (0, 1)$. The proof is based on a number of observations which I will list next with a brief justification.
\begin{enumerate}
%\item If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$ then $S(\xx)=\{m\}$, and vice-versa: This is because any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of $(1+\delta/k)$. 
%\item If $\exists i \in S(\yy) \cap \{1,\dots,n\}$ such that $y_i \ge \frac{1}{k-1}$, then $S(\xx)\cap \{1,\dots,n\} = \emptyset$, and vice-versa: Let $i^* = \argmax_{i \le n} y_i$, then payoff of player one from strategy $n+i^*$ is $ky_{i^*}-My_m=(k-1)y_{i^*} + y_{i^*} -My_m\ge 1+y_{i^*}-My_m$. While for any $i\le n$, her payoff is at most $1+\delta y_i - M y_{n+i} - M y_m<1+y_{i^*}-My_m$. The claim follows.
\item $\forall i \in S(\xx)$, $(Ry)_i \ge 1+\delta/k$, and similarly for player two: This follows from the fact that the last strategy always gives $(1+\delta/k)$ payoff regardless of what the other player is playing. 
\item $\forall i\le n, x_i > 0 \Rightarrow y_i \ge \frac{1}{k}$, and $y_i>0 \Rightarrow x_i \ge \frac{1}{k}$: This follows from the fact that player one gets at most $(1+\delta y_i)$ payoff from strategy $i\le n$. Therefore using point (1), $x_i > 0 \Rightarrow (1+\delta y_i) \ge 1+\delta/k$, and the claim follows.  
%\item $\forall i\le n, x_{n+i}>0 \Rightarrow y_i \ge \frac{1}{k} + \frac{\delta}{k^2}$, and $y_{n+i}>0 \Rightarrow x_i \ge \frac{1}{k} + \frac{\delta}{k^2}$: Proof follows from the fact that payoff of the two players from strategy $(n+i)$ is $k*y_i$ or $k*x_i$ respectively. They need to be at least $(1+\delta/k)$ due to point (2).
%\item From point (4) it follows that $|S(\xx) \cap \{n+1,\dots,2n\}|\le (k-1)$ and $|S(\yy) \cap \{n+1,\dots,2n\} \le (k-1)$.
\item $y_L <1$ together with point (2) implies $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$. Point (2) also implies $S(\yy) \cap \{1,\dots,n\} =S(\xx) \cap \{1,\dots,n\}\Rightarrow |S(\yy) \cap \{1,\dots,n\}|\le (k-1)$. 
\end{enumerate}
From point (3) we know that $\exists i,i' \in S(\yy) \cap \{1,\dots,n\}$ such that $y_i \le y_L/a$ and $y_{i'}\ge y_L/a$, where $a=|S(\yy) \cap \{1,\dots,n\}|\ge 1$ (because, $y_L>0$). And then point (3) implies $x_i>0$ as well. The payoff$_1(i) \le y_L + \delta y_i - M y_{n+i} - M y_m \le y_L + \delta y_i\le (1+\delta/a)y_L$, while the payoff$_1(n+i') = k y_{i'} \ge ky_L/a$. From (3) we have $a \le (k-1)$ and therfore 
\[
\mbox{payoff}_1(n+i') - \mbox{payoff}_1(i) \ge (k/a - 1 - \delta/a) y_L = (k - a - \delta)y_L/a \ge (1-\delta)y_L/a \ge (a/k) (1/2a) = 1/(2k)
\]
Last inequality follows taking $\delta\le 1/2$ and since we have $y_L \ge a/k$ using (3). %y_i \ge \frac{1}{k}$
This contradicts strategy $i$ being best response of player one against $\yy$. 
\end{proof}



\begin{comment}
\item If $S(\xx) \cap \{1,\dots, n\}\neq \emptyset$ then $\exists i \le n$ such that $x_i>0$ and payoff$_1(i) < (1+1/(k-1)) y_L$: For each $i\le n$ payoff$_1(i) \le y_L + \delta y_i - M y_{n+i}-M y_m$. Summing these up for non-zero $x_i$'s, using points (3) and (4), we get $\sum_{i\le n: x_i>0} \mbox{ payoff}_1(i) < (k-1) y_L + \delta y_L $. Since there are at most $(k-1)$ non-zero startagies among first $n$ strategies (point (4)), one of them has to give payoff at most $(k-1)$ of this value i.e., $\exists i\le n$ such that $x_i>0$ and payoff$_1(i)< (1+\delta/(k-1)) y_L < (1+1/(k-1)) y_L$ 
\item $\exists i \le n$ such that payoff$_1(n+i)\ge (1+1/(k-1)) y_L$: From point (4) it follows that if $i^* = \argmax_{i\le n} y_i$ then $y_{i^*} \ge y_L/(k-1)$. Therefore, payoff$_1(n+i^*) = ky_{i^*} \ge (1+1/(k-1)) y_L$. 
%\item $y_R = \sum_{i=n+1}^{2n} y_i \le \frac{2\delta}{M}$ and $x_R = \sum_{i=n+1}^{2n} y_i \le \frac{2\delta}{M}$
\end{enumerate}
If there is a strategy $i\le n$ that is a best response of the first player, i.e., $i \in S(\xx)$, then points (5) and (6) implies that there will be one played with non-zero probability that gives lower than highest payoff, which can not be the case at a Nash equilibrium. Therefore, essentially last two points imply that $S(\xx) \cap \{1,\dots,n\} =\emptyset$. This with point (1) implies that $S(\yy)=2n+1$, a contradiction to the initial assumption. 
\end{proof}
\end{comment}
\medskip

\noindent{\bf Approximation.} Note that in Lemma \ref{lem:gz1} when $|S(\yy)|<k$ then the difference in first player's payoff from its $j^*$th strategy and $(n+j^*)$th strategy is at least $(1-\delta)/(k-1)$. Now on we will set $\delta=1/2$, this gives $1/2(k-1)$ gap. Therefore, for $epsilon = \frac{1}{3k}$ and slightly modified game where last row of matrix $R$ and last column of matrix $C$ to $1+\frac{\delta}{k} + \frac{2\delta}{3k}$, Lemma \ref{lem:gz1} will follow even for $\epsilon$-approximate well-supported equilibrium. However, Lemma \ref{lem:gz2} is a bit tricky that we show next.


\begin{lemma}\label{lem:approx-gz2}
Given that graph $G$ does not have a clique of size $k$, if $(\xx,\yy)$ is a $\frac{1}{3k}$-approximate well-supported Nash equilibrium of game $(R,C)$ then either $S(\xx)=S(\yy)=\{2n+1\}$. % \in \{1,\dots,n\}$ or $S(\xx)=S(\yy) = 2n+1$. 
\end{lemma}
\begin{proof}
To the contrary suppose $S(\yy)\neq \{2n+1\}$. Recall that $m=2n+1$. %neither holds for $S(\yy)\Rightarrow y_L =  \sum_{i=1}^n y_i <1$. 
This proof is based on a number of observations which we list next with a brief justification.
\begin{enumerate}
\item $S(\yy) \cap \{1,\dots,n\} \neq \emptyset$ and $S(\xx) \cap \{1,\dots,n\} \neq \emptyset$: If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$, then $S(\xx)=\{2n+1\}$ since any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of at least $1$. In that case, by the same argument $S(\yy)=\{2n+1\}$, a contradiction. Second part follows similarly. 

\item $\forall i \in S(\xx)$, $(Ry)_i \ge 1+\delta/k$, and similarly for player two: This follows from the fact that the last strategy always gives $(R\yy)_m = (1+\delta/k + \delta/2k^3)$ payoff regardless of what the other player is playing, and that $(R\yy)_m -\epsilon = 1+\delta/k$. 

\item $\forall i\le n, x_i > 0 \Rightarrow y_i \ge \frac{1}{k}$, and $y_i>0 \Rightarrow x_i \ge \frac{1}{k}$: This follows from the fact that player one gets at most $(1+\delta y_i)$ payoff from strategy $i\le n$. Therefore using point (2), $x_i > 0 \Rightarrow (1+\delta y_i) \ge 1+\delta/k$, and the claim follows.  

%\item $\forall i \in S(\yy) \cap \{1,\dots,n\}$, $y_i < \frac{1}{k-1}$, and similary for $\xx$: Let $i^* = \argmax_{i \le n} y_i$, then payoff of player one from strategy $n+i^*$ is $ky_{i^*}-My_m=(k-1)y_{i^*} + y_{i^*} -My_m\ge 1+y_{i^*}-My_m$. While for any $i\le n$, her payoff is at most $1+\delta y_i - M y_{n+i} - M y_m<1+\frac{y_{i^*}}{2}-My_m$. Thus payoff from strategy $n+i^*$ is at least $y_{i^*}/2$ higher than any of the strategies $i \le n$. From (3) we get a lower bound of $\frac{1}{k}$ on $y_{i^*}$, which would imply $S(\xx) \cap \{1,\dots,n\}=\emptyset$ contradicting (1). 

%\item $\forall i\le n, x_{n+i}>0 \Rightarrow y_i \ge \frac{1}{k} + \frac{\delta}{k^2}$, and $y_{n+i}>0 \Rightarrow x_i \ge \frac{1}{k} + \frac{\delta}{k^2}$: Proof follows from the fact that payoff of the two players from strategy $(n+i)$ is $k*y_i$ or $k*x_i$ respectively. They need to be at least $(1+\delta/k)$ due to point (2).
%\item From point (4) it follows that $|S(\xx) \cap \{n+1,\dots,2n\}|\le (k-1)$ and $|S(\yy) \cap \{n+1,\dots,2n\} \le (k-1)$.

\item $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$ and $|S(\yy) \cap \{1,\dots,n\}| \le (k-1)$: Since $G$ does not have a $k$-clique, from Lemma \ref{lem:gz1} we know that either $y_L=\sum_{i\le n} y_i<1$ or $x_L=\sum_{i\le n} x_i<1$. Suppose the first holds, then (3) implies $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$. Point (3) also implies $S(\yy) \cap \{1,\dots,n\} =S(\xx) \cap \{1,\dots,n\}$ giving us $|S(\yy) \cap \{1,\dots,n\}|\le (k-1)$ as well.
\end{enumerate}

The lemma follows by the same argument as in the proof of Lemma \ref{lem:gz2} since there exist $i \in S(\xx) \cap \{1,\dots,n\}$ such that payoff$_1(i)$ is at least $1/2k$ less than payoff$_1(n+i')$ for some $i'\le n$. This contradicts $\xx$ being $\frac{1}{3k}$-approximate well supported equilibrium.
\end{proof}


%Let $S= S(\yy) \cap \{1,\dots,n\}$ ($=S(\xx) \cap \{1,\dots,n\}$ due to (3)). 
%Since $G$ does not have a clique of size $k-1$, there is some $i \in S$ that has $R(i,j)=0$ for some $j \in S$. Therefore, payoff$_1(i) = (R\yy)_i \le y_L - y_j + \delta y_i$. From (3) we know that $y_j \ge \frac{1}{k}$ and from (4) we have $y_i \le \frac{1}{k-1}$. Applying these to payoff expression we get payoff$_1(i) \le y_L - \frac{1}{k} + \frac{1}{2(k-1)}$. From (2) this value has to be at least $1+1/2k$, which would require $k \le 1/2$, a contradiction. 
%\end{proof}

To allow assumption that $k$-clique does not exist in graph $G$ in the above lemma, 
%To allow graphs with $(k-1)$ sized clique, but no $k$ sized clique, 
we can make the above proof work by setting last row of $R$ and last column of $C$ to $1+\delta/(k-1)+\delta/2k^3$. This would also simplify the proof because essentially we will get lower bound of $1/(k-1)$ in point (3), and then point (4) will contradict it. 


For game constructed from graphs with $k$-clique, we want to ensure that no $\epsilon$-approximate equilibrium gives non-zero probability to the last startegy. We can do this by changing last row and last column of $R$ and $C$ respectively to $-1$. 


==> content/Old/abstract.tex <==
%!TEX root = ../main.tex
We attempt to design subexponential time algorithms for computing Nash Equilibria in two player games.

==> content/Old/notes.tex <==
%!TEX root=../main.tex
\section{Preliminaries and Notation}
We denote the simplex in $n$ dimensions by $\Delta_n = \{x \in \R^n \mid x_i \geq 0 \text{ for every } i \text{ and } \sum_{i = 1}^n x_i = 1\}.$
\section{Correlated Equilibrium Formulation}
We state the problem of computing correlated equilibria in general two player games.
The input is a pair of payoff matrices $A, B \in \R^{n \times n}$ (for players Alice and Bob respectively) where to avoid notational clutter, we assume that the two players have the same number of pure strategies. $A$ and $B$ are assumed to normalized so that every entry of the two matrices is in $[0,1].$

\begin{definition}[Correlated Equilibrium]
A correlated equilibrium in a two player games with payoff matrices $A$ and $B$ is a distribution $p$ on ordered pairs of strategies $(i,j)$ for $1 \leq i , j \leq n$ such that the following complementary slackness conditions hold:
\begin{enumerate}
\item For every $i \in [n]$, $\sum_{j} A_{i,j} p_{i,j} \geq \sum_{j} A_{i',j} p_{i,j}$ for every $i' \in [n].$
\item For every $j \in [n]$, $\sum_{i} B_{i,j} p_{i,j} \geq \sum_{i} B_{i,j'} p_{i,j}$ for every $j' \in [n].$
\end{enumerate}
\end{definition} 

A correlated equilibrium is a Nash equilibrium in the usual sense, if $p = ab^{\top}$ for probability distributions $a,b\in \Delta_n.$ 

Correlated equilibria have a nice interpretation as follows: Imagine that there's a neutral third-party overseer that advises the two players on their strategies! Then, the overseer can force equilibrium by choosing a pair of strategies $(i,j)$ according to $p_{i,j}$ and sending advice $i$ to Alice and $j$ to Bob. The complementary slackness conditions above then say that no party has a (strict) incentive to deviate from the advised strategy.

The usefulness of the concept of correlated equilibrium is due to the fact that it can be efficiently computed using linear programming as is evident from the definition itself. 

The central question we now have is the following, stated in the language of correlated equilibrium.

\begin{question}
Suppose there's a set of possible advice that the overseer can give (say $[N]$, typically exponentially large in $n$)). Suppose there's a map from $[N]$ into a Nash equilibrium $a_ib_i^{\top}$. Suppose further, that following kind of distribution $\cD$  describes a correlated equilibrium for the bi-matrix game $(A,B)$: Choose $i \sim \cD$, output $a_i$ and $b_i$ as the probability distributions over  pure strategies for Alice and Bob respectively. 

For every distribution $\cD$ on $[N]$ as above, is there an event $E$ with probability $\ll 2^{-n}$ such that conditioning $\cD$ on $E$ yields a distribution $\cD'$ such that $\E_{i \sim \cD'} a_i b_i^{\top} \approx ab^{\top}$ for $a,b \in \Delta_n$ and the notion of approximation relevant to satisfying both of types of the complementary slackness conditions in the definnition above? 

\end{question}


==> content/Old/old-stuff.tex <==
%!TEX root=../main.tex
\section{Nash Equilibrium (NE) Formulations}
Given a two player game, where both the players have $n$ actions to choose from, it can be represented by two $n\times n$ matrices $(A,B)$. Following is a NE characterization of such games:

Strategy profile $(x,y)$ where $x,y\in \Delta_n$ is a NE of $(A,B)$ iff


If the game is symmetric then, $B=A^T$. And a symmetric profile $(x,x)$ is a NE iff
\begin{equation}\label{eq:SNEchar}
\begin{array}{llcl}
\forall i\le n, & x_i >0 &\Rightarrow &(Ax)_i = \max_k (Ax)_k\\
\end{array}
\end{equation}

From (\ref{eq:NEchar}) we can derive following quadratic formulation that captures NE exactly, where $\pi_1$ and $\pi_2$ capture the maximum payoff of players one and two respectively.

\begin{equation}\label{eq:NEQP}
\begin{array}{rl}
\max: & x^T(A+B)y - \pi_1 - \pi_2 \\
s.t. & (Ay)_i \le \pi_1,\ \ \ \forall i\le n \\
& (x^TB)_j \le \pi_2,\ \ \ \forall j \le n \\
& \sum_i x_i =1,\ \ \ \sum_j y_j =1 \\
& x\ge 0,\ \ \ y\ge 0
\end{array}
\end{equation}

Similarly, for symmetric NE we can write the following formulation:
\begin{equation}\label{eq:SNEQP}
\begin{array}{rl}
\max: & x^TAy - \pi\\
s.t. & (Ax)_i \le \pi,\ \ \ \forall i\le n \\
& \sum_i x_i =1;\ \ \ \ \ x\ge 0;
\end{array}
\end{equation}

A joint distribution $P=[P_{ij]}]_{i,j\le n}$ is a correlated equilibrium iff
\begin{equation}\label{eq:CE}
\forall i\le n,\ \ \  \ \sum_j A_{ij} P_{ij} \ge \sum_j A_{i'j} P_{ij} \\
\forall i\le n,\ \ \ \ \ \sum_j B_{ij} P_{ij} \ge \sum_j B_{ij'} P_{ij} \\
\end{equation}

It is well known that correlated equilibrium matrices $P$ with rank-1 are exactly the NE.
\medskip

\subsection{Polymatrix Game} This is an $k$ player game with an underlying interaction graph $G=(V,E)$ representing which player plays with who all in a two-player game like interaction. Here $V$ is the set of $k$ players, and if $(u,v)\in V$ then players $u$ and $v$ are playing game $(A_{uv}, A_{vu})$ with each other. For now let us assume that each player has $2$ strategies, then $A_{uv}$ and $A_{vu}$ for all $(u,v)\in E$ are $2 \times 2$ matrices. 

Let $A$ be a block matrix with $2k \times 2k$ dimension, where $(u,v)^{th}$ block has matrix $A_{uv}$ and $(v,u)^{th}$ block is matrix $A_{vu}^T$. NE in this game can be captured via the following quadratic formulation:
\begin{equation}\label{eq:PMQP}
\begin{array}{ll}
\max:& x^TAx - \sum_{u \in V} \pi_u \\
s.t. & \forall u\le n, (Ax)_{2u-1} \le \pi_u;\ \ \ (Ax)_{2u} \le \pi_u \\
& \forall u\le n,\ \ \ \ x_{2u-1} + x_{2u}=1 \\
& x\ge 0
\end{array}
\end{equation}


A slightly different formulation:

\begin{equation}\label{eq:PMQP-feasibility}
\begin{array}{ll}
%\max:& x^TAx - \sum_{u \in V} \pi_u \\
& \forall u\le n, (Ax)_{2u-1} \le \pi_u;\ \ \ (Ax)_{2u} \le \pi_u \\
& \forall u\le n,\ \ \ \ x_{2u-1} + x_{2u}=1 \\
& \forall u \le n, \ \ \  (Ax)_{2u-1} x_{2u-1} +(Ax)_{2u} x_{2u}  = \pi_u\\
& x\ge 0
\end{array}
\end{equation}

\noindent{\bf Net-Coordination Game.}
If every edge is a coordination game, {\em i.e.,} $A_{uv}=A_{vu}$ then it is called net-coordination game. Such a game always has a pure equilibrium, and finding one is PLS-complete. The hardness result is by reduction from {\em local max-cut}, where the problem is to find a cut in the graph which can not be improved by moving exactly one vertex from one partition to another. 

The reduction is as follows: Let $G=(V,E)$ be the input graph of local max-cut problem with weight $w_{uv}$ on edge $(u,v)\in E$. Every vertex is a player, each with two strategies $0$ and $1$. Think of the two strategies as two partitions. Then, every edge $(u,v) \in E$ is a game where ($u$ as first player and $v$ as second player) matrices are $A_{uv}=A_{vu} = \left[\begin{array}{cc} 0 & w_{uv}\\ w_{uv} & 0 \end{array}\right]$.

Let us assume that $w_{uv}\in[0,\ 1]$. Since this is a potential game, where sum of the utilities of all the agents is the potential function, finding $\epsilon$-approximate equilibrium can be done in $O(n^2/\epsilon)$ time just by best-response dynamics. This is because potential is bounded above by $n^2$, and in every step it increases by at least $\epsilon$ when we are not an approximate equilibrium. 



\subsection{Approximation}
Given a two player game, let us assume (wlog) that $(A,B)\in [0,\ 1]$. Profile $(x,y)$ is an $\epsilon$-approximate NE iff
\[
x^Ay \ge x'^TAy - \epsilon,\ \forall x'\in \Delta_n;\ \ \ \ x^TBy \ge x^TBy' - \epsilon,\ \ \forall y'\in \Delta_n
\]

An $\epsilon$-approximate {\em well-supported} NE for given $\epsilon>0$ is $(x,y)$, s.t.
\begin{equation}
\label{eq:ANEchar}
\begin{array}{llcl}
\forall i\le n, & x_i >0 &\Rightarrow &(Ay)_i \ge \max_k (Ay)_k - \epsilon\\
\forall j\le n, & y_i >0 &\Rightarrow &(x^TB)_j = \max_k (x^TB)_k - \epsilon\\
\end{array}
\end{equation}

Similarly, we can define approximate symmetric NE in symmetric game, and approximate NE in polymatrix game. 


\begin{theorem}[ChenDengTeng'06]
End of Line PPAD problem with size $n$ can be reduced to finding $O(\frac{1}{m^4})$-approximate NE in two-player $O(m) \times O(m)$ game, where $m=O(n^4)$. 
\end{theorem}

\begin{theorem}[NeedToShow]
End of Line PPAD problem with size $n$ can be reduced to finding $O(\frac{1}{m})$-approximate NE in a two-player $m \times m$ game, where $m=O(n^4)$ (we may be able to bring this down to O(n)).  
\end{theorem}

\Pnote{I see. So at this point, we need a $2^{o(n^{1/4})}$ time algorithm for $1/n$-approximate Nash equilibrium computation in order t refute ETH for PPAD.}

\Rnote{Looks like that. $1/m$-approximate NE in $2^{o(m^{1/4})}$ would give $2^{o(n)}$ for $m=O(n^4)$. I really hope to bring $m$ down to $O(n)$.}

\section{An SDP Lower Bound?}
Is there an instance of a poly-matrix game with players denoted by $u \in [2n]$ and a SDP solution such that for every $q$ players $Q \subseteq [2n]$, $|Q| = q$, the marginal distribution over $\{ x_u \in \Delta_2 | u \in Q\}$ is pairwise uniform? 

We want to construct a pay-off matrix $A$ over a $3$-regular graph $G$ such that there's an SDP solution to 3.7 the marginal distribution on any $q$ of the player's strategies is pairwise uniform. 

\section{SDPs and stuff}
Max-Cut Problem
\begin{align*}
\max & \langle L, xx^{\top} \rangle \\
\text{s.t. } x_i^2 & = 1 \text{ for every i }\\
\end{align*}

Here's the standard way to write SDP relaxation. 
\begin{align*}
\max & \langle L, X \rangle\\
\text{s.t.} X & \succeq 0 \\
X_{i,i} &= 1 \text{ for every i}.
\end{align*}

One standard way to obtain an $n \times n$ PSD matrix  $X$ is to think of $n$ vectors in whatever dimensions and $X_{i,j} = \langle v_i, v_j \rangle.$ This is PSD is easy. And only slightly harder is the claim that every psd matrix can be written as a gram matrix of some vectors. 

This kind of thinking is fine for the basic SDP that we wrote above. 

We could think of adding more constraints to the SDP above in order to strengthen it - this sum-of-squares is a way of adding more constraints. 

Sum of squares SDP has constraints for any group of small number of variables. Let me write down $SoS_d$ relaxation for max cut. The above SDP can be thought of as $SoS_1$ relaxation. 

Let me write this down next. 

First, $ \langle L, xx^{\top} \rangle$ equals the size of the cut denoted by $x$. This is same as $\sum_{i,j \in [n]} x_i x_j L_{i,j}.$ In the intended solution, $X_{\{i\}, \{j\}} = x_i x_j$.   

It is less awkward to write a constraint in tensor notation. Let $X$ be an object that lives in $\R^{n^{2d}}$ seen as a $2d$-tuples on $[n]$. This will be the object we want to optimize over. 

The indices of this object can be thought of as ordered $\leq 2d$-tuples of elements from $[n]$. Of course, as usual, the intended solution is $X_S = \Pi_{i \in S} x_i$ for every $S \subseteq [n]$, $|S| \leq 2d.$

Before, we relaxed rank 1 matrix constraint to PSD constraint and trace constraint. In notation, we wrote the constraint $X = \sum_{i} \lambda_i u_iu_i^{\top}$ where the $\lambda_i$s are non-negative and sum up to $n$ and $u_i$s are unit vectors, as a relaxation of $X = xx^{\top}$ for $x$ being a vector of norm $\sqrt{n}$ (since it's a plus-minus 1 vector)

This time, we could observe that $X$ is intended to be a rank $1$ tensor of $2d$ dimensions. The natural generalization of PSDness with bounded trace that we can think of would be 
\begin{equation} \label{tensor-psd}
X = \sum_{i} \lambda_i u_i^{\otimes 2d}
\end{equation}
where $\lambda_i$s sum up to $n$ and $u_i$s are unit vectors. Clearly, this would be a valid relaxation. However, unfortunately, we cannot optimize over such "PSD-tensors" unlike PSD matrices. So this relaxation is too strong.

Instead, we arrange the intended solution as a $n^d$ by $n^d$ matrix. Any matrix obtained from a rank $1$ tensor would be rank $1$ (rank 1 as a tensor is a much stronger condition than rank 1 as a matrix). We then relax this rank 1 constraint to PSDness with bounded trace.

All is not lost though - we can capture more properties of rank 1 tensors by forcing the symmetry constraints that are properties of rank 1 tensors (and not arbitrary rank 1 $n^d \times n^d$ matrices).

Okay - so doing this more concretely now.

Let $M(X)$ be the $\approx n^d \times n^d$ matrix representation of $X$. That is, $M_{S,T}$ for any $S, T \subseteq [n]$, $|S|, |T| \leq d$, $M_{S,T} = X_{S} X_{T}.$ 

The intended solution $X$ is supposed to be a rank 1 tensor.
Observe that for the intended actual solution, $M(X)$ is PSD

\begin{align*}
\max & \sum_{i,j} X_{i,j} \cdot L_{i,j}\\
M(X) &\succeq 0\\
\text{ For every $\leq d-2$ tuple $S$} &\text{for every $i$ } X_{S} = X_{(S, i,i)}\\
\text{ For every $\leq d$} & \text{ tuple $S$, $T$ that are permutations of each other } X_S = X_T
\end{align*}

The second last constraint follows from $x_i^2 = 1$ (to see this, check that the constraint holds for the intended solution for $X$). 

The last constraint are the symmetries of the intended rank 1 tensor solution.

This is the sum of squares SDP. What we can show is that for $d = n$ this is an exact relaxation! Now the vector version is not a good enough - so we think of distributions. 

To think of SDP solutions as distributions, we think of any feasible $X$ to the above SDP as the "moment-tensor" of the distribution. 

Recall that for a distribution $\mu$ over $\R^n$, the degree $\leq d$ moment tensor  $Q$ of $\mu$ is the following object:

$Q$ is indexed by tuples of size at most $d$. The entry at any tuple $$Q(i_1, i_2, ..., i_{d'}) = \E_{x \sim \mu}[] \Pi_{j\leq d'} x_{i_j'}].$$

Recall our intended relaxation that unfortunately wasn't efficiently optimizable  - the convex combinations of rank 1 tensors. That is (not hard to see) equivalent to the constraint that the $X$ is a $2d$-moment tensor of some distribution. As we discussed above, we can't hope to enforce that constraint efficiently. We instead did the symmetry + matrix-psd relaxation above. That captures only some properties of being a moment tensor so in actuality, we cannot assume that SDP solution is a moment tensor. 

Regardless, it turns out to be a good device in coming up with rounding algorithms to think of actual distributions and their moment tensors as solutions that the SDP returns. Usually, under fairly general situations, we can convert our ideas for actual distributions into those that work for these funny relaxations of them.

One of the properties (that is not hard to show) of a 2d degree SDP solution above is that over any 2d variables, the "marginal" SDP solution (that is "moments" restricted to only some 2d variables) is always an ACTUAL moment tensor.

Going to stop rambling now! :-)

\section{Gilbow-Zemel Construction: Independent Set to Game}
Given an undirected graph $G$ on $n$ vertices represented by an adjacency matrix $E$ (abuse of notation), we wish to check if it has an independent set of size $k\le n$ ($k$-IS). We will reduce this problem to checking if a two player game has more than one equilibrium. 

For $\delta \in (0, 1)$, $M>1$ , and $A=\ones_{n\times n} -E + \delta I_{n\times n}$, $B=-M* I_{n\times n}$ and $B'=k*I_{n\times n}$, consider the following $2n+1 \times 2n+1$ block matrices:
\[
R=\left[\begin{array}{cc}
\begin{array}{cc}
A & B\\
B' & \zeros_{n\times n}\\
\end{array}
& -M \ones_{2n \times 1}\\
(1+\frac{\delta}{k}) \ones_{1\times 2n} & 1+\frac{\delta}{k}
\end{array}\right]
\ \ \ \ \ \ 
C=\left[\begin{array}{cc}
\begin{array}{cc}
A & B'\\
B & \zeros_{n\times n}\\
\end{array}
& (1+\frac{\delta}{k}) \ones_{2n\times 1}\\
-M \ones_{2n\times 1}& 1+\frac{\delta}{k}
\end{array}\right]
\]

In the above contruction, submatrix $A$ has entry one in $(u,v)$th position if edge $(u,v)$ is {\em not present} in graph $G$, otherwise the entry is zero. Furhter, all its diagonals are $(1+\delta)$. Note that game $(R,C)$ is symmetric, i.e., $C=R^T$. For ease of notation let $m=2n+1$. For any given mixed strategy $\xx \in \Delta_{m}$, we will denote its support by $S(\xx)=\{i \ |\ x_i>0\}$. 


\begin{lemma}\label{lem:gz1}
$(\xx,\yy)$ is a NE of game $(R,C)$ where $S(\xx),S(\yy) \subseteq \{1,\dots,n\}$ iff graph $G$ has an independent set of size $k$. 
\end{lemma}
\begin{proof}
From independent set to NE is easy to see. Let $K\subset \{1,\dots,n\}$ be the vertices on the $k$-IS. Then setting $x_u=y_u=1/k,\ \forall u \in K$, and $x_u=y_u=0$ otherwise is a Nash equilibrium. This is because payoff from each non-zero strategy is $(1+\delta/k)$, and from strategies with zero probability it is at most $(1+\delta/k)$. 

To map NE supported on first $n$ strategies to an independent set in graph $G$, first observe that no matter what the column player is playing, row player gets $(1+\delta/k)$ from the last strategy $m$, and vice-versa. Therefore, all the non-zero strategies of both the players has to give at least $(1+\delta/k)$ payoff. Payoff of the row player from strategy $u \in S(\xx)$ is at most $1+\delta y_u$ implying $y_u \ge \frac{1}{k}$, in turn implying $u \in S(\yy)$. Same holds for the column player as well, giving us $S(\xx)=S(\yy)$, and $x_u,y_u \ge 1/k,\ \ \forall u \in S(\xx)$. The latter also implies that $|S(\xx)|=|S(\yy)|\le k$. 

Now suppose for some $u\neq v \in [n]$, we have $y_u,y_v>0$ and $E(u,v)=1\Rightarrow A(u,v)=0$. Then, we have $x_u,x_v>0$ and 
\[
\mbox{payoff}_1(u,\yy) + \mbox{payoff}_1(v,\yy) \le (1+\delta)(y_u+y_v) - 2 (1-y_u-y_v) < 2\ \ \ \ (\mbox{because } \delta<1)
\]

This is a contradiction to payoff being at leaset $(1+\delta/k)$. Therefore, it follows that vertices corresponding to $S(\xx)=S(\yy)$ form an independent set.

Now it suffices to argue that $|S(\yy)|=k$. To the contrary suppose $|S(\yy)|<k$. Let $j^* = \argmax_{j \le m} y_j$, then clearly $y_{j^*} \ge \frac{1}{k-1}$. 
Row player's payoff from any $i\in \{1,\dots, n\}$ is at most $1+\delta y_{j^*}<1+y_{j^*}$, where the inequality is due to $\delta<1$. While from strategy $n+j$ it is $k * y_{j^*} = (k-1) y_{j^*} + y_{j^*} \ge 1+y_{j^*}$, where the last inequality is due to $y_{j^*}\ge \frac{1}{(k-1)}$. A contradiction to $S(\xx)\subseteq \{1,\dots,n\}$. 
\end{proof}

\begin{lemma}\label{lem:gz2}
If $(\xx,\yy)$ is a Nash equilibrium of game $(R,C)$ then either $S(\xx),S(\yy) \subseteq \{1,\dots,n\}$ or $S(\xx)=S(\yy) = \{2n+1\}$. 
\end{lemma}
\begin{proof}
To the contrary suppose neither holds for $S(\yy)$. If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$ then $S(\xx)=\{m\}$, and vice-versa. This is because any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of $(1+\delta/k)$. Therefore, we have that $S(\yy) \not\subseteq\{n+1,\dots, 2n+1\}$ and hence $y_L =  \sum_{i=1}^n y_i \in (0, 1)$. The proof is based on a number of observations which we list next with a brief justification.
\begin{enumerate}
%\item If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$ then $S(\xx)=\{m\}$, and vice-versa: This is because any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of $(1+\delta/k)$. 
%\item If $\exists i \in S(\yy) \cap \{1,\dots,n\}$ such that $y_i \ge \frac{1}{k-1}$, then $S(\xx)\cap \{1,\dots,n\} = \emptyset$, and vice-versa: Let $i^* = \argmax_{i \le n} y_i$, then payoff of player one from strategy $n+i^*$ is $ky_{i^*}-My_m=(k-1)y_{i^*} + y_{i^*} -My_m\ge 1+y_{i^*}-My_m$. While for any $i\le n$, her payoff is at most $1+\delta y_i - M y_{n+i} - M y_m<1+y_{i^*}-My_m$. The claim follows.
\item $\forall i \in S(\xx)$, $(Ry)_i \ge 1+\delta/k$, and similarly for player two: This follows from the fact that the last strategy always gives $(1+\delta/k)$ payoff regardless of what the other player is playing. 
\item $\forall i\le n, x_i > 0 \Rightarrow y_i \ge \frac{1}{k}$, and $y_i>0 \Rightarrow x_i \ge \frac{1}{k}$: This follows from the fact that player one gets at most $(1+\delta y_i)$ payoff from strategy $i\le n$. Therefore using point (1), $x_i > 0 \Rightarrow (1+\delta y_i) \ge 1+\delta/k$, and the claim follows.  
%\item $\forall i\le n, x_{n+i}>0 \Rightarrow y_i \ge \frac{1}{k} + \frac{\delta}{k^2}$, and $y_{n+i}>0 \Rightarrow x_i \ge \frac{1}{k} + \frac{\delta}{k^2}$: Proof follows from the fact that payoff of the two players from strategy $(n+i)$ is $k*y_i$ or $k*x_i$ respectively. They need to be at least $(1+\delta/k)$ due to point (2).
%\item From point (4) it follows that $|S(\xx) \cap \{n+1,\dots,2n\}|\le (k-1)$ and $|S(\yy) \cap \{n+1,\dots,2n\} \le (k-1)$.
\item $y_L <1$ together with point (2) implies $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$. Point (2) also implies $S(\yy) \cap \{1,\dots,n\} =S(\xx) \cap \{1,\dots,n\}\Rightarrow |S(\yy) \cap \{1,\dots,n\}|\le (k-1)$. 
\end{enumerate}
From point (3) we know that $\exists i,i' \in S(\yy) \cap \{1,\dots,n\}$ such that $y_i \le y_L/a$ and $y_{i'}\ge y_L/a$, where $a=|S(\yy) \cap \{1,\dots,n\}|\ge (k-1)$ (because, $y_L>0$). And then point (2) implies $x_i>0$ as well. The payoff$_1(i) \le y_L + \delta y_i - M y_{n+i} - M y_m \le y_L + \delta y_i\le (1+\delta/a)y_L$, while the payoff$_1(n+i') = k y_{i'} \ge ky_L/a$. From (3) we have $a \le (k-1)$ and therfore 
\[
\mbox{payoff}_1(n+i') - \mbox{payoff}_1(i) \ge (k/a - 1 - \delta/a) y_L = (k - a - \delta)y_L/a \ge (1-\delta)y_L/a \ge (a/k) (1/2a) = 1/(2k)
\]
Last inequality follows taking $\delta\le 1/2$ and since we have $y_L \ge a/k$ using (2). %y_i \ge \frac{1}{k}$
This contradicts strategy $i$ being best response of player one against $\yy$. 
\end{proof}


\medskip\subsection{$1/n$ Approximation.} Note that in Lemma \ref{lem:gz1} when $|S(\yy)|<k$ then the difference in first player's payoff from its $j^*$th strategy and $(n+j^*)$th strategy is at least $(1-\delta)/(k-1)$. Now on we will set $\delta=1/2$, this gives $1/2(k-1)$ gap. Therefore, for $epsilon = \frac{1}{3k}$ and slightly modified game where last row of matrix $R$ and last column of matrix $C$ are set to $1+\frac{\delta}{k} + \frac{2\delta}{3k}$, Lemma \ref{lem:gz1} will follow even for $\epsilon$-approximate well-supported equilibrium. However, Lemma \ref{lem:gz2} is a bit tricky that we show next.


\begin{lemma}\label{lem:approx-gz2}
If $(\xx,\yy)$ is a $\frac{1}{3k}$-approximate well-supported Nash equilibrium of game $(R,C)$ then either $S(\xx),S(\yy) \subseteq \{1,\dots,n\}$ or $S(\xx)=S(\yy) = 2n+1$. 
%Given that graph $G$ does not have a clique of size $k$, if $(\xx,\yy)$ is a $\frac{1}{3k}$-approximate well-supported Nash equilibrium of game $(R,C)$ then either $S(\xx)=S(\yy)=\{2n+1\}$. % \in \{1,\dots,n\}$ or $S(\xx)=S(\yy) = 2n+1$. 
\end{lemma}
\begin{proof}
To the contrary suppose the claim does not hold for $S(\yy)$. Let $\epsilon = \frac{1}{3k}$. 
This proof is based on a number of observations which we list next with a brief justification.
\begin{enumerate}
\item $S(\yy) \cap \{1,\dots,n\} \neq \emptyset$ and $S(\xx) \cap \{1,\dots,n\} \neq \emptyset$: If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$, then $S(\xx)=\{2n+1\}$ since any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of at least $1$. In that case, by the same argument $S(\yy)=\{2n+1\}$, a contradiction. Second part follows similarly. 

\item $\forall i \in S(\xx)$, $(Ry)_i \ge 1+\delta/k$, and similarly for player two: This follows from the fact that the last strategy always gives $(R\yy)_m = (1+\delta/k + 2\delta/3k)$ payoff regardless of what the other player is playing, and that $(R\yy)_m -\epsilon = 1+\delta/k$. 

\item $\forall i\le n, x_i > 0 \Rightarrow y_i \ge \frac{1}{k}$, and $y_i>0 \Rightarrow x_i \ge \frac{1}{k}$: This follows from the fact that player one gets at most $(1+\delta y_i)$ payoff from strategy $i\le n$. Therefore using point (2), $x_i > 0 \Rightarrow (1+\delta y_i) \ge 1+\delta/k$, and the claim follows.  

\item $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$ and $|S(\yy) \cap \{1,\dots,n\}| \le (k-1)$: First we have assumed that $S(\yy) \not\subseteq \{1,\dots,n\}$, and therefore $y_L=\sum_{i\le n} y_i<1$. Then (3) implies $|S(\yy) \cap \{1,\dots,n\}| \le (k-1)$. Point (3) also implies $S(\xx) \cap \{1,\dots,n\} =S(\yy) \cap \{1,\dots,n\}$ giving us $|S(\xx) \cap \{1,\dots,n\}|\le (k-1)$ as well.
\end{enumerate}

From point (4) we know that $\exists i,i' \in S(\yy) \cap \{1,\dots,n\}$ such that $y_i \le y_L/a$ and $y_{i'}\ge y_L/a$, where $a=|S(\yy) \cap \{1,\dots,n\}|\ge (k-1)$ (because, $y_L>0$ due to point (1)). And then point (3) implies $x_i>0$ as well. The payoff$_1(i) \le y_L + \delta y_i - M y_{n+i} - M y_m \le y_L + \delta y_i\le (1+\delta/a)y_L$, while the payoff$_1(n+i') = k y_{i'} \ge ky_L/a$. Therfore 
\[
\mbox{payoff}_1(n+i') - \mbox{payoff}_1(i) \ge (k/a - 1 - \delta/a) y_L = (k - a - \delta)y_L/a \ge (1-\delta)y_L/a \ge (a/k) (1/2a) = 1/(2k)
\]
Last inequality follows since $\delta= 1/2$ and since we have $y_L \ge a/k$ using (3). This contradicts strategy $i$ giving at least best payoff minus $1/3k$ to player one against $\yy$, i.e., contradiction to $(\xx,\yy)$ being $\frac{1}{3k}$-approximate well-supported equilibrium.
\end{proof}

\begin{comment}
To allow assumption that $k$-clique does not exist in graph $G$ in the above lemma, 
%To allow graphs with $(k-1)$ sized clique, but no $k$ sized clique, 
we can make the above proof work by setting last row of $R$ and last column of $C$ to $1+\delta/(k-1)+\delta/2k^3$. This would also simplify the proof because essentially we will get lower bound of $1/(k-1)$ in point (3), and then point (4) will contradict it. 


For game constructed from graphs with $k$-clique, we want to ensure that no $\epsilon$-approximate equilibrium gives non-zero probability to the last startegy. We can do this by changing last row and last column of $R$ and $C$ respectively to $-1$. 

\noindent{\bf Question.} Now can we show that SDPs of these two games will have a common solution?

I will next try to see if the 3SAT example works as well. 
\end{comment}

==> content/Old/untitled.tex <==
%!TEX root=../main.tex
\section{Algorithmic Framework}

==> content/abstractGame-old.tex <==
%!TEX root=../main.tex
\section{Family of Hard Games: An Abstract Construction}
In this section we discuss a general method to construct family of games for which finding approximate NE using ``SoS relaxation + enumeration'' type methods is not possible. %to show hardness of approximation agains enumeration + SoS relaxation type of methods. 
For this we will first work with a stronger notion of approximation, namely $\epsilon$-well-supported NE (henceforth denoted by $\eps$-\WNE), described next.

We will use $[n]$ to denote set of numbers $\{1,\dots,n\}$.
\alert{Given an integer $n$ and a subset $T\subseteq[n]$, define vector $\ud{n,T}$ to be a probability distribution of size $n$ that is uniform on coordinates of $T$ and zero everywhere else, and when $T=[n]$ we use the short-hand notation $\ud{n}$.} 

\subsection{Well-Supported NE vs. Approximate NE}
For a two player game $(R,C)$, a strategy profile $(x,y)$ is an $\epsilon$-approximate well-supported Nash equilibrium ($\epsilon$-\WNE) iff \[\mbox{for every } i \leq n,\ x_i > 0 \Rightarrow \max_k e_k^{\top} R y -\epsilon \leq e_i^{\top} R y \ \ \ \mbox{ and } \ \ \ y_i>0 \Rightarrow \max_k x^{\top} C e_k-\epsilon \leq x^{\top} C y.\]

Strategies giving maximum payoff to a player are called her best response, and those giving at least maximum minus $\eps$ payoff $\eps$-best response, i.e. $\BR_1(\yy) = \{i\le n\ |\  e_i^{\top} A y = \max_k e_k^{\top} A y\}$ and $\eps$-$\BR_1(\yy) = \{ i \le n\ |\ x^{\top} A e_i \ge \max_k x^{\top} A e_k-\eps\}$, and similarly $\BR_2(\xx)$ and $\eps$-$\BR_2(\xx)$ can be defined. Let us denote support of a probability vector $\vv$ by $\Supp(\vv) = \{i\ |\ v_i>0\}$. 
Note that by definition, $(\xx,\yy)$ is an $\eps$-\WNE iff $\Supp(\xx) \subseteq \eBR_1(\yy)$ and $\Supp(\yy) \subseteq\eBR_2(\xx)$. 

\begin{lemma}\label{lem:ne-prop}
For any two player game $(A,B)$ with payoffs in $[0,1]$ the following holds. 
\begin{enumerate}
\item If $(x,y)$ is an NE iff $\Supp(\xx) \subseteq \BR_1(\yy)  \ \ \ \mbox{ and } \ \ \ \Supp(\yy) \subseteq \BR_2(\xx)$.
\item Every $\eps$-\WNE is $\eps$-$\NE$.
\item If $(\xx,\yy)$ is an $\eps$-$\NE$ then $\sum_{i \notin \sqrt{\eps}\mbox{-}\BR_1(\yy)} x_i \le \sqrt{\eps}$ and $\sum_{i \notin \sqrt{\eps}\mbox{-}\BR_2(\xx)} y_i \le \sqrt{\eps}$. 
\item Given $\eps$-$\NE$ $(\xx,\yy)$ we can construct $3\sqrt{\eps}$-\WNE $(\xx',\yy')$ such that $\Supp(\xx') \subseteq \sqrt{\eps}\mbox{-}\BR_1(\yy)$ and $\Supp(\yy') \subseteq \sqrt{\eps}\mbox{-}\BR_2(\xx)$. 
\end{enumerate}
\end{lemma}
\begin{proof}
Proofs of first and second part follows by definition. The argument that follows for the third and fourth part are essentially from the proof of Lemma 2.2 of \cite{CDT} due to Chen, Deng, and Teng.

For the third part, let $i^* \in \BR_1(\yy)$. Then, for each $i\notin \sqrt{\eps}\mbox{-}\BR_1(\yy)$ we have $(A\yy)_i < (A\yy)_{i^*} -\sqrt{\eps}$. Therefore, if $\sum_{i \notin \sqrt{\eps}\mbox{-}\BR_1(\yy)} x_i > \sqrt{\eps}$, then row player's payoff $\xx^{\top}A\yy < (A\yy)_{i^*} -\eps$, a contradiction. Similarly for $\yy$.

For the fourth part, for the construction of $(\xx',\yy')$ we will remove the probability mass from strategies outside $\sqrt{\eps}\mbox{-}\BR_1(\yy)$ and uniformly distribute them on strategies of $\sqrt{\eps}\mbox{-}\BR_1(\yy)$. Since payoffs are in $[0, 1]$, this will increase or decrease payoffs of any strategy at most by $\sqrt{\eps}$. Therefore, $(\xx',\yy')$ is $(3\sqrt{\eps})$-\WNE. And $\Supp(\xx') \subseteq \sqrt{\eps}\mbox{-}\BR_1(\yy)$ and $\Supp(\yy') \subseteq \sqrt{\eps}\mbox{-}\BR_2(\xx)$.
\end{proof}


\subsection{Abstract Game Construction}
% <<<<<<< HEAD
% Each of our reduction is from an NP-complete combinatorial problem. Such reductions are known to show hardness of decision versions of NE \cite{}. 
% Given such a combinatorial problem $\copt$ on graph $G=(V,E)$, like clique, independent set, etc., we define corresponding $\nice$-game as follows.
% \alert{Given an integer $n$ and a subset $T\subseteq[n]$, define vector $u(n,T)$ to be a probability distribution of size $n$ that is uniform on coordinates of $T$ and zero everywhere else.}  \Pnote{I use the notatino $\mathcal{U}_T$ for this distribution.}
% =======
%Each of our reduction is from an NP-complete discrete optimization problem. Such reductions are known to show hardness of decision versions of NE \cite{GW,CS,HK,DFS}. 

Our construction of the hard games are based on combining construction of integrality gap against Sum-of-Squares relaxations computing equilibria that maximize social welfare and games that are hard for enumeration based algorithms. We abstract out the properties of these two kinds of hard games in this section. Our hardness results in the next two sections will invoke the general combining strategy from this section. 

 

%Given such a discrete optimization problem $\copt$ of size $n$ such that its solution can be described by an index set $T\subseteq [n]$, {\em e.g.,} $k\le n$ sized independent-set in graph $G=(V,E)$ with $n$ vertices, we define corresponding $\nice$-game as follows.  

%graph $G=(V,E)$, like clique, independent set, etc., we define corresponding $\nice$-game as follows.


% \begin{definition}\label{def:nicegame}
% Given a discrete optimization problem $\copt$ of size $n$, parameters $\eps>0$ and $\delta>\eps$, we say that game $(R,C)$ is $(\eps,\delta)$-\nice with respect to (w.r.t.) $\copt$ if 
% \begin{enumerate}
% \item Matrices $R$ and $C$ are $N\times N$ where $N=\poly(n)$, first $n$ strategies of both players are associated with the $n$ elements of the discrete problem $\copt$, and the payoffs are in $[-1,1]$.
% \item \textbf{Completeness: } If $\copt$ has a solution $z \in \zo^n$ then profile $(\vv, \vv)$, where $\Supp(\vv)\subset[n]$ and first $n$ coordinates forms vector $\ud{n,T}$, is an $\eps$-\WNE of game $(R,C)$. % where both $\xx$ and $\yy$ are uniform distribution over the strategies corresponding to vertices in $T$. 
% And at this equilibrium, both the players get payoff of at least $\delta$. 
% \item \textbf{Soundness: } If $\copt$ has no solution, then every $\eps$-\WNE $(\xx,\yy)$ of $(R,C)$ has total payoff $\xx^{\top}(R+C)\yy < 2(\delta-\eps)$. 
% \end{enumerate}
% \end{definition}
First, we define two player games such that maximizing social welfare is hard for SoS.
\begin{definition}[Games Hard for SoS] \label{def:nicegame}
A game $(R,C)$ for $R,C \in [-1,1]^{N \times N}$ is said to be degree $t$, $(\epsilon,\delta)$-\nice if:
\begin{enumerate}
\item \textbf{Completeness: } There's a degree $t$ pseudo-distribution on $\epsilon$-$\NE$ of the game $(R,C)$ that have payoffs for both players at least $\delta.$
\item \textbf{ Soundness: } Every $\eps$-\WNE $(\xx,\yy)$ of $(R,C)$ has total payoff $\xx^{\top}(R+C)\yy < 2(\delta-\eps)$.
\end{enumerate}   
\end{definition}

%We note that the above game can also be defined for non-graph combinatorial problems as well, like 3-SAT. 
%We will use this game to plant SoS solution.

Next we need a game to construct the family of games with disjoint set of equilibria, and the property we need from these is as follows. 


\begin{definition}[Games Hard for Enumeration]
\label{def:goodgame}
A $K\times K$ game $(R_S,C_S)$ where $S\subseteq[K]$ is said to be $(\eps,\tau)$-\good for $\eps>0$ and $\tau>0$ if $R_S,C_S \in [-1, 1]^{K\times K}$, and 
\begin{enumerate}
\item For any strategy $\yy$ of the column player $\exists i \in [K]$ such that $(R_S\yy)_i \ge 1/2$, and vice-versa.
\item For any $\eps$-\WNE $(\xx,\yy)$ the following holds:
\begin{enumerate}
\item $\Supp(\xx)\subseteq S$. 
\item $||\xx - \ud{K,S}||_1 \le \tau\eps$. %where $u_S$ is the uniform distribution on the strategies of $S$. 
\end{enumerate}
\end{enumerate}
\end{definition}

% Given a discrete optimization problem $\copt$, and parameters $\eps>0$, $\eps<\delta\le 1/2$, and $\tau>0$, let $(R,C)$ be an $N\times N$ game that is an $(\eps,\delta)$-\nice w.r.t. $\copt$ where $N=poly(n)$.

Given parameters $1/2 \geq \delta > \eps>0$ and $\tau>0$, let $(R,C)$ be an $N\times N$ game that is degree $t$, $(\eps,\delta)$-\nice. And for $K=\poly(n)$ and $S\subset [K]$ let $(R_S,C_S)$ be an $(\eps, \tau)$-\good game of size $K\times K$. Construct game $(R',C')$ of size $(N+K)\times (N+K)$ as follows: 

\begin{equation}\label{eq:absGame}
R' = \left[\begin{array}{cc} R \ & \ -2 \\ \delta \ &\ R_S \end{array}\right]\ \ \ \mbox{ and } C' =\left[ \begin{array}{cc} C \ & \ \delta \\ -2 \ & \ C_S \end{array}\right]
\end{equation}

where the constants, namely $\delta$ and $-2$, represent matrices of appropriate size with all entries set to the stated constant. 

\begin{lemma}\label{lem:abstract}
%Given a combinatorial problem $\copt$ on graph $G=(V,E)$ on $n$ vertices, and parameters $\eps>0$ and $\eps<\delta\le 1/2$, let $(R,C)$ be an $(\eps,\delta)$-\nice game for $(G,\copt)$ of size $N\times N$ where $N=poly(n)$. And for $K=\poly(n)$ and $S\subset [K]$ let $(R_S,C_S)$ be an $(\eps)$-\good game of size $K\times K$. Construct 
%If the discrete problem $\copt$ does not have a solution, then 
For $0<\eps'<2\eps/3$ every $\eps'$-\WNE $(\xx,\yy)$ of game $(R',C')$ we have $\Supp(\xx), \Supp(\yy) \subset\{(N+1),\dots,(N+K)\}$. 
\end{lemma}
\begin{proof}
Let us denote $x_L = \sum_{i\in[N]} x_i$, $x_R=(1-x_L)$, $y_L=\sum_{i\in[N]} y_i$ and $y_R=(1-Y_L)$. It suffices to show that $x_L=y_L=0$.Suppose not, and $x_L>0$ or $y_L>0$. First we show that $x_L>0$ if and only if $y_L>0$. 
By construction, if $y_L=0$ then payoff of the row player from any $i\in[N]$ is $-2$ while from any $i>N$ it is $\delta>0$. In that case if $x_i$ is non-zero for an $i\in [N]$ then it contradicts $(\xx,\yy)$ being $\eps$-\WNE. Therefore, $x_L=0$. Simlarly, $x_L=0\Rightarrow y_L=0$ follows.

Next we show that if $x_L>0$ then it should be significantly bigger.
\begin{claim}\label{clm:1}
If $x_L>0$ then $x_L>2/3$. And if $y_L>0$ then $y_L>2/3$. 
\end{claim}
\begin{proof}
Let us prove the first part and the second part follows similarly. 
By property $(1)$ of \good game  $(R_S,C_S)$ there exists an $j\in\{(N+1),\dots, (N+K)\}$ such that payoff of the row player from strategy $j$, namely $(R'y)_j$, is at least $\delta y_L + \frac{y_R}{2}$. Therefore, if $x_L>0$ the strategy $i\in[N]$ with $x_i>0$ should have payoff at least $\delta y_L + \frac{y_R}{2} - \eps'$. On the other hand, payoff from any $i\le N$ is at most $y_L - 2y_R$, implying. 
\[
\begin{array}{lcl}
y_L - 2 y_R \ge \delta y_L + \frac{1}{2}y_R - \eps' & \Rightarrow & y_L (1-\delta) \ge 2.5 y_R -\eps \ \ \ (\because\ \eps>\eps') \\
& \Rightarrow & y_L(1-\delta) \ge 2.5  - 2.5y_L -\delta \ \ \ (\because \ \delta\ge \eps)\\
& \Rightarrow & y_L(3.5-\delta) \ge 2.5-\delta \Rightarrow y_L \ge 2/3 \ \ \ (\because\ \delta\le 1/2)
\end{array}\qedhere
\]
\end{proof}

Let $\hxx$ and $\hyy$ be truncation of $\xx$ and $\yy$ to first $N$ coordinates, and let $\hxx'=\hxx/x_L$ and $\hyy'=\hyy/y_L$ be their normalized vectors. Then, row player's payoff from $i \le N$ is $(R\hyy)_i -2y_R$. Furthermore, if $x_i>0$, then this payoff must be at least $\max_{k\le N} (R\hyy)_k - 2y_R - \eps' \ge \max_{k\le N} R(\hyy)_k - 2y_R -2\eps/3$. This implies, $\forall i\in[N],\ x_i>0 \Rightarrow (R\hyy)_i/y_L \ge \frac{1}{y_L}(\max_{k\le N} (R\hyy)_k - 2\eps/3) \Rightarrow (R\hyy')_i \ge \max_{k\le N} (R\hyy')_k - \eps$. The last implication uses $y_L>2/3$ from Claim \ref{clm:1}. Similarly, we can show that if $\forall i\in[N],\ y_i>0\Rightarrow (\hxx'^{\top}C)_i \ge \max_{k\in[N} (\hxx'^{\top}C)_i -\eps$. These two together implies that $(\hxx',\hyy')$ is an $\eps$-\WNE of game $(R,C)$. Therefore, by property $(2)$ of \nice games, $\hxx'^{\top}(R+C)\hyy'\le 2(\delta - \eps)\Rightarrow \hxx^{\top}(R+C)\hyy \le (\delta - \eps) x_L y_L$. 

We have either $\hxx^{\top}R \hyy< (\delta-\eps) x_L y_L$ or $\hxx^{\top}C \hyy< (1-\epshat) x_L y_L$. We will show contradiction for the former and the contradiction for the latter follows similarly by symmetry of construction. 


Suppose, $\hxx^{\top}R \hyy< (\delta-\eps) x_L y_L$. 
There exists $i\in [N]$ such that $x_i>0$ and $(R\hyy)_i < (\delta-\eps) y_L$. Therefore, $(R'\yy)_i = (R\hyy)_i - 2y_R < (\delta-\eps)y_L - 2y_R$. 
By property $(1)$ of \good game $(R_S,C_S)$, exists $j > N$ such that $(R'\yy)_{j} \ge y_L + \frac{y_R}{2} = y_L+2y_R$. By requirement of $\eps'$-\WNE, payoff from strategy $i$ above should be at least payoff from $j$ minus $\eps'$. This gives,

\[
(\delta-\eps) y_L - 2y_R > \delta y_L+\frac{y_R}{2} - \eps' \ge y_L+2y_R - \eps \Rightarrow (1-y_L) \eps> 2.5 y_R \Rightarrow \eps > 2.5 
\]
A contradiction.
%Again there exists $i\in [N]$ such that $y_i>0$ and $(\hxx^{\top}C)_i < (1-\epshat) x_L$. Therefore, $(\xx^{\top} C')_i = (\hxx^{\top}C)_i  - x_R < (1-\epshat)x_L - x_R$. 
%
%Similar to the previous case we will show that there is a strategy $i >N$ that give much better payoff, and thereby lead to a contradiction. Let $x_{R1} = \sum_{j \in S} x_{N+j}$ and $x_{R2}=x_R - x_{R1}$. Among the row player's strategies corresponding to $S$ consider those $l/2$ whose total probability is at least $\xx_{R1}/2$. Denote this set by $W$. By construction there exists a subset $S_t\subset S$ of size $l/2$ such that $S_t=W$. Then, column player's payoff from the strategy corresponding to $S_t$ is $(\xx^{\top} C'_S)_{(N+t)} \ge x_L + 4 x_{R1} + 2 x_{R2} \ge x_L + 2 x_R$. 
%Similar to the previous case, $\eps$-\WNE imposes $(\xx^{\top} C'_S)_i \ge (\xx^{\top} C'_S)_{(N+t)} - \eps \Rightarrow (1-\epshat)x_L - x_R > x_L + 2 x_R -\eps$. By the same argument as above it leads to a contradiction. 
\end{proof}


\begin{lemma}[Completeness]
There's a degree $t$ pseudo-distribution on $\eps$-$\NE$ of the game $(R',C').$
\label{lem:abstract-completeness} 
\end{lemma}
\begin{proof}
By construction of $(R',C')$ together with property $(1)$ of a degree $t$, $(\eps, \delta)$-\nice game, we know that there's a pseudo-distribution of degree $t$ on strategy profiles $(\xx,\yy)$ that form an $\NE$ for $(R,C).$ This immediately yields a pseudo-distribution $\pE$ on strategy profiles for the game $(R',C')$ by padding $\xx$ and $\yy$ with zeros on the last $K$ coordinates. We claim that this is a pseudo-distribution on $\NE$ of $(R',C').$ 

Since $\pE$ is a pseudo-distribution on equilibria of $(R,C)$, it satisfies the inequality constraints $\xx^{\top} R \yy \geq e_i^{\top} R \yy$ for every $i \leq N.$ Further, by property $(1)$, the $\pE$ satisfies the constraint $\xx^{\top} R \yy \geq \delta$. On the other hand, by construction of $(R',C')$, $e_i^{\top} R \yy \leq \delta$ since $\yy$ satisfies $\yy_i = 0$ for all $i \geq N+1.$ A similar argument shows that $\pE$ satifies the inequality constraint $\xx^{\top} C \yy \geq \xx^{\top} C e_i$ for every $i \leq N+K.$ This yields that $\pE$ satisfies the constraints of $\NE$ for $(R',C')$ as required. 
\end{proof}


% \begin{theorem}\label{thm:absGame}
% The following holds for game $(R',C')$.
% \begin{itemize}
% \item If $T\subset V$ is a solution to $\copt$ in $G$ then game $(R', C')$ has an $\eps$-\WNE $(\vv,\vv)$ where $\Supp(\vv) \subset[n]$, and first $n$ coordinates of $\vv$ form vector $\ud{n,T}$. 
% \item If graph $G$ has no solution to problem $\copt$, then for $0\le \epshat<\eps/15$ every $(4\epshat^2)$-$\NE$ $(\xx,\yy)$ of game $(R',C')$ satisfies $||\xx - (\zeros_{N}, \ud{K,S})||_1 \le 9(\tau+1)\epshat$, where $\zeros_N$ is an $N$ dimensional zero vector and $\ud{K,S}$ is a $K$ dimensional vector representing a uniform distribution over coordinates of $S$.
% \end{itemize}
% \end{theorem}

\begin{lemma}[Soundness]
%If graph $G$ has no solution to problem $\copt$, then 
For $0\le \epshat<\eps/15$ every $(4\epshat^2)$-$\NE$ $(\xx,\yy)$ of game $(R',C')$ satisfies $||\xx - (\zeros_{N}, \ud{K,S})||_1 \le 9(\tau+1)\epshat$, where $\zeros_N$ is an $N$ dimensional zero vector and $\ud{K,S}$ is a $K$ dimensional vector representing a uniform distribution over coordinates of $S$.
\label{lem:abstract-soundness}
\end{lemma}
\begin{proof}
% The first part essentially follows from construction of $(R',C')$ together with the property $(1)$ of an $(\eps,\delta)$-\nice game (Definition \ref{def:nicegame}). By construction of $\vv$ its truncation to first $n$ coordinates, call it $\hvv$, is a NE of game $(R,C)$ that satisfy property $(2)$. Therefore, payoffs of players at $(\vv,\vv)$ are respectively, $\vv^{\top}R\vv = \hvv^{\top} R'\hvv =\delta$ and $(\vv,\vv)$ are $\vv^{\top}C\vv = \hvv^{\top} C'\hvv =\delta$. If it is not a NE of game $(R',C')$ then the only incentive for players could be to move to a strategy $j>N$. However, such a strategy gives payoff at most $\delta$ to either player, which is the payoff at $(\vv,\vv)$.

%For the second part,
Note that additive scalling of payoff matrices preserves approximate NE, while multiplicative scaling scales the approximation factor by the same amount. Since every entry in $R', C'$ are in $[-2, 1]$ we first add $2$ to all of them and then divide them by $3$. Thus, $(\xx,\yy)$ is now $4\epshat^2/3$-NE of the scaled game, which is also its $\epshat^2$-NE. Lets denote the scalled game by $(\rh,\ch)$. 

Then by Lemma~\ref{lem:ne-prop}(4) there exists $(\xx',\yy')$ that is $3\epshat$-\WNE of game $(\rh,\ch)$, which is $9\epshat$-\WNE of game $(R',C')$. 
 Note that $9\epshat < 2\eps/3$. Applying Lemma \ref{lem:abstract} we get that $\Supp(\xx') , \Supp(\yy') \subseteq\{(N+1),\dots, (N+K)\}$. Therefore, strategy $(\xx',\yy')$ projected to last $K$ coordinates is a $9\epshat$-\WNE of game $(R_S,C_S)$. The latter is an $(\eps,\tau)$-\good game, whose property $(2.a)$ implies $||\xx' - (\zeros_N, \ud{K,S})||_1 \le 9\tau \epshat$. 

If we get an upper bound on $l_1$ distance between $\xx$ and $\xx'$, then due to triangle inequality we will get an upper bound on $l_1$ distance between $\xx$ and $\ud{K,S}$. By construction of $(\xx',\yy')$, we have that $\Supp(\xx') \subseteq \epshat$-$\BR_1(\yy)$ and $\Supp(\yy') \subseteq \epshat$-$\BR_2(\xx)$. Furthermore, Part $(3)$ of Lemma \ref{lem:ne-prop} implies $\sum_{i \notin \ehBR_1(\yy)} x_i \le \epshat$ and $\sum_{i\notin\ehBR_2(\xx)} y_i \le \epshat$. While constructing $\xx'$ from $\xx$ we set the probability of all strategies not in $\ehBR_1(\yy)$ to zero and redistribute their mass to strategies in $\ehBR_1(\yy)$ uniformly. Therefore, $||\xx - \xx'||_1 \le 2\epshat$. Finally, $||\xx - (\zeros_N, \ud{K,S})||_1 \le ||\xx - \xx'||_1 + ||\xx' - (\zeros_N, \ud{K,S})||_1 \le (9\tau+2)\epshat$. 
\end{proof}

Using the \nice game and a family of \good games on far-apart sets, next we construct a family of hard games. The proof of the next theorem will crucially use Lemmas \ref{lem:abstract-soundness} and \ref{lem:abstract-completeness}.
% Theorem \ref{thm:absGame}. 

\begin{theorem}\label{thm:absFamily}
Given parameters $\eps>0$, $\delta>\eps$ and $\tau>0$,% and a discrete optimization problem $\copt$ of size $n$, % graph $G=(V,E)$ on $n$ vertices with combinatorial problem \copt, 
\begin{itemize}
\item[$(h_1)$] let $(R,C)$ be a degree $t$, $(\eps,\delta)$-\nice game of dimension $N\times N$. % w.r.t. $\copt$, where $N=\poly(n)$,
\item[$(h_2)$] and for $K=\poly(n)$ and subsets $S_1,\dots, S_f$ of $[K]$ such that $||\ud{K,S_i} - \ud{K,S_j}||_1 > 18(\tau+1)\eps$, let $(R_{S_i}, C_{S_i})$ is a $(\eps,\tau)$-\good game for each $i\in\{1,\dots,f\}$. 
\end{itemize}

Then, for the family of games $\CF=\{\CG_i\ |\  \CG_i= (R'_i,C'_i) \mbox{ is the game of \eqref{eq:absGame} using $(R,C)$ and $(R_{S_i},C_{S_i})$}\}$, the following hold.
\begin{enumerate}
\item There's a degree $t$ pseudo-distribution supported on $\eps$-$\NE$ for \emph{every} $\CG_i \in \CF$. 
\item %If $\copt$ does not have a solution, then 
For any pair of games $\CG_i \neq \CG_j \in \CF$, their set of $\eps'$-$\NE$ do not intersect, where $0\le \eps' \le (\eps/8)^2$.
\end{enumerate}
\end{theorem}


% \begin{theorem}\label{thm:absFamily}
% Given parameters $\eps>0$, $\delta>\eps$ and $\tau>0$, and a discrete optimization problem $\copt$ of size $n$, % graph $G=(V,E)$ on $n$ vertices with combinatorial problem \copt, 
% \begin{itemize}
% \item[$(h_1)$] let $(R,C)$ be a degree $t$, (\eps,\delta)$-\nice game of dimension $N\times N$. % w.r.t. $\copt$, where $N=\poly(n)$,
% \item[$(h_2)$] and for $K=\poly(n)$ and subsets $S_1,\dots, S_f$ of $[K]$ such that $||\ud{K,S_i} - \ud{K,S_j}||_1 > 18(\tau+1)\eps$, let $(R_{S_i}, C_{S_i})$ is a $(\eps,\tau)$-\good game for each $i\in\{1,\dots,f\}$. 
% \end{itemize}

% Then, for the family of games $\CF=\{\CG_i\ |\  \CG_i= (R'_i,C'_i) \mbox{ is the game of \eqref{eq:absGame} using $(R,C)$ and $(R_{S_i},C_{S_i})$}\}$, the following hold.
% \begin{enumerate}
% \item If $T\subset [n]$ is a solution of \copt, then $(\vv,\vv)$ where $\vv=(\ud{n,T},\zeros_{N+K-1})$, is an $\eps$-\WNE of game $\CG_i$, for all $\CG_i \in \CF$. 
% \item If $\copt$ does not have a solution, then for any pair of games $\CG_i \neq \CG_j \in \CF$, their set of $\eps'$-$\NE$ do not intersect, where $0\le \eps' \le (\eps/8)^2$.
% \end{enumerate}
% \end{theorem}
\begin{proof}
The first part for each game $\CG_i$ follows from the first part of Lemma \ref{lem:abstract-completeness}. %\ref{thm:absGame} 
For the second part, let $(\xx^i,\yy^i)$ and $(\xx^j,\yy^j)$ be $\eps'$-$\NE$ of games $\CG_i$ and $\CG_j$ respectively. If we think of $\eps' = 4\epshat^2$ then clearly $\epshat <\eps/5$ is satisfied, then using Lemma \ref{lem:abstract-soundness},
 %second part of Theorem \ref{thm:absGame}, 
 we have $||\xx^i - (\zeros_N, \ud{K,S_i})||_1 \le 9(\tau+1)$ and $||\xx^j - (\zeros_N, \ud{K,S_j})||_1 \le 9(\tau+1)$. If $\xx^i=\xx^j$ then by triangle ineuality of $l_1$ norm, $||\ud{K,S_i} - \ud{K,S_j}||_1 \le 18(\tau+1)\eps$, a contradicition to an assumption in the hypothesis.
\end{proof}




==> content/algorithmic-framework.tex <==
%!TEX root=../main.tex
\section{Algorithmic Framework and Formal Statement of Results}
% In this paper, we will analyze the utility of convex relaxations in computing exact/approximate equilibria. The classical paradigm for approximation algorithm design using convex relaxations involves writing a convex relaxation for some intractable formulation of the underlying problem and then \emph{rounding} the solution to the relaxation to obtain an \emph{actual} solution. Our algorithmic framework would involve using the degree $d$ (for a parameter $d$) SoS relaxation for the quadratic programming formulation for $\NE$ and $\epsilon$-$\NE$ followed by a broad but restricted class of rounding algorithms. As we will see, the restriction on the rounding would come from the necessity of forcing the rounding procedure to ``use'' the solution to the convex relaxation. 

% In what follows, we define two classes of rounding algorithms for algorithmic problems in general and explain why they form a meaningful class to look at. We will then specialize the discussion to $\NE$ and $\epsilon$-$\NE$.

% An algorithmic problem for us will be described by a pair $(V,X)$. We think of $V$ as all possible instances of some fixed size for the problem and $X$ as the space where any solution to any instance lives. The goal of the problem given


% \begin{definition}[Oblivious Rounding for $\NE$/$\epsilon$-$\NE$]
% For any game $(A,B)$, let $\C(A,B)$ be a convex relaxation for the quadratic programming formulation of $\NE$/$\epsilon$-$\NE$ for the game described by $(A,B)$. A rounding algorithm for $\C$ takes input a solution to $\C(A,B)$ (but not $A,B$ themselves) and outputs a strategy profile $(\xx,\yy)$ that forms an $\NE$/$\epsilon$-$\NE$ for $(A,B).$
% \end{definition}




% \begin{definiteach of degree at most $d$ and outputs either ``infeasible'' or either outputsreturns a degree $d$ pseudo-expectation $\pE_{\tmu}i satisfying the above constraints.on$[Sum-of-Squares Algorithm] \end{definition} Fact \ref{fact:reductions-within-SoS} implies that the degree $d$ SoS algorithm runs in time $n^{O(d)}.

\subsection{The Model: Oblivious Rounding with Verification} 
In this section, we present our algorithmic framework based on restricted roundings of sum-of-squares relaxation for polynomial feasibility problems. Let $\Psi(P)$ be a system of polynomial inequalities in $x \in \R^n$ parameterized by $P \in \R^m$. We allow $P$ to vary in some domain and interpret each different valid value of $P$ as a new instance. For example, the natural quadratic programming formulation for finding equilibria is a system of degree 2 polynomial inequalities over $\Delta_n \times \Delta_n$ parameterized by the payoff matrices $A,B$ that encode instances of two-player games. 


We can now define two algorithmic models that use sum-of-squares relaxations to find solutions to polynomial feasibility program $\Psi(P).$

\begin{definition}[Oblivious Rounding]
Let $\Psi(P)$ be a polynomial feasibility problem parameterized by instances $P$. An degree $d$ oblivious rounding algorithm for $\Psi(P)$ takes input a degree $d$ pseudo-expectation satisfying the constraints in $\Psi(P)$ and outputs a point $x \in \R^n$ that satisfies $\Psi(P).$
\end{definition}

Oblivious rounding for generic combinatorial optimization problems has received significant attention in works beginning with Feige who observed that most natural algorithms based on rounding LPs/SDPs are in fact oblivious rounding algorithms. He also observed some notable exceptions such as the Facility Location algorithm of \cite??, the generic rounding algorithm for Raghavendra and Steurer for constraint satisfaction and \cite??. This list in fact can be expanded as most of the recent works on roundings sum-of-squares relaxations for various polynomial optimization problems are \emph{not} oblivious. The CSP rounding algorithm of Raghavendra-Steurer and the recent algorithms based on rounding the SoS hierarchy for various polynomial optimization problem all can be seen as generating a small list of candidate solutions based on the SoS solution and then arguing that one of the candidates is a good solution to the problem at hand. 

Inspired by these algorithms, we generalize our framework to allow generating a list of candidates based on the SoS solution to yield the central algorithmic model of interest in this work. This allows us to capture all known rounding algorithms mentioned above with the exception of the facility location algorithm of...and \cite??.

For every instance of the underlying problem encoded by $\Psi(P)$, we define the \emph{verification oracle} as follows. 

\begin{definition}[Verification Oracle]
Let $\Psi(P)$ be a polynomial feasibility problem over $\R^n$. A verification oracle for $P$ takes input a $y \in \R^n$ and accepts if $y$ satisfies every polynomial inequality in $\Psi(P)$ and rejects otherwise.
\end{definition}


\begin{definition}[Oblivious Rounding with Verification Oracle]
Let $\Psi(P)$ be a polynomial feasibility problem parameterized by instances $P$. An degree $d$, $q$ query oblivious rounding with verification algorithm for $\Psi(P)$ takes input a degree $d$ pseudo-expectation satisfying the constraints in $\Psi(P)$ and outputs a list of $q$ points $x_1, x_2, \ldots, x_q \in \R^n$ such that at least one of the $x_i$s satisfies $\Psi(P).$
\end{definition}


\subsection{Our Results}
We are now ready to describe our main results.

Observe that the algorithm of Lipton-Markakis-Mehta is a degree $0$, $n^{O(\log{(n)}/\epsilon^2}$-query algorithm for finding $\epsilon$-approximate equilibria in two-player games. We show that there's an oblivious rounding algorithm for degree $O(\log{(n)}/\epsilon^2)$ SoS relaxation for finding $\NE$ that finds sparse $\epsilon$-$\NE$. This, in particular, yields a non enumerative algorithm matching the guarantees of the LMM algorithm. 


\begin{theorem}
There's a degree $O(\log{(n)}/\epsilon^2)$, oblivious rounding algorithm (with zero queries to the verification oracle) for finding $\epsilon$-approximate equilibria in two-player games with $n$ strategies.
\end{theorem}

This result shows that SoS relaxations for computing equilibria can be quite powerful and thus motivates the question of understanding whether we can round SoS solutions to good equilibria. Our next result shows a strong limitation of this approach and provides an exponential lower bound on algorithms using oblivious rounding with verification oracle for computing $\Theta(1/n)$-approximate equilibria in two-player games with $n$ strategies. 

\begin{theorem} \label{thm:main-exact}
Suppose there exists a degree $d$, $q$-query algorithm for computing $\Theta(1/n)$-approximate equilibria in two-player games with $n$ strategies. Then, either $d = \Omega(n)$ or $q = 2^{\Omega(n)}.$
\end{theorem}

Our second result is a similar statement for constant-approximate equilibria.
\begin{theorem} \label{thm:main-approx}
Suppose there exists a degree $d$, $q$-query algorithm for computing $\epsilon$-approximate equilibria in two-player games with $n$ strategies for some small enough $\epsilon = \Theta(1)$. Then, either $d = \Omega(\log{(n)})$ or $q = n^{\Omega(\log{(n)}}.$
\end{theorem}


\begin{remark}
\WNE is a stronger notion of approximation that has been widely studied. The above lower bounds follow for it as well. 
Digging further into our results, it turns out that we can show exponential lower bounds for $O(1/n^2)$ approximation, and quasi-polynomial for much better constant factor approximation. Furthermore, all results can be extended to even more powerful oracle that is only possible for \WNE, namely take supports of both players' strategies, and output if there is an $\eps$-\WNE with the given support.
To keep the exposition clean and intuitive, we stick to $\NE$. 
\end{remark}


==> content/constant-approximate-old.tex <==
%!TEX root=../main.tex
\section{Quasipolynomial Hardness for Finding Approximate Equilibria}
The goal of this section is to prove Theorem \ref{thm:main-approx}. Concretely, we will show the following result which can be seen to immediately imply Theorem \ref{thm:main-approx}.



\begin{theorem} [Quasi-polynomial Hardness for Approximate $\NE$]
For every $m$ large enough, there's a family of $N = m^{\Omega(\log{(m)})}$ two-player games $\{(A_i,B_i)\}_{i = 1}^{N}$ with $m$ pure strategies for both players and all payoffs in $[-1,1]$ such that:
\begin{enumerate}
\item \textbf{Completeness:} There exists a pseudo-distribution $\tmu$ of degree $\Theta(\log{(m)})$ that satisfies the constraints of \FIXME for finding $\epsilon$-$\NE$ in every $G_i$ simultaneously for some absolute constant $\epsilon.$
\item \textbf{Soundness:} For any $i,j$ and any pair of $\epsilon$-$\NE$ in $G_i$, $G_j$, say $(\xx,\yy)$ and $(\xx',\yy')$ respectively, $\norm{\xx-\xx'} > \FIXME.$ %\norm{\yy-\yy'} > \FIXME.$
\end{enumerate}
\label{thm:approx-nash-hardness-technical}
\end{theorem}

Again we will use the meta-result of Theorem \ref{thm:absFamily} to prove this result. For this essentially we need to constrcut one \nice game and a family of $m^{\Omega{\log{(m)}}}$ \good games for a constant $\epsilon$. 

\subsection{Constructing \nice and \good games}
We will next show construction of \nice and \good games for a constant $\eps>0$. 


\Rnote{Lemma from Arrow}
\begin{lemma}[Games Hard for SoS] \label{lem:sos-hard-approximate}
There exists a game $(R,C)$ for $R,C \in [-1,1]^{N \times N}$ such that for $t = \Omega(\log{(N)})$, $(R,C)$ is a degree $t$, $(\epsilon,\delta)$-\nice game.   
\end{lemma}


We employ the recent reduction due to \cite{Deligkas-...} to construct $(R,C)$ via reduction from the \emph{free game} who recently showed ETH-hardness for maximizing social welfare in bimatrix games. We observe that their reduction also yields a SoS hard game by a direct application of Fact \ref{fact:reductions-within-SoS}. We remark that a recent work of \cite{Arrow..} also shows SoS hardness for a certain decision problem associated with computing equilibria by working through the hardness reduction of \cite{BKW}. However, their result does not prove SoS-hardness of maximizing social welfare. Since such a result would be of interest (beyond our application in obtaining hardness against rounding algorithms), we state it below in a more direct form which immediately implies Lemma \ref{lem:sos-hard-approximate} (indeed, it's essentially equivalent to Lemma \ref{lem:sos-hard-approximate} up to the distinction between $\epsilon$-\WNE and $\epsilon$-$\NE$.)

\begin{lemma}
There exists a game $(R,C)$ for $R,C \in [-1,1]^{N \times N}$ such that 
\begin{enumerate}
\item \textbf{Completeness: } There's a degree $t$ pseudo-distribution on $\epsilon$-$\NE$ of the game $(R,C)$ that have payoffs for both players at least $\delta.$
\item \textbf{ Soundness: } Every $\eps$-$\NE$ $(\xx,\yy)$ of $(R,C)$ has total payoff $\xx^{\top}(R+C)\yy < 2(\delta-\eps)$.
\end{enumerate}
\end{lemma}

\subsection{The Reduction}
In this section, we present the reduction of Deligkas et. al. The starting point is the hardness of approximation for the 3SAT problem. While for ETH-hardness, one has to start from worst-case hard instance of 3SAT and apply the PCP theorem to get a hard-to-approximate instance, for SoS-hardness, we can simply start from the random instance of 3SAT and use Grigoriev's theorem to get exponential SoS-hardness of approximating 3SAT. Alternatively, one can view this as saying that ETH is unconditionally true when restricted to the SoS framework and in fact the hard instance is simply a random one!

\begin{fact}[Grigoriev's Theorem] \label{fact:Grigoriev}
Let $\phi$ be a random instance of 3SAT with $m =\Theta(n/\epsilon^2)$ constraints and $n$ variables. Then, with probability at least $1-1/n$, 
\begin{itemize}
\item For every $x \in \zo^n$, the fraction of clauses satisfied in $\phi$ by $x$ is at most $7/8+\epsilon$, and
\item there exists a degree $\Theta(n)$ pseudo-distribution over the satisfying assignments for the instance $\phi.$
\end{itemize}
\end{fact}

Given a hard instance of 3SAT, one transforms it into a 2 prover, \emph{free} game. 

Recall that a two prover game is defined by a distribution $\cD$ over a finite set of question pairs $(Q_1, Q_2)$ with a collection of admissible answer pairs and two players Alice and Bob. In a run of the game, the referee draws a question pair $(Q_1, Q_2)$ from $\cD$ and sends $Q_1$ to Alice and $Q_2$ to Bob and receives answers from them and accepts if the answer pair is in the list of admissible answer pairs for $(Q_1, Q_2).$ A two prover game is said to be \emph{free} if $\cD$ is a product distribution.

A \emph{strategy} for a two prover game is a  pair of functions $f_1$ and $f_2$ that maps questions to an answer. The value of the strategy is the probability that  $(f_1(Q_1),f_2(Q_2))$ belongs to an admissible answer pair for the question pair $(Q_1, Q_2)$ picked at random from $\cD.$



\begin{definition}[Free Game from 3SAT] \label{def:free-game}
Let $\phi$ be a 3SAT instance from Fact \ref{fact:Grigoriev} with $m$ clauses and $n$ variables. 
Let the clauses and variables appearing in $\phi$ each be partitioned into $\sqrt{n}$ different groups, say, $S_1, S_2, \ldots, S_{\sqrt{m}}$ and $T_1, T_2, \ldots, T_{\sqrt{n}}$, respectively. Then, $\phi$ defines a free game as follows:

Let $\cD$ be the uniform distribution on $(S_i,T_j)$ for $i \sim [\sqrt{m}], j \sim [\sqrt{n}]$ define the distribution on question pairs. For $(S_i,T_j)$, an admissible answer pair is an assignment to the variables appearing in each clause in $S_i$ and each variable in $T_j$ such that 1) every clause in $S_i$ is satisfied by the assignment chosen 2) for every variable that appears in some clause in $S_i$ and in $T_j$, the assignments given by the answer pairs match.  

Note that the number of strategies for Merlin 1 are at most $N_1 = 2^{3\sqrt{m}}$ and that for Merlin 2, at most $N_2 = 2^{\sqrt{n}}.$
\end{definition}

The following completeness result holds for every free game produced from 3SAT instances from Fact \ref{fact:Grigoriev}. 
\begin{lemma}[SoS Completeness for Free Game]
Let $\phi$ be the 3SAT instance with $m = \Theta(n/\epsilon^2)$ clauses and $n$ variables from Fact \ref{fact:Grigoriev}. 
Let $\cF$ be the free game constructed in Definition \ref{def:free-game} from $\phi.$  
Then, there's a pseudo-distribution of degree $\Theta(n)$ on strategies of $\cF$ that value $1$.
\end{lemma}
\begin{proof}
We will start from the pseudo-distribution of degree $\Theta(n)$ given to us by Fact \ref{fact:Grigoriev} that satisfies every constraint of $\phi$ and use Fact \ref{fact:reductions-within-SoS}. To do this, we need to build a low-degree map from any satisfying assignment $x$ of $\phi$ to a strategy for the Merlins in the free game $\cF$. This is very simple: for any question set $(S_i,T_j)$ - the strategy is described by a bit string of length $3 \sqrt{m}$ and $\sqrt{n}$ respectively - where the bit string corresponds to the assignment for the variables appearing in the clauses in $S_i$ and variables in $T_j$ respectively. Using $x_i$ as the assignment for the variable $i$ wherever it appears gives a degree 1 map into strategies of $\cF$. It is easy to see that since $x$ (purportedly) satisfies all constraints of $\phi$, it satisfies all clauses in $S_i$ and further, the assignments to variables appearing in both $S_i$ and $T_j$ match. Thus, we obtain a degree $1$ map from any satisfying assignment $x$ into a strategy for $\cF$ with value $1$. By Fact \ref{fact:reductions-within-SoS}, we immediately obtain a pseudo-distribution of degree $\Theta(n)$ on strategies with value $1$ for $\cF$.

\end{proof}

The following soundness result holds for the partitions $S_1, S_2, \ldots, S_{\sqrt{m}}$ and $T_1, T_2, \ldots, T_{\sqrt{n}}$ chosen appropriately (we invite the reader to find the details of the reduction in Deligkas et. al...):

\begin{fact}[Soundness, \cite{?}]
There is no strategy for $\cF$ produced from $\phi$ in Fact \ref{fact:Grigoriev} with value exceeding $1-\Omega(1).$
\end{fact}

Next, we describe the relevant aspects of the reduction shown in Deligkas et. al. 

\begin{fact}[\cite{??}]
Let $\cF$ be a free game with $\sqrt{m}$ ($\sqrt{n}$, respectively) possible questions and $N_1$ ($N_2$, respectively) possible strategies for Merlin 1 (2, respectively.)  
Then, there's a two player game with $\sqrt{m} \cdot N_1$ strategies for the row player and $\sqrt{n} \cdot N_2$ strategies for the column payer such that: 
\begin{enumerate}
\item \textbf{Completeness: }

\item \textbf{Soundness: }
\end{enumerate}

\end{fact}


\subsubsection{\good games with constant $\eps$}
In this section we will construct a two-player game parameterized by a subset of strategies such that: $(i)$ both players' strategies at Nash equilibrium is largely supported on the subset, and $(ii)$ for a constant $\eps$, all its $\eps$-\WNE are near the actual NE. Daskalakis and Papadimitriou \cite{} gave a construction that ensures row-player's all \WNE strategy being near the uniform distribution over the subset. Constructing such a game for $n^{log(n)}$ carefully selected subsets, they showed non-existence of an oblivious PTAS under Oracle \ref{}, i.e., checks if given profile is a \WNE. However, in their construction the column player's NE (\WNE) strategies are common across games. Therefore it breaks under our more powerful Oracle \ref{}, {\em i.e.,} given any {\em one} player's strategy the oracle either outputs corresponding NE profile, or says no NE corresponding to the given strategy exists.

Since we need hardness against Oracle \ref{}, construction of \cite{DP} can not be used directly. We will have to ensure that, for each player, her NE strategy sets are far apart across games. Our construction builds on that of \cite{DP}, and therefore first we discuss the latter and its result. 

\paragraph{Construction of \cite{DP}.} Let $l$ be an even integer and $n={l \choose l/2}$. For each $S\subset [n]$ of size $l$, we will construct an $n \times n$ game. Fix such a subset $S$, and denote the corresponding game by $(A_S, B_S)$. In this game, row player cares about only strategies from $S$, {\em i.e.,} strategies outside of $S$ are strictly dominated by that of $S$. Since $|S|$ is $l$, number of $(l/2)$ sized subsets of $S$ are exactly $n$.  
The $n$ strategies of the column player correspond to these $(l/2)$ sized subsets of set $S$. In other words, if $S_1,\dots,S_{{l \choose l/2}}$ are all the $(l/2)$ subsets of $S$, then think of column player's strategies being indexed by these subsets. 
The payoffs in column $j$, corresponding to subset $S_j$ of $S$, are:

\begin{itemize}
\item For each $i\notin S$, set $A_S(i,j)=-1$ and $B_S(i,j)=1$.
\item For each $i \in S\cap S_j$, set $A_S(i,j)=1$ and $B_S(i,j)=0$.
\item For each $i \in S\setminus S_j$, set $A_S(i,j)=0$ and $B_S(i,j)=1$.
\end{itemize}

\begin{theorem}{\cite{DP}}
\begin{itemize}
\item[$(a)$] For any given $\eps < 1$, if $(\xx,\yy)$ is an $\eps$-\WNE of game $(A_S,B_S)$, then $(i)$ for all $i \notin S$, $x_i=0$, and $(ii)$ $||\xx - \ud{S}||_1 \le 8 \eps$.
\item[$(b)$] For $V=\{\ud{S} \ |\ S\subseteq[n], |S|=l\}$, $|V|= \Omega(n^{0.8\log_2 n})$. And for any $c>0$ there exists $V'\subset V$ of size $\Omega(n^{(0.8-2c\eps)\log_2 n})$ such that for any two vectors $\ud{S}, \ud{S'}\in V'$ we have $||\ud{S'} - \ud{S}||_1 > c\eps$.
\end{itemize}
\end{theorem}

Note that, column player playing each of its $n$ strategies uniformly at random is her NE strategy in game $(A_S,B_S)$ for all $S\subset [n]$ of size $l$. Thus querying Oracle \ref{} with strategy $\yy=\ud{[n]}$ for the column player will return a NE or of the given game. To prevent this next we combine two games of \cite{DK}, where the roles of the two players are switched in the second game. To ensure that both players put non-trivial probability mass on both games, we combine it with the matching-pennies game. 

\paragraph{Our Construction.}
Again fix an even integer $l$ and let $n={l \choose l/2}$. Fix an $l$ sized subset $S\subset [n]$, and corresponding game $(A,S, B_S)$ as described above. We construct a $2n \times 2n$ game $(R_S, C_S)$ as follows: if we think of matrices of this game as $2 \times 2$ block matrix, each block of size $n\times n$, then

\begin{equation}\label{eq:const-goodgame}
R_S = \left[\begin{array}{cc}2+A_S & -2\\
-2 & 2+B_S^{\top}\end{array}\right]
\ \ \ \ \ 
C_S = \left[\begin{array}{cc}-2+B_S & 2 \\
2 & -2+A_S^{\top} \end{array}\right]
\end{equation}

In \eqref{eq:cont-goodgame}, the constants $2$ and $-2$ represents block matrices of size $n\times n$ with all entries set to $2$ and $-2$ respectively. 
For any strategy profile $(\xx,\yy)$ of game $(R_S,C_S)$, let us divide each of $\xx$ and $\yy$ into two vectors corresponding to first $n$ and last $n$ strategies. These are $\xx^L = (x_1,\dots,x_n)$, $\xx^R = (x_{(n+1)},\dots,x_{2n})$, $\yy^L=(y_1,\dots,y_n)$, and $\yy^R=(y_{(n+1)},\dots,y_{2n})$. For any vector $\vv$, we will use $\sigma(\vv)$ denote sum of its coordinates $(\sum_i v_i)$. 

Using the matching pennies property of game $(R_S,C_S)$, next we show that both $\xx^L$ and $\xx^R$ have enough probability mass, and similarly $\yy^L$ and $\yy^R$.
\begin{lemma}
For an $\eps\in [0,1)$, let $(\xx,\yy)$ be an $\eps$-\WNE of game $(R_S,C_S)$. Then, 
$\frac{9}{19} - \frac{\eps}{9} \le \sigma(\xx^L), \sigma(\xx^R), \sigma(\yy^L), \sigma(\yy^R) \le \frac{10}{19} +\frac{\eps}{9}$. 
\end{lemma}
\begin{proof}
First we show that $\sigma(\xx^L), \sigma(\xx^R), \sigma(\yy^L), \sigma(\yy^R) >0$. To the contrary suppose $\sigma(\xx^R)=0$, then column player gets payoff at most $-1$ from any stragety $j \le n$, while gets payoff of $2$ from any $k > n$. Therefore $\sigma(\yy^L)=0$. In that case, the row player gets payoff at most $-1$ from any $i \le n$, while gets at least $2$ payoff from any $h>n$. Since there exists $i \le n$ such that $x_i>0$, this contradicts $(\xx,\yy)$ being $\eps$-\WNE. Similar argument follows for each of $\sigma(\xx^L), \sigma(\yy^L), \sigma(\yy^R)$ being zero.

Next we will argue that $\frac{9}{19} - \frac{\eps}{9} \le \sigma(\yy^L) \le \frac{10}{19} +\frac{\eps}{9}$, and then using $\sigma(\yy^R)=1-\sigma(\yy^L)$ the inequalities will follow for $\sigma(\yy^R)$ as well. For this we need properties of payoffs from $A_S$ and $B_S$ blocks of $R_S$. 

\begin{claim}\label{cl:const1}
For all $k \le n$ we have $(A_S\yy^L)_k \le 1$ and $(B_S^{\top}\yy^R)_k \le 1$, and there exists an $i,i'\le n$ such that $(A_S\yy^L)_i \ge \frac{\sigma(\yy^L)}{2}$ and $(B_S^\top \yy^R)_{i'}\ge \frac{\sigma(\yy^R)}{2}$. 
\end{claim}
\begin{proof}
The first part follows by the fact that coordinates of both $A_S$ and $B_S$ are at most one. For the second part, note that for each column $j\in[n]$ of $A_S$ exactly $(l/2)$ coordinates are $1$ out of $l$ coordinates of $S$. Therefore, summing up payoffs corresponding to strategis of $S$, we have
\[
\sum_{i \in S} (A_S\yy^L)_i = \sum_{j \le [n]} \yy^L *(l/2) = \sigma(\yy^L) (l/2)
\]
Since $|S|$ is $l$, among the strategies of $S$ there is at least one $i \in S$ such that $(A_S\yy^L)_i \ge frac{\sigma(\yy^L)}{2}$. 
For the second part, a row of $B_S^\top$ is a column of $B_S$. Note that every entry in $B_S$ is at least zero, and in a column all entries corresponding to rows in $S$ are one. Let us divide $\yy^R$ further into coordiantes corresponding to set $S$, namely $\yy^{R,S}$, and those outside $S$, namely $\yy^{R,\bS}$. In block $B_S$ the role of first player is that of column-player in game $(A_S,B_S)$. Therefore, strategies $(n+1),\dots,2n$ correspond to the $n={l \choose (l/2)}$ subsets of $S$. There is one such set that correspond to largest $(l/2)$ coordinates of $\yy^{R,S}$. Let this be $S_{i'}$. Then, $(B_S^\top\yy^R)_{i'} \ge \sigma(\yy^{R,\bS}) + \sigma(\yy^{R,S})/2 \ge \sigma(\yy^R)/2$. 
\end{proof}

Consider the $i,i' \le n$ as in the above claim. Since $\sigma(\xx^L),\sigma(\xx^R)>0$, there exists $h,h' \le n$ such that $x_h,x_{(n+h')} >0$. 
Row player's payoffs from strategies $i,(n+i'),h,$ and $(n+h')$ are:
\[
\begin{array}{l}
(R_S\yy)_h = 2\sigma(\yy^L) + (A_S\yy^L)_h - 2 \sigma(\yy^R), \ \ \ (R_S\yy)_{(n+i')} = -2 \sigma(\yy^L) + (B_S^\top\yy^R)_{i'} + 2 \sigma(\yy^R)
(R_S\yy)_i = 2\sigma(\yy^L) + (A_S\yy^L)_i - 2 \sigma(\yy^R), \ \ \ (R_S\yy)_{(n+h')} = -2 \sigma(\yy^L) + (B_S^\top\yy^R)_{h'} + 2 \sigma(\yy^R)
\end{array}
\]

Since $(\xx,\yy)$ is an $\eps$-\WNE we must have $(R_S\yy)_h \ge (R_S\yy)_{(n+i')} - \eps$ and $(R_S\yy)_{(n+h')} \ge (R_S\yy)_i -\eps$. Using Claim \ref{cl:const1}, the former gives,
\[
\begin{array}{lcl}
3\sigma(\yy^L) - 2\sigma(\yy^R) \ge -2\sigma(\yy^L) + \frac{\sigma(\yy^R)}{2}+ 2\sigma(\yy^R) -\eps & \Rightarrow & 5\sigma(\yy^L) \ge \frac{9}{2} \sigma(\yy^R) -\eps\\ 
& \Rightarrow & \sigma(\yy^L) \ge \frac{9}{10}\sigma(\yy^R) -\frac{\eps}{5} = \frac{9}{10}(1-\sigma(\yy^L)) -\frac{\eps}{5}\\
& \Rightarrow & (1+\frac{9}{10}) \sigma(\yy^L) \ge \frac{9}{10} -\frac{\eps}{5}\\
& \Rightarrow & \sigma(\yy^L) \ge \frac{9}{19} - \frac{2}{19}\eps\ge \frac{9}{19} - \frac{\eps}{9}
\end{array}
\]
Similarly, using $(R_S\yy)_{(n+h')} \ge (R_S\yy)_i -\eps$ together with Claim \ref{cl:const1} we will get $\sigma(\yy^R) \ge \frac{9}{10}\sigma(\yy^L) -\frac{\eps}{5}$. Simplifying this using $\sigma(\yy^R) = 1-\sigma(\yy^L)$ gives $\sigma(\yy^L) \le \frac{10}{19}+\frac{\eps}{9}$. 

Bounds on $\sigma(\xx^L)$ and $\sigma(\xx^R)$ can be obtained through similar arguments for the payoff of the column-player w.r.t. $C_S$. 
\end{proof}

For any $\eps<1$ the bounds obtained in Lemma \ref{lem:const-goodgame1} implies lower bound of at least $\frac{1}{3}$ and upper bound of at most $\frac{2}{3}$ on the each of $\sigma(\xx^L), \sigma(\xx^R), \sigma(\yy^L)$, and $\sigma(\yy^R)$.

\begin{lemma}
For an $\eps\in [0,1)$, let $(\xx,\yy)$ be an $\eps$-\WNE of game $(R_S,C_S)$. Then, $(\frac{\xx^L}{\sigma(\xx^L)}, \frac{\yy^L}{\sigma(\yy^L)})$ and $(\frac{\yy^R}{\sigma(\yy^R)}, \frac{\xx^R}{\sigma(\xx^R)})$ are $3\eps$-\WNE of game $(A_S,B_S)$. 
\end{lemma}
\begin{proof}
If $x_i$ for an $i\le n$, then it must be the case that $(R_S\yy)_i \ge (R_S\yy)_k -\eps$ for all $k\le n$. This implies,
\[
(A_S\yy^L)_i \ge (A_S\yy^L)_k - \eps \Rightarrow \frac{(A_S\yy^L)_i}{\sigma(\yy^L)} \ge \frac{(A_S\yy^L)_k}{\sigma(\yy^L)} - \frac{\eps}{\sigma(\yy^L)} \Rightarrow (A_S\frac{\yy^L}{\sigma(\yy^L)})_i \ge (A_S\frac{\yy^L}{\sigma(\yy^L)})_k - 3\eps
\]
The last inequality follows using Lemma \ref{lem:const-goodgame1}. Similarly, we can argue that if $y_j >0$ for a $j \le n$, then for all $k \le n$ we have $(\frac{\xx^{L^\top}}{\sigma(\xx^L)}B_S)_j \ge (\frac{\xx^{L^\top}}{\sigma(\xx^L)}B_S)_k - 3\eps$. These two together implies $(\frac{\xx^L}{\sigma(\xx^L)}, \frac{\yy^L}{\sigma(\yy^L)})$ is a $3\eps$-\WNE of game $(A_S,B_S)$.

In the lower diagonal block, the game is $(B_S^T, A_S^T)$, or in otherwords the roles of the two players are switched. Therefore, it follows that if $x_i>0$ for an $i>n$ then for all $k>n$ we have $(B_S^T\frac{\yy^R}{\sigma(\yy^R)})_i = (\frac{\yy^{R^\top}}{\sigma(\yy^R)}B_S)_i \ge (\frac{\yy^{R^\top}}{\sigma(\yy^R)}B_S)_k - 3\eps$. And similarly, if $y_j>0$ for $j>n$ then for all $k>n$ we have $(A_S\frac{\xx^R}{\sigma(\xx^R)})_j \ge (A_S\frac{\xx^R}{\sigma(\xx^R)})_k - 3\eps$. These two together implies $(\frac{\yy^R}{\sigma(\yy^R)}, \frac{\xx^R}{\sigma(\xx^R)})$ are $3\eps$-\WNE of game $(A_S,B_S)$.
The lemma follows.
\end{proof}

The above lemma together with Theorem \ref{thm:DP} implies that for any $\eps$-\WNE $(\xx,\yy)$, vector $\xx^L$ is near uniform distribution over strategis of $S$ scaled by $\sigma(\xx^L)$. In order to show non-overlapping equilibrium sets across games corresponding to different subsets, we will need that $\xx^L$ is near such a uniform distribution scaled by $\frac{1}{2}$. For this we need a tighter upper-lower bound on $\sigma(\xx^L)$, that we show next.  

\begin{lemma}
If $(\xx,\yy)$ is an $\eps$-\WNE of game $(R_S,C_S)$, then $\forall i \le n,\ (A_S\yy^L)_i \le \frac{\sigma(\yy^L)}{2} +4\eps$ and $(\xx^{L^\top}B_S)_i \le \frac{\sigma(\xx^L)}{2} +4\eps$. And similarly, $(B_S^\top\yy^R)_i\le \frac{\sigma(\yy^L)}{2} +4\eps$ and $(A_S\xx^R)_i \le \frac{\sigma(\xx^R)}+4\eps$ for each $i \in [n]$.
\end{lemma}
\begin{proof}
Let $\txx=\frac{\xx^L}{\sigma(\xx^L)}$ and $\tyy=\frac{\yy^L}{\sigma(\yy^L}$. Lemma \ref{lem:const-goodgame2} implies that $(\txx,\tyy)$ is a $3\eps$-\WNE of game $(A_S,B_S)$. Then due to Theorem \ref{thm:DP} part $(a)$, we have $\tx_i=0$ for all $i\notin S$. Since sum of the payoffs for rows in $S$ is always $1$ in this game, we have $\txx^\top\top (A_S+B_S)\tyy=1$. There are two possible scenarios:

{\bf Case I -} $\txx^\top A_S \tyy \le \frac{1}{2}$. 
Then it must be the case that $\forall i \le n,\ (A_S\tyy)_i \le \frac{1}{2} + 3\eps$, or else $(\txx,\tyy)$ is not a $3\eps$-\WNE of $(A_S,B_S)$. 
Multiplying by $\sigma(\yy^L)$ gives, $(A_S\yy^L)_i \le \frac{\sigma(\yy^L)}{2} + \sigma(\yy^L)3\eps \le \frac{\sigma(\yy^L)}{2} + 2\eps$ for each $i\in [n]$. The last inequality uses $\sigma(\yy^L) \le \frac{2}{3}$ from Lemma \ref{lem:const-goodgame1}. 

To get similar bound on $(\xx^{L^\top}B_S)_i$, note that Claim \ref{clm:const-goodgame1} gives existence of $i \in [n]$ such that $(A_S\tyy)_i \ge \frac{1}{2}$. Therefore $\txx^\top A_S \tyy \ge \frac{1}{2} - 3\eps$, implying $\txx^\top B_S \tyy \le \frac{1}{2} + 3\eps$. Therefore, again $3\eps$-\WNE condition gives that for each $i\in [n]$ we should have $(\txx^\top B_S)_i \le \frac{1}{2} + 6\eps$. Through similar analysis as above we would get that for each $i\in [n]$, $(\xx^{L^\top}B_S)_i \le \frac{\sigma(\xx^L)}{2} + 4\eps$. 

{\bf Case II -} $\txx^\top B_S \tyy \le \frac{1}{2}$. 
Again by similar analysis as Case I, we will get that for each $i \in [n]$ we have $(A_S\yy^L)_i \le \frac{\sigma(\yy^L)} + 4\eps$ and $(\xx^{L^\top}B_S)_i \le \frac{\sigma(\xx^L)}{2} + 2\eps$.

The second part follows similarly using the fact that $(\frac{\yy^R}{\sigma(\yy^R)},\frac{\xx^R}{\sigma(\xx^R)})$ is also a $3\eps$-\WNE of game $(A_S,B_S)$ from Lemma \ref{lem:const-goodgame2}.
\end{proof}

Now we are ready to show that vector $\xx^L$ and $\yy^R$ corresponding to any $\eps$-\WNE are near uniform distribution on set $S$ scaled by $1/2$. 

\begin{lemma}
If $(\xx,\yy)$ is an $\eps$-\WNE of game $(R_S,C_S)$, then $(i)$ $\supp(\xx^L), \supp(\yy^R) \subseteq S$, and $(ii)$ $||\xx^L - \ud{S}/2||_1 \le 17\eps$ and $||\yy^R - \ud{S}/2||_1 \le 17\eps$. 
\end{lemma}
\begin{proof}
From Lemma \ref{lem:const-goodgame2} we have that $(\xx^L/\sigma(\xx^L), \yy^L/\sigma(\yy^L))$ is a $3\eps$-\WNE of game $(A_S,B_S)$. Then part $(a)$ of Theorem \ref{thm:DP} implies $\supp(\xx^L) \subset S$ and $||\xx^L/\sigma(\xx^L) - \ud{S}||_1 \le 24\eps$. Multiplying by $\sigma(\xx^L)$ gives $||\xx^L - \sigma(\xx^L)\ud{S}||_1 \le \sigma(\xx^L) 24\eps \Rightarrow ||\xx^L - \ud{S}/2||_1 -\eps \le 16\eps \Rightarrow ||\xx^L - \ud{S}/2||_1 \le 17\eps$.

Similarly, using $(\yy^R/\sigma(\yy^R), \xx^R/\sigma(\xx^R))$ being a $3\eps$-\WNE of game $(A_S,B_S)$ from Lemma \ref{lem:const-goodgame2}, together with part $(a)$ of Theorem \ref{tm:DP}, we can show that $\supp(\yy^R)\subseteq S$ and $||\yy^R -\ud{S}/2||_1 \le 17\eps$.
\end{proof}

\begin{lemma}
Given an $\eps\in [0,1)$, if $(\xx,\yy)$ is an $\eps$-\WNE of game $(R_S,C_S)$ then $\frac{1}{2} - \eps \le \sigma(\xx^L), \sigma(\xx^R),\sigma(\yy^L),\sigma(\yy^R) \le \frac{1}{2} +\eps$. 
\end{lemma}
\begin{proof}
The proof follows similar argument as of the proof of Lemma \ref{lem:const-goodgame1}. 
We will first show the claim for $\sigma(\yy^L)$ and thereby it will follow for $\sigma(\yy^R)$ as well since $\yy^R=1-\yy^L$. Let $i,i'\in [n]$ be the indices from Claim \ref{clm:const-goodgame1}. Let $h,h'\in [n]$ be such that $x_h,x_{(n+h')}>0$. Then, $(R_S\yy)_h \ge (R_S\yy)_{(n+i')} -\eps$ gives
\[
2\sigma(\yy^L) + (A_S\yy^L)_i - 2\sigma(\yy^R) \ge -2\sigma(\yy^L) +(B_S^\top\yy^R)_{i'}+ 2\sigma(\yy^R) -\eps \Rightarrow 4\sigma(\yy^L) + \frac{\sigma(\yy^L)}{2} +\eps \ge 2\sigma(\yy^R) + \frac{\sigma(\yy^R)}{2} -\eps
\]
The last inequality uses $(A_S\yy^L)_i \le \frac{\sigma(\yy^L)}{2} + 4\eps$ from Lemma \ref{lem:cost-goodgame3}. 
Simplifying the above gives $\sigma(\yy^L) \ge \sigma(\yy^R) -2\eps \Rightarrow \sigma(\yy^L) \ge \frac{1}{2} - \eps$. Similarly, simpliying $(R_S\yy)_{(n+h')} \ge (R_S\yy)_i -\eps$ by making use of $(A_S\yy^L)_i\ge \frac{\sigma(\yy^L)}{2}$ from Claim \ref{clm:const-goodgame1} and $(B_S^\top \yy^R)\le \frac{\sigma(\yy^R)}{2} +4\eps$ from Lemma \ref{lem:const-goodgame3}, we get $\sigma(\yy^L) \le \frac{1}{2} +\eps$. 

Bounds for $\sigma(\xx^L),\sigma(\xx^R)$ follows using similar argument for the payoffs of the column player. 
\end{proof}


\begin{lemma}
For an $\eps \in [0,1)$ and $c>1$, if two strategies $\xx$ and $\txx$ of the row-player are such that $\frac{1}{2} - \frac{\eps}{9} \le \sigma(\xx^L) \le \frac{1}{2} +\frac{\eps}{9}$, and $||\xx^L - \txx^L||_1 \ge c\eps$, then $||\xx - \txx||_1 \ge (c-1) \eps$. 
\end{lemma}






extend their construction to ensure that both player's NE sets are far apart across games. Let $l$ be an even integer and $n = \choose{l}{l/2}$. For each $S\subset [n]$ of size $l$, we will construct a $2n \times 2n$ game. If we think of this game as $2 \times 2$ block game where each block is of size $n \times n$, then it is a combination of block matching pennies game and two games of \cite{DP} in the block-diagonal. That is, 

to ensure that strategies




















%#######################################################################################################
%#######################################################################################################
%#######################################################################################################
%#######################################################################################################




\begin{comment}

We prove Theorem \ref{thm:approx-nash-hardness-technical} in the following two steps. 
% \begin{lemma} \label{lem:free-game-reduction}
% Let $\cI$ be a 3SAT instance with $n$ variables and $\Theta(n)$ constraints. There's a transformation of $\cI$ into a two-player game $(A,B)$ with $m = 2^{O(\sqrt{n})}$ pure strategies and a constant $\epsilon$ with the following properties:
% \begin{enumerate}
% 	\item If there exists a pseudo-distribution of degree $\Theta(n)$ satisfying the 3SAT constraints in $\cI$ and $\{x_i^2 = x_i\}$ for $1 \leq i \leq n$, then there exists a pseudo-distribution satisfying the constraints of $\NE$ formulation \eqref{eq:NEchar} for the game $(A,B)$, of degree $\Theta(\sqrt{n})$ and total payoff 1.
% 	\item If every assignment to the variables $x$ satisfies at most $7/8+\gamma$-fraction of the constraints in $\cI$ then every $\epsilon$-$\NE$ of $(A,B)$ has total payoff at most $2(1-\epsilon).$
% \end{enumerate}
The first step is a hardness of approximating social welfare (any ``quality'' measure of equilibria would have worked for us here.)

\begin{lemma} \label{lem:reduction}
There exists a game $(A,B)$ with $n$ pure strategies with all payoffs between $[-1,1]$ and a constant $\epsilon > 0$ satisfying:
\begin{enumerate}
\item \textbf{Completeness: } There exists a pseudo-distribution of degree $\Theta(\log{(n)})$ satisfying the constraints of the $\NE$-formulation for the game $(A,B)$ and sum of the payoffs of the players equalling $2$.
\item \textbf{Soundness:} The sum of the payoffs of the players at any $\epsilon$-equilibrium is at most $2(1-\epsilon).$
\end{enumerate}
\end{lemma}
% \begin{itemize}
% \item If the graph $G$ has planted $k=\chat \log{n}$ clique, then game $(R,C)$ has an equilibrium $(x,y)$ where for each $i\in [n]$ corresponding to a vertex in the clique $x_i=y_i=1/k$, with probability $\frac{1}{n^2}$. Both players get payoff one at this equilibrium.
% \item Given an $\epshat$-$\NE$ $(\xx,\yy)$ of game $(R,C)$ with total payoff at least $2(1-\epshat)$ we can find the planted $\chat\log{n}$-clique in graph $G$ with high probability. \Rnote{Do we need exact probability value? From their proof it seems to be (1 - inverse poly).} % has a planted clique of size $k=\chat \log{n}$.
% \end{itemize}



The second lemma is a tool that gives a construction of an exponentially large family of two-player games with $n$ strategies such that any pair of equilibria of any two games in the family are far apart. 
\begin{lemma} \label{lem:very-different-games}
There exists a family of games $G_1, G_2, \ldots, G_N$ with $n$ pure strategies, $N = 2^{\Theta(n)}$, and all payoffs between $[-1,1]$ such that if $(\xx^i,\yy^i)$ and $(\xx^j,\yy^j)$ are $\Theta(1/n)$-approximate equilibria of $G_i$ and $G_j$ respectively for $i \neq j$, then $\norm{\xx^i-\xx^j}_1, \norm{\yy^i-\yy^j}_1> \FIXME$
\end{lemma}

The final ingredient in the proof of Theorem \ref{thm:approx-nash-hardness-technical} is a way to combine the exponentially large family of games from Lemma \ref{lem:very-different-games} with the game $G$ from Lemma \ref{lem:reduction}.

\begin{lemma}[Combining Hard Games] \label{lem:combining-dummy-game-with-reduction}
Let $G_1$ be an $n$-strategy game such that any $\epsilon$-equilibrium achieves a total payoff of at most $2(1-\epsilon).$ Let $G_2$ be an $m$-strategy game such that all $\epsilon$-WNE \FIXME equilibria in $G_2$ have payoffs at least \FIXME $1-\epsilon$. 

Then, there exists a $m+n$ strategy game $G$ such that for any $(\xx,\yy)$ that forms an $\epsilon$-WNE of $G$, there's an $\epsilon$-WNE $(\xx',\yy')$ of $G_2$ such that the strategy profile $(\xx'',\yy'')$ for $G$ obtained by adding $0$s in the first $n$ coordinates and using $(\xx',\yy')$ in the last $m$ coordinates satisfies: $\norm{\xx''-\xx}_1, \norm{\yy''-\yy}_1 \leq \FIXME$
\end{lemma}
\Pnote{clean up and fix the statement of this lemma depending on what exactly is required of the game $G_2$}

We can easily complete the proof of Theorem \ref{thm:approx-nash-hardness-technical} using the three lemmas above.

\begin{proof}[Proof of Theorem \ref{thm:approx-nash-hardness-technical}]

\end{proof}

In the following two subsections, we prove Lemmas \ref{lem:very-different-games} and \ref{lem:combining-dummy-game-with-reduction} respectively. 

\subsection{Proof of Lemma \ref{lem:very-different-games}}


\subsection{Proof of Lemma \ref{lem:combining-dummy-game-with-reduction}}



\subsection{Planted Clique to Constant Approximation}
In this section we will reduce the problem of finding a planted clique of size $c\log{n}$ in a random graph $G(n,1/2)$ to finding a non-trivial constant approximate Nash equilibrium. We will first show results for a stronger notion of approximation described next, and then relate it to $\eps$-NE. 
A strategy profile $(x,y)$ is an $\epsilon$-approximate well-supported Nash equilibrium (written as $\epsilon$-\WNE) iff \[\mbox{for every } i \leq n,\ x_i > 0 \Rightarrow \max_k e_k^{\top} A y -\epsilon \leq e_i^{\top} A y \ \ \ \mbox{ and } \ \ \ y_i>0 \Rightarrow \max_k x^{\top} B e_k-\epsilon \leq x^{\top} B y.\]

Strategies giving maximum payoff to a player are called her best response, and those giving at least maximum payoff minus $\eps$ payoff $\eps$-best response, i.e. $\BR_1(\yy) = \{i\le n\ |\  e_i^{\top} A y = \max_k e_k^{\top} A y\}$ and $\eps-\BR_1(\yy) = \{ i \le n\ |\ x^{\top} A e_i \ge \max_k x^{\top} A e_k-\eps\}$, and similarly $\BR_2(\xx)$ and $\eps-\BR_2(\xx)$ can be defined. Let us denote support of a probability vector $\vv$ by $\Supp(\vv) = \{i\ |\ v_i>0\}$. 
Note that by definition, $(\xx,\yy)$ is an $\eps$-\WNE iff $\Supp(\xx) \subseteq \eps-\BR_1(\yy)$ and $\Supp(\yy) \subseteq\eps-\BR_2(\xx)$. 

\begin{lemma}\label{lem:ne-prop}
\begin{enumerate}
\item If $(x,y)$ is an NE iff $\Supp(\xx) \subseteq \BR_1(\yy)  \ \ \ \mbox{ and } \ \ \ \Supp(\yy) \subseteq \BR_2(\xx)$.
\item Every $\eps$-\WNE is $\eps$-$\NE$.
\item If $(\xx,\yy)$ is an $\eps$-$\NE$ then $\sum_{i \notin \sqrt{\eps}-\BR_1(\yy)} x_i \le \sqrt{\eps}$ and $\sum_{i \notin \sqrt{\eps}-\BR_2(\xx)} y_i \le \sqrt{\eps}$. 
\item Given $\eps$-$\NE$ $(\xx,\yy)$ we can construct $3\sqrt{\eps}$-\WNE $(\xx',\yy')$ such that $\Supp(\xx') \subseteq \sqrt{\eps}-\BR_1(\yy)$ and $\Supp(\yy') \subseteq \sqrt{\eps}-\BR_2(\xx)$. 
\end{enumerate}
\end{lemma}
\begin{proof}
Proofs of first and second part follows by definition. The third and fourth part essentially follows from the proof of Lemma 2.2 of \cite{CDT} due to Chen, Deng, and Teng.
\end{proof}

Now we are ready to state our construction which is a modification of the construction by Hazan and Krauthgamer \cite{}. Their construction and guarantees are as follows.

{\bf Hazan Krauthgamer Construction.} 
Given an instance $G(n,1/2)$, we want to check if it has a clique of size $k=\chat\log{n}$. 
It will be reduced to checking existence of $\epshat$-$\NE$ where both players get payoff at least $(1-\epshat)$. 
Define the following parameters: $M=12$, $c_2=200$, $c_1=2+c_2\log(4M/3)$, $\chat = 32M^2(c_1+2)$, and $\epshat = 1/50M$.
Consider the two-player game defined by the following payoff matrices (for the row-player and the column player, respectively):
\begin{equation}\label{eq:HK}
R=\left[\begin{array}{cc}A & -B^T \\  B & \zeros \end{array}\right]\ \ \ \ \ C=\left[\begin{array}{cc}A & B^T \\  -B & \zeros \end{array}\right]
\end{equation}

The matrices $R,C$ are of size $N\times N$ for $N = n^{c_1}$. These
matrices are constructed from the following blocks: $(i)$ The upper left $n\times n$ block in both $R,C$ is the adjacency matrix of $G$ with self loops added.
$(ii)$ The lower right block $\zeros$ in both $R,C$ is the all zeros
matrix of size $(N-n)\times (N-n)$ $(iii)$ All other entries are set via an $(N-n)\times n$ matrix
$B$ whose entries are set independently at random to be
\[
B(i,j) = \left\{\begin{array}{ll} M & \mbox{with probability } \frac{3}{4M}\\
0 & \mbox{otherwise} \end{array}\right.
\]



We modify the construction by adding one extra strategy to both players: 
\[
R' = \left[\begin{array}{cc} \ R \ & -\ones \\ \ones & 1 \end{array}\right] \ \ \ \ \ 
C' = \left[\begin{array}{cc} \ C \ & \ones \\ -\ones & 1\end{array}\right]
\]


\begin{lemma}
\begin{itemize}
\item If the graph has planted $k=\chat \log{n}$ clique, then game $(R',C')$ has an equilibrium $(x,y)$ where for each $i\in [n]$ corresponding to a vertex in the clique $x_i=y_i=1/k$, with probability $\frac{1}{n^2}$. Both players get payoff one at this equilibrium.
\item If graph $G$ does not have a clique of size $k \chat \log{n}$ then for an $\epshat$-equilibrium $(x,y)$ we have $||x-e_{(N+1)}||_\infty \le \frac{\epshat}{2}$ and $||y - e_{(N+1)}||_\infty \le \frac{\epshat}{2}$ with high probability. 
\end{itemize}
\end{lemma}
\begin{proof}
For simplicity let us denote the last strategy $(N+1)$ by $m$. 
First part of the lemma follows from the first part of Lemma \ref{lem:HK} since the payoff from strategy $m$ is at most $1$.  

For the second part, first note that if $\yy= \ee_m$ then $\xx=\ee_m$ and vice-versa. Therefore, to the contrary suppose $x_m<1$ and $y_m<1$. 
Divide vectors $\xx$ and $\yy$ into two parts, one corresponding to $R,C$ and second corresponding to strategy $m$, i.e., let $\xx=(\xx', x_m)$ and $\yy=(\yy', y_m)$. Normalize $\xx'$ and $\yy'$ to get $\hxx$ and $\hyy$ respectively. Since, payoffs in the last column of $R'$ and last row of $C'$ are the same, namely $-1$, $(\hxx,\hyy)$ is an $\epshat$-equilibrium of $(R,C)$. Therefore, by second part of Lemma \ref{lem:HK} we have that with high probability either $\hxx^T (R+C) \hyy < 2(1-\epshat)$ 

Note that $\hxx =\frac{\xx'}{(1-x_m)}$ and similarly $\hyy = \frac{\yy'}{(1-y_m)}$. Payoff of the row player in game $R',C'$ from $(\xx,\yy)$ is:

$\xx^T R' \yy = \xx' R \yy'  - y_m (1-x_m) + x_m = (\hxx^T R \hyy) (1-x_m)(1-y_m) - y_m (1-x_m) + x_m. %< (1-\epshat) (1-x_m)(1-y_m) - y_m (1-x_m) + x_m
$
Similarly, payoff of the column player is:
$
\xx^T C' \yy = \xx' C \yy'  - x_m (1-y_m) + y_m = (\hxx^T C \hyy) (1-y_m)(1-x_m) - x_m (1-y_m) + y_m. %< (1-\epshat) (1-x_m)(1-y_m) - x_m (1-y_m) + y_m
$

Since strategy $m$ gives payoff $1$ to both the players no matter what the other player is playing, payoff of both players at any $\epshat$-equilibrium is at least $(1-\epshat)$. Imposing this lower bound on the above expressions of payoffs and summing them up gives,

\[
2(1-\epshat) \le \xx^T(R' + C') \yy =  (\hxx^T R+C \hyy) (1-x_m)(1-y_m) - y_m (1-x_m) - x_m (1-y_m) + x_m + y_m < 2(1-\epshat) (1-x_m)(1-y_m) - y_m (1-x_m) - x_m (1-y_m) + x_m + y_m.
\]

Simplifying, 

\[
\begin{array}{clcl}
& 2 -2\epshat & < &  (2-2\epshat) (1-x_m - y_m + x_my_m) - y_m + x_m y_m - x_m + x_m y_m + x_m + y_m \\
& & = & 2 - 2\epshat - (2 - 2\epshat)(x_m+y_m) + (2 - 2\epshat) x_m y_m +2 x_m y_m \\
\Rightarrow & (2 - 2\epshat) (x_m+ y_m) & < & (4- 2\epshat) x_m y_m 
\end{array}
\]

Let us first focus on getting a lower bound for $y_m$. Above inequality gives: $y_m [(4-2\epshat)x_m - (2-2\epshat)] > (2-2\epshat) x_m$. Note that RHS is always non-negative, while LHS is non-negative only if $x_m \ge (2-2\epshat)/(4-2\epshat)$. Call this lower bound $x_{lb}$. The lower bound on $y_m$ as a function of $x_m$ is 
\[
y_m > \frac{(2-2\epshat) x_m}{(4-2\epshat)x_m - (2-2\epshat)}
\]

RHS in the above expression as a function of $x_m$ is strictly decreasing within range $[x_{lb}, 1]$. Therefore, its minimum value is achieved at $x_m=1$ which is 
\[
y_m > \frac{(2-2\epshat)}{(4-2\epshat) - (2-2\epshat)} = \frac{2(1-\epshat)}{2} = 1-\frac{\epshat}{2}
\]

The same lower-bound can be derived for $x_m$ through similar argument. This directly implies that all other coordinates of vectors $\yy$ and $\xx$ are at most $\frac{\epshat}{2}$, proving the lemma. 
\end{proof}

\subsection{Lower bound against (SoS + enumeration)}
In this section we obtain lower bound against any method that allows checking if a pair of strategies gives NE for a set of pairs based on the solution from SoS relaxation. For this we will combine the construction from the previous section with the Daskalakis and Papadimitriou \cite{DP} construction.

{\bf Daskalakis and Papadimitriou \cite{} Construction.} Let $l$ be an integer such that ${l \choose l/2} \ge N$. Denote ${l \choose l/2}$ by $K$ and fix a subset $S\subset [K]$ of size $l$. We will construct a two-player game $G_S=(\Rdp,\Cdp)$ with $K\times K$ payoff matrices. Let $S_1,\dots,S_K$ be $l/2$ sized subsets of set $S$. We will think of column $j$ of payoff matrices to be associated with set $S_j$. For every $j \in [K]$, fill $j^{th}$ column of $\Rdp$ and $\Cdp$ as follows: $(i)$ For all $i \notin S$ set $\Rdp(i,j) = -4$ and $\Cdp(i,j)=4$. $(ii)$ For all $i \in S_j$ set $\Rdp(i,j) = 4$ and $\Cdp(i,j) =0$. $(iii)$ For all $i \in S\setminus S_j$ set $\Rdp(i,j)=0$ and $\Cdp(i,j)=4$. 

\begin{lemma}{Daskalakis and Papadimitriou \cite{DP}}\label{lem:DP}
Let $\eps<1$. If $(\xx,\yy)$ is an $\eps$-\WNE of game $G_S$, then following are satisfied,
\begin{enumerate}
\item For all $i\notin S$, $x_i=0$.
\item $||\xx - u_S||_1 \le 2\eps$, where $u_S$ is the uniform distribution over $S$.
\end{enumerate}
\end{lemma}


{\bf Our Construction.} Given a random graph $G(n,1/2)$ construct game $(R,C)$ of dimension $N \times N$ as per \ref{eq:HK}. As above let $K={l \choose l/2} \ge N$ for an integer $l$. For each subset $S\subset [K]$ of size $l/2$ construct game $G_S=(\Rdp,\Cdp)$ as above. Using these two, construct the following game with $(N+K) \times (N+K)$ payoff matrices. 
\begin{equation}\label{eq:our2}
R'_S = \begin{array}{cc} R \ & \ -O^T \\ O \ &\ \Rdp \end{array}\ \ \ \mbox{ and } C'_S = \begin{array}{cc} C \ & \ O^T \\ -O \ & \ \Cdp \end{array}
\end{equation}

\begin{lemma}\label{lem:constApprox-enum1}
If graph $G$ does not have a clique of size $k=\chat \log{n}$ then for an $0\le \eps \le \epshat$ any $\eps$-\WNE $(\xx,\yy)$ of game $(R'_S, C'_S)$, we have $x_i=y_i=0$ for each $i\in[N]$ and the truncated strategy pair $((x_{(N+1)},\dots,x_{(N+K)}), (y_{(N+1)},\dots,y_{(N+K)})$ is an $\eps$-\WNE of game $(\Rdp, \Cdp)$. 
\end{lemma}
\begin{proof}
If $\Supp(\xx), \Supp(\yy) \subseteq\{N+1, \dots, N+K\}$ then the lemma follows by definition of $\eps$-\WNE. Next we show that $\Supp(\xx), \Supp(\yy) \subseteq\{N+1, \dots, N+K\}$. Let $x_L=\sum_{i\in[N]} x_i$, $x_R=1-X_L$, $y_L=\sum_{i\in [N]} y_i$, and $y_R=1-Y_L$. 

To the contrary suppose $x_L>0$ then $y_L>0$ as well. Otherwise payoff of the first player form any strategy $i\in[N]$ is $-1$. While for any $j \in S$ strategy $(N+j)$ gives her at least zero-payoff. This contradicts $\Supp(\xx) \subseteq \eps-\BR_1(\yy)$. 

Let $\hxx= (x_1,\dots,x_N)$ and $\hyy=(y_1,\dots,y_N)$. Since graph $G$ has no clique of size $\chat\log{n}$, Lemma \ref{lem:HK} implies that with high probability either $\hxx^{\top}R \hyy< (1-\epshat) x_L y_L$ or $\hxx^{\top}C\hyy< (1-\epshat) x_L y_L$. 
\medskip

{\bf Case I: $\hxx^{\top}R \hyy< (1-\epshat) x_L y_L$}\\
There exists $i\in [N]$ such that $x_i>0$ and $(R\hyy)_i < (1-\epshat) y_L$. Therefore, $(R'_S\yy)_i = (R\hyy)_i - y_R < (1-\epshat)y_L - y_R$. 

\begin{claim}\label{clm1}
$\exists j \in S$ such that $(R'_S\yy)_{(N+j)}\ge y_L + 2y_R$.
\end{claim}
\begin{proof}
Let $\yy' = (y_{(N+1)},\dots,y_{(N+K)})$, then by construction of $R'_S$, we have $(R'_S\yy)_{(N+j)} = y_L + (R\yy')_j$. 
Recall that $|S|$ is $l$ and columns of $\Rdp$ are indexed by $l/2$ sized subsets of set $S$, namely $S_1,\dots,S_K$. 
For each $j \in S$, define $T_j=\{t \in [K]\ |\ j \in S_t\}$. By construction we have $\Rdp(j,t)=4,\ \forall t\in T\}$. Therefore it suffices to show that there exists $j \in [K]$ with $\sum_{t \in T_j} y'_t \ge \frac{y_R}{2}$. For simplicity, let us denote $\sum_{t \in T_j}$ by $\delta_j$. Since each $S_t$ contains $l/2$ elements of $S$, we get $\sum_{j\in S} \delta_j = l/2 \sum_{t\in[K]} y'(S_t) = \frac{l}{2} y_R$. Since $|S|=l$, there has to exist $j$ with $\delta_j \ge y_R/2$. 
\end{proof}

For $j\in S$ that satisfies Claim \ref{clm1}, we have $(R'_S\yy)_{(N+j)} \ge y_L + 2 y_R = y_L+2y_R$. By requirement of $\eps$-\WNE, payoff from strategy $i$ above should be at least payoff from $(N+j)$ minus $\eps$. This gives,
\[
(1-\epshat) y_L - y_R > y_L+2y_R - \eps \ge y_L+2y_R - \epshat \Rightarrow (1-y_L) \epshat - y_R > 2y_R \Rightarrow (\epshat-1)y_R > 2y_R. 
\]
A contradiction.
\medskip


{\bf Case II: $\hxx^{\top}C \hyy< (1-\epshat) x_L y_L$}\\
Again there exists $i\in [N]$ such that $y_i>0$ and $(\hxx^{\top}C)_i < (1-\epshat) x_L$. Therefore, $(\xx^{\top} C'_S)_i = (\hxx^{\top}C)_i  - x_R < (1-\epshat)x_L - x_R$. 

Similar to the previous case we will show that there is a strategy $i >N$ that give much better payoff, and thereby lead to a contradiction. Let $x_{R1} = \sum_{j \in S} x_{N+j}$ and $x_{R2}=x_R - x_{R1}$. Among the row player's strategies corresponding to $S$ consider those $l/2$ whose total probability is at least $\xx_{R1}/2$. Denote this set by $W$. By construction there exists a subset $S_t\subset S$ of size $l/2$ such that $S_t=W$. Then, column player's payoff from the strategy corresponding to $S_t$ is $(\xx^{\top} C'_S)_{(N+t)} \ge x_L + 4 x_{R1} + 2 x_{R2} \ge x_L + 2 x_R$. 
Similar to the previous case, $\eps$-\WNE imposes $(\xx^{\top} C'_S)_i \ge (\xx^{\top} C'_S)_{(N+t)} - \eps \Rightarrow (1-\epshat)x_L - x_R > x_L + 2 x_R -\eps$. By the same argument as above it leads to a contradiction. 
\end{proof}

\begin{lemma}
If $(\xx,\yy)$ is an $\eps^2$-$\NE$ of game $(R'_S,C'_S)$ then $||\xx - u_S||_1 \le 8\eps$, where $u_S$ is an $(N+K)$-dimensional vector whose first $N$ coordinates are zero and last $k$ co-ordinates constitutes uniform distribution over set $S$. 
\end{lemma}
\begin{proof}
By Lemma~\ref{lem:ne-prop}(4) there exists $(\xx',\yy')$ that is $3\eps$-\WNE of game $(R'_S,C'_S)$, and in addition $\Supp(\xx') \subseteq \eps$-$\BR_1(\yy)$ 
and $\Supp(\yy') \subseteq \eps$-$\BR_2(\xx)$. Part $(3)$ of Lemma \ref{lem:ne-prop} implies $\sum_{i\notin \eBR_1(\yy)} x_i \le \eps$ and $\sum_{i\notin\eBR_2(\xx)} y_i \le \eps$. In the construction of $\xx'$ from $\xx$ we set the probability of all strategies not in $\eBR_1(\yy)$ to zero and redistribute their mass to strategies in $\eBR_1(\yy)$ uniformly. Therefore, $||\xx - \xx'||_1 \le 2\eps$. Lemma \ref{lem:constApprox-enum1} together with Lemma \ref{lem:DP} implies that $||\xx' - u_S|| \le 6 \eps$ (assuming $3\eps <\epshat$). Thus, $||\xx - u_S||_1 \le ||\xx - \xx'||_1 + ||\xx' - u_S||_1 \le 8\eps$. 
\end{proof}
\end{comment}


==> content/notes.tex <==
%!TEX root=../main.tex
% \section{Preliminaries and Notation}
% We denote the simplex in $n$ dimensions by $\Delta_n = \{x \in \R^n \mid x_i \geq 0 \text{ for every } i \text{ and } \sum_{i = 1}^n x_i = 1\}.$
% \section{Correlated Equilibrium Formulation}
% We state the problem of computing correlated equilibria in general two player games.
% The input is a pair of payoff matrices $A, B \in \R^{n \times n}$ (for players Alice and Bob respectively) where to avoid notational clutter, we assume that the two players have the same number of pure strategies. $A$ and $B$ are assumed to normalized so that every entry of the two matrices is in $[0,1].$

% \begin{definition}[Correlated Equilibrium]
% A correlated equilibrium in a two player games with payoff matrices $A$ and $B$ is a distribution $p$ on ordered pairs of strategies $(i,j)$ for $1 \leq i , j \leq n$ such that the following complementary slackness conditions hold:
% \begin{enumerate}
% \item For every $i \in [n]$, $\sum_{j} A_{i,j} p_{i,j} \geq \sum_{j} A_{i',j} p_{i,j}$ for every $i' \in [n].$
% \item For every $j \in [n]$, $\sum_{i} B_{i,j} p_{i,j} \geq \sum_{i} B_{i,j'} p_{i,j}$ for every $j' \in [n].$
% \end{enumerate}
% \end{definition} 

% A correlated equilibrium is a Nash equilibrium in the usual sense, if $p = ab^{\top}$ for probability distributions $a,b\in \Delta_n.$ 

% Correlated equilibria have a nice interpretation as follows: Imagine that there's a neutral third-party overseer that advises the two players on their strategies! Then, the overseer can force equilibrium by choosing a pair of strategies $(i,j)$ according to $p_{i,j}$ and sending advice $i$ to Alice and $j$ to Bob. The complementary slackness conditions above then say that no party has a (strict) incentive to deviate from the advised strategy.

% The usefulness of the concept of correlated equilibrium is due to the fact that it can be efficiently computed using linear programming as is evident from the definition itself. 

% The central question we now have is the following, stated in the language of correlated equilibrium.

% \begin{question}
% Suppose there's a set of possible advice that the overseer can give (say $[N]$, typically exponentially large in $n$)). Suppose there's a map from $[N]$ into a Nash equilibrium $a_ib_i^{\top}$. Suppose further, that following kind of distribution $\cD$  describes a correlated equilibrium for the bi-matrix game $(A,B)$: Choose $i \sim \cD$, output $a_i$ and $b_i$ as the probability distributions over  pure strategies for Alice and Bob respectively. 

% For every distribution $\cD$ on $[N]$ as above, is there an event $E$ with probability $\ll 2^{-n}$ such that conditioning $\cD$ on $E$ yields a distribution $\cD'$ such that $\E_{i \sim \cD'} a_i b_i^{\top} \approx ab^{\top}$ for $a,b \in \Delta_n$ and the notion of approximation relevant to satisfying both of types of the complementary slackness conditions in the definnition above? 

% \end{question}


% \section{Nash Equilibrium (NE) Formulations}
% Given a two player game, where both the players have $n$ actions to choose from, it can be represented by two $n\times n$ matrices $(A,B)$. Following is a NE characterization of such games:

% Strategy profile $(x,y)$ where $x,y\in \Delta_n$ is a NE of $(A,B)$ iff
% \begin{equation}\label{eq:NEchar}
% \begin{array}{llcl}
% \forall i\le n, & x_i >0 &\Rightarrow &(Ay)_i = \max_k (Ay)_k\\
% \forall j\le n, & y_i >0 &\Rightarrow &(x^TB)_j = \max_k (x^TB)_k\\
% \end{array}
% \end{equation}

% If the game is symmetric then, $B=A^T$. And a symmetric profile $(x,x)$ is a NE iff
% \begin{equation}\label{eq:SNEchar}
% \begin{array}{llcl}
% \forall i\le n, & x_i >0 &\Rightarrow &(Ax)_i = \max_k (Ax)_k\\
% \end{array}
% \end{equation}

% From (\ref{eq:NEchar}) we can derive following quadratic formulation that captures NE exactly, where $\pi_1$ and $\pi_2$ capture the maximum payoff of players one and two respectively.

% \begin{equation}\label{eq:NEQP}
% \begin{array}{rl}
% \max: & x^T(A+B)y - \pi_1 - \pi_2 \\
% s.t. & (Ay)_i \le \pi_1,\ \ \ \forall i\le n \\
% & (x^TB)_j \le \pi_2,\ \ \ \forall j \le n \\
% & \sum_i x_i =1,\ \ \ \sum_j y_j =1 \\
% & x\ge 0,\ \ \ y\ge 0
% \end{array}
% \end{equation}

% Similarly, for symmetric NE we can write the following formulation:
% \begin{equation}\label{eq:SNEQP}
% \begin{array}{rl}
% \max: & x^TAy - \pi\\
% s.t. & (Ax)_i \le \pi,\ \ \ \forall i\le n \\
% & \sum_i x_i =1;\ \ \ \ \ x\ge 0;
% \end{array}
% \end{equation}

% A joint distribution $P=[P_{ij]}]_{i,j\le n}$ is a correlated equilibrium iff
% \begin{equation}\label{eq:CE}
% \forall i\le n,\ \ \  \ \sum_j A_{ij} P_{ij} \ge \sum_j A_{i'j} P_{ij} \\
% \forall i\le n,\ \ \ \ \ \sum_j B_{ij} P_{ij} \ge \sum_j B_{ij'} P_{ij} \\
% \end{equation}

% It is well known that correlated equilibrium matrices $P$ with rank-1 are exactly the NE.
% \medskip

% \subsection{Polymatrix Game} This is an $k$ player game with an underlying interaction graph $G=(V,E)$ representing which player plays with who all in a two-player game like interaction. Here $V$ is the set of $k$ players, and if $(u,v)\in V$ then players $u$ and $v$ are playing game $(A_{uv}, A_{vu})$ with each other. For now let us assume that each player has $2$ strategies, then $A_{uv}$ and $A_{vu}$ for all $(u,v)\in E$ are $2 \times 2$ matrices. 

% Let $A$ be a block matrix with $2k \times 2k$ dimension, where $(u,v)^{th}$ block has matrix $A_{uv}$ and $(v,u)^{th}$ block is matrix $A_{vu}^T$. NE in this game can be captured via the following quadratic formulation:
% \begin{equation}\label{eq:PMQP}
% \begin{array}{ll}
% \max:& x^TAx - \sum_{u \in V} \pi_u \\
% s.t. & \forall u\le n, (Ax)_{2u-1} \le \pi_u;\ \ \ (Ax)_{2u} \le \pi_u \\
% & \forall u\le n,\ \ \ \ x_{2u-1} + x_{2u}=1 \\
% & x\ge 0
% \end{array}
% \end{equation}


% A slightly different formulation:

% \begin{equation}\label{eq:PMQP-feasibility}
% \begin{array}{ll}
% %\max:& x^TAx - \sum_{u \in V} \pi_u \\
% & \forall u\le n, (Ax)_{2u-1} \le \pi_u;\ \ \ (Ax)_{2u} \le \pi_u \\
% & \forall u\le n,\ \ \ \ x_{2u-1} + x_{2u}=1 \\
% & \forall u \le n, \ \ \  (Ax)_{2u-1} x_{2u-1} +(Ax)_{2u} x_{2u}  = \pi_u\\
% & x\ge 0
% \end{array}
% \end{equation}

% \noindent{\bf Net-Coordination Game.}
% If every edge is a coordination game, {\em i.e.,} $A_{uv}=A_{vu}$ then it is called net-coordination game. Such a game always has a pure equilibrium, and finding one is PLS-complete. The hardness result is by reduction from {\em local max-cut}, where the problem is to find a cut in the graph which can not be improved by moving exactly one vertex from one partition to another. 

% The reduction is as follows: Let $G=(V,E)$ be the input graph of local max-cut problem with weight $w_{uv}$ on edge $(u,v)\in E$. Every vertex is a player, each with two strategies $0$ and $1$. Think of the two strategies as two partitions. Then, every edge $(u,v) \in E$ is a game where ($u$ as first player and $v$ as second player) matrices are $A_{uv}=A_{vu} = \left[\begin{array}{cc} 0 & w_{uv}\\ w_{uv} & 0 \end{array}\right]$.

% Let us assume that $w_{uv}\in[0,\ 1]$. Since this is a potential game, where sum of the utilities of all the agents is the potential function, finding $\epsilon$-approximate equilibrium can be done in $O(n^2/\epsilon)$ time just by best-response dynamics. This is because potential is bounded above by $n^2$, and in every step it increases by at least $\epsilon$ when we are not an approximate equilibrium. 



% \subsection{Approximation}
% Given a two player game, let us assume (wlog) that $(A,B)\in [0,\ 1]$. Profile $(x,y)$ is an $\epsilon$-approximate NE iff
% \[
% x^Ay \ge x'^TAy - \epsilon,\ \forall x'\in \Delta_n;\ \ \ \ x^TBy \ge x^TBy' - \epsilon,\ \ \forall y'\in \Delta_n
% \]

% An $\epsilon$-approximate {\em well-supported} NE for given $\epsilon>0$ is $(x,y)$, s.t.
% \begin{equation}
% \label{eq:ANEchar}
% \begin{array}{llcl}
% \forall i\le n, & x_i >0 &\Rightarrow &(Ay)_i \ge \max_k (Ay)_k - \epsilon\\
% \forall j\le n, & y_i >0 &\Rightarrow &(x^TB)_j = \max_k (x^TB)_k - \epsilon\\
% \end{array}
% \end{equation}

% Similarly, we can define approximate symmetric NE in symmetric game, and approximate NE in polymatrix game. 


% \begin{theorem}[ChenDengTeng'06]
% End of Line PPAD problem with size $n$ can be reduced to finding $O(\frac{1}{m^4})$-approximate NE in two-player $O(m) \times O(m)$ game, where $m=O(n^4)$. 
% \end{theorem}

% \begin{theorem}[NeedToShow]
% End of Line PPAD problem with size $n$ can be reduced to finding $O(\frac{1}{m})$-approximate NE in a two-player $m \times m$ game, where $m=O(n^4)$ (we may be able to bring this down to O(n)).  
% \end{theorem}

% \Pnote{I see. So at this point, we need a $2^{o(n^{1/4})}$ time algorithm for $1/n$-approximate Nash equilibrium computation in order t refute ETH for PPAD.}

% \Rnote{Looks like that. $1/m$-approximate NE in $2^{o(m^{1/4})}$ would give $2^{o(n)}$ for $m=O(n^4)$. I really hope to bring $m$ down to $O(n)$.}

% \section{An SDP Lower Bound?}
% Is there an instance of a poly-matrix game with players denoted by $u \in [2n]$ and a SDP solution such that for every $q$ players $Q \subseteq [2n]$, $|Q| = q$, the marginal distribution over $\{ x_u \in \Delta_2 | u \in Q\}$ is pairwise uniform? 

% We want to construct a pay-off matrix $A$ over a $3$-regular graph $G$ such that there's an SDP solution to 3.7 the marginal distribution on any $q$ of the player's strategies is pairwise uniform. 

% \section{SDPs and stuff}
% Max-Cut Problem
% \begin{align*}
% \max & \langle L, xx^{\top} \rangle \\
% \text{s.t. } x_i^2 & = 1 \text{ for every i }\\
% \end{align*}

% Here's the standard way to write SDP relaxation. 
% \begin{align*}
% \max & \langle L, X \rangle\\
% \text{s.t.} X & \succeq 0 \\
% X_{i,i} &= 1 \text{ for every i}.
% \end{align*}

% One standard way to obtain an $n \times n$ PSD matrix  $X$ is to think of $n$ vectors in whatever dimensions and $X_{i,j} = \langle v_i, v_j \rangle.$ This is PSD is easy. And only slightly harder is the claim that every psd matrix can be written as a gram matrix of some vectors. 

% This kind of thinking is fine for the basic SDP that we wrote above. 

% We could think of adding more constraints to the SDP above in order to strengthen it - this sum-of-squares is a way of adding more constraints. 

% Sum of squares SDP has constraints for any group of small number of variables. Let me write down $SoS_d$ relaxation for max cut. The above SDP can be thought of as $SoS_1$ relaxation. 

% Let me write this down next. 

% First, $ \langle L, xx^{\top} \rangle$ equals the size of the cut denoted by $x$. This is same as $\sum_{i,j \in [n]} x_i x_j L_{i,j}.$ In the intended solution, $X_{\{i\}, \{j\}} = x_i x_j$.   

% It is less awkward to write a constraint in tensor notation. Let $X$ be an object that lives in $\R^{n^{2d}}$ seen as a $2d$-tuples on $[n]$. This will be the object we want to optimize over. 

% The indices of this object can be thought of as ordered $\leq 2d$-tuples of elements from $[n]$. Of course, as usual, the intended solution is $X_S = \Pi_{i \in S} x_i$ for every $S \subseteq [n]$, $|S| \leq 2d.$

% Before, we relaxed rank 1 matrix constraint to PSD constraint and trace constraint. In notation, we wrote the constraint $X = \sum_{i} \lambda_i u_iu_i^{\top}$ where the $\lambda_i$s are non-negative and sum up to $n$ and $u_i$s are unit vectors, as a relaxation of $X = xx^{\top}$ for $x$ being a vector of norm $\sqrt{n}$ (since it's a plus-minus 1 vector)

% This time, we could observe that $X$ is intended to be a rank $1$ tensor of $2d$ dimensions. The natural generalization of PSDness with bounded trace that we can think of would be 
% \begin{equation} \label{tensor-psd}
% X = \sum_{i} \lambda_i u_i^{\otimes 2d}
% \end{equation}
% where $\lambda_i$s sum up to $n$ and $u_i$s are unit vectors. Clearly, this would be a valid relaxation. However, unfortunately, we cannot optimize over such "PSD-tensors" unlike PSD matrices. So this relaxation is too strong.

% Instead, we arrange the intended solution as a $n^d$ by $n^d$ matrix. Any matrix obtained from a rank $1$ tensor would be rank $1$ (rank 1 as a tensor is a much stronger condition than rank 1 as a matrix). We then relax this rank 1 constraint to PSDness with bounded trace.

% All is not lost though - we can capture more properties of rank 1 tensors by forcing the symmetry constraints that are properties of rank 1 tensors (and not arbitrary rank 1 $n^d \times n^d$ matrices).

% Okay - so doing this more concretely now.

% Let $M(X)$ be the $\approx n^d \times n^d$ matrix representation of $X$. That is, $M_{S,T}$ for any $S, T \subseteq [n]$, $|S|, |T| \leq d$, $M_{S,T} = X_{S} X_{T}.$ 

% The intended solution $X$ is supposed to be a rank 1 tensor.
% Observe that for the intended actual solution, $M(X)$ is PSD

% \begin{align*}
% \max & \sum_{i,j} X_{i,j} \cdot L_{i,j}\\
% M(X) &\succeq 0\\
% \text{ For every $\leq d-2$ tuple $S$} &\text{for every $i$ } X_{S} = X_{(S, i,i)}\\
% \text{ For every $\leq d$} & \text{ tuple $S$, $T$ that are permutations of each other } X_S = X_T
% \end{align*}

% The second last constraint follows from $x_i^2 = 1$ (to see this, check that the constraint holds for the intended solution for $X$). 

% The last constraint are the symmetries of the intended rank 1 tensor solution.

% This is the sum of squares SDP. What we can show is that for $d = n$ this is an exact relaxation! Now the vector version is not a good enough - so we think of distributions. 

% To think of SDP solutions as distributions, we think of any feasible $X$ to the above SDP as the "moment-tensor" of the distribution. 

% Recall that for a distribution $\mu$ over $\R^n$, the degree $\leq d$ moment tensor  $Q$ of $\mu$ is the following object:

% $Q$ is indexed by tuples of size at most $d$. The entry at any tuple $$Q(i_1, i_2, ..., i_{d'}) = \E_{x \sim \mu}[] \Pi_{j\leq d'} x_{i_j'}].$$

% Recall our intended relaxation that unfortunately wasn't efficiently optimizable  - the convex combinations of rank 1 tensors. That is (not hard to see) equivalent to the constraint that the $X$ is a $2d$-moment tensor of some distribution. As we discussed above, we can't hope to enforce that constraint efficiently. We instead did the symmetry + matrix-psd relaxation above. That captures only some properties of being a moment tensor so in actuality, we cannot assume that SDP solution is a moment tensor. 

% Regardless, it turns out to be a good device in coming up with rounding algorithms to think of actual distributions and their moment tensors as solutions that the SDP returns. Usually, under fairly general situations, we can convert our ideas for actual distributions into those that work for these funny relaxations of them.

% One of the properties (that is not hard to show) of a 2d degree SDP solution above is that over any 2d variables, the "marginal" SDP solution (that is "moments" restricted to only some 2d variables) is always an ACTUAL moment tensor.

% Going to stop rambling now! :-)

\section{Gilbow-Zemel Construction: Clique to Game}
Given an undirected graph $G$ on $n$ vertices represented by an adjacency matrix $E$ (abuse of notation), we wish to check if it has a clique of size $k\le n$. We will reduce this problem to checking if a two player game has more than one equilibrium. 

For $\delta \in (0, 1)$, $M>1$ , and $A=E + (1+\delta) I_{n\times n}$, $B=-M* I_{n\times n}$ and $B'=k*I_{n\times n}$, consider the following $2n+1 \times 2n+1$ block matrices:
\[
R=\left[\begin{array}{cc}
\begin{array}{cc}
A & B\\
B' & \zeros_{n\times n}\\
\end{array}
& -M \ones_{2n \times 1}\\
(1+\frac{\delta}{k}) \ones_{1\times 2n} & 1+\frac{\delta}{k}
\end{array}\right]
\ \ \ \ \ \ 
C=\left[\begin{array}{cc}
\begin{array}{cc}
A & B'\\
B & \zeros_{n\times n}\\
\end{array}
& (1+\frac{\delta}{k}) \ones_{2n\times 1}\\
-M \ones_{2n\times 1}& 1+\frac{\delta}{k}
\end{array}\right]
\]


Note that game $(R,C)$ is symmetric, i.e., $C=R^T$. For ease of notation let $m=2n+1$. For any given mixed strategy $\xx \in \Delta_{m}$, we will denote its support by $S(\xx)=\{i \ |\ x_i>0\}$. 


\begin{lemma}\label{lem:gz1}
$(\xx,\yy)$ is a NE of game $(R,C)$ where $S(\xx),S(\yy) \subseteq \{1,\dots,n\}$ iff graph $G$ has a clique of size $k$. 
\end{lemma}
\begin{proof}
From clique to NE is easy to see. Let $K\subset \{1,\dots,n\}$ be the vertices on the $k$-clique. Then setting $x_u=y_u=1/k,\ \forall u \in K$, and $x_u=y_u=0$ otherwise is a Nash equilibrium. This is because payoff from each non-zero strategy is $(1+\delta/k)$, and from strategies with zero probability it is at most $(1+\delta/k)$. 

To map NE supported on first $n$ strategies to clique in graph $G$, first observe that no matter what the column player is playing, row player gets $(1+\delta/k)$ from the last strategy $m$, and vice-versa. Therefore, all the non-zero strategies of both the players has to give at least $(1+\delta/k)$ payoff. This is possible for the row player only if $S(\yy)$ forms a clique, and for each $j \in S(\yy),\ y_j\ge \frac{1}{k}$. This implies $|S(\yy)|\le k$.

Now it suffices to argue that $|S(\yy)|=k$. To the contrary suppose $|S(\yy)|<k$. Let $j^* = \argmax_{j \le m} y_j$, then clearly $y_{j^*} \ge \frac{1}{k-1}$. 
Row player's payoff from any $i\in \{1,\dots, n\}$ is at most $1+\delta y_{j^*}<1+y_{j^*}$, where the inequality is due to $\delta<1$. While from strategy $n+j$ it is $k * y_{j^*} = (k-1) y_{j^*} + y_{j^*} \ge 1+y_{j^*}$, where the last inequality is due to $y_{j^*}\ge \frac{1}{(k-1)}$. A contradiction to $S(\xx)\subseteq \{1,\dots,n\}$. 

Since the game is symmetric, we can similarly argue that vertices corresponding strategies in $S(\xx)$ forms a $k$-clique in graph $G$. 
\end{proof}

\begin{lemma}\label{lem:gz2}
If $(\xx,\yy)$ is a Nash equilibrium of game $(R,C)$ then either $S(\xx),S(\yy) \in \{1,\dots,n\}$ or $S(\xx)=S(\yy) = 2n+1$. 
\end{lemma}
\begin{proof}
To the contrary suppose neither holds for $S(\yy)\Rightarrow y_L =  \sum_{i=1}^n y_i <1$. 
This proof is based on a number of observations which I will list next with a brief justification.
\begin{enumerate}
\item If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$ then $S(\xx)=\{m\}$, and vice-versa: This is because any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of $(1+\delta/k)$. 
%\item If $\exists i \in S(\yy) \cap \{1,\dots,n\}$ such that $y_i \ge \frac{1}{k-1}$, then $S(\xx)\cap \{1,\dots,n\} = \emptyset$, and vice-versa: Let $i^* = \argmax_{i \le n} y_i$, then payoff of player one from strategy $n+i^*$ is $ky_{i^*}-My_m=(k-1)y_{i^*} + y_{i^*} -My_m\ge 1+y_{i^*}-My_m$. While for any $i\le n$, her payoff is at most $1+\delta y_i - M y_{n+i} - M y_m<1+y_{i^*}-My_m$. The claim follows.
\item $\forall i \in S(\xx)$, $(Ry)_i \ge 1+\delta/k$, and similarly for player two: This follows from the fact that the last strategy always gives $(1+\delta/k)$ payoff regardless of what the other player is playing. 
\item $\forall i\le n, x_i > 0 \Rightarrow y_i \ge \frac{1}{k}$, and $y_i>0 \Rightarrow x_i \ge \frac{1}{k}$: This follows from the fact that player one gets at most $(1+\delta y_i)$ payoff from strategy $i\le n$. Therefore using point (2), $x_i > 0 \Rightarrow (1+\delta y_i) \ge 1+\delta/k$, and the claim follows.  
%\item $\forall i\le n, x_{n+i}>0 \Rightarrow y_i \ge \frac{1}{k} + \frac{\delta}{k^2}$, and $y_{n+i}>0 \Rightarrow x_i \ge \frac{1}{k} + \frac{\delta}{k^2}$: Proof follows from the fact that payoff of the two players from strategy $(n+i)$ is $k*y_i$ or $k*x_i$ respectively. They need to be at least $(1+\delta/k)$ due to point (2).
%\item From point (4) it follows that $|S(\xx) \cap \{n+1,\dots,2n\}|\le (k-1)$ and $|S(\yy) \cap \{n+1,\dots,2n\} \le (k-1)$.
\item $y_L <1$ together with point (3) implies $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$. Point (3) also implies $S(\yy) \cap \{1,\dots,n\} =S(\xx) \cap \{1,\dots,n\}\Rightarrow |S(\yy) \cap \{1,\dots,n\}|\le (k-1)$. 
\item If $S(\xx) \cap \{1,\dots, n\}\neq \emptyset$ then $\exists i \le n$ such that $x_i>0$ and payoff$_1(i) < (1+1/(k-1)) y_L$: For each $i\le n$ payoff$_1(i) \le y_L + \delta y_i - M y_{n+i}-M y_m$. Summing these up for non-zero $x_i$'s, using points (3) and (4), we get $\sum_{i\le n: x_i>0} \mbox{ payoff}_1(i) < (k-1) y_L + \delta y_L $. Since there are at most $(k-1)$ non-zero startagies among first $n$ strategies (point (4)), one of them has to give payoff at most $(k-1)$ of this value i.e., $\exists i\le n$ such that $x_i>0$ and payoff$_1(i)< (1+\delta/(k-1)) y_L < (1+1/(k-1)) y_L$ 
\item $\exists i \le n$ such that payoff$_1(n+i)\ge (1+1/(k-1)) y_L$: From point (4) it follows that if $i^* = \argmax_{i\le n} y_i$ then $y_{i^*} \ge y_L/(k-1)$. Therefore, payoff$_1(n+i^*) = ky_{i^*} \ge (1+1/(k-1)) y_L$. 
%\item $y_R = \sum_{i=n+1}^{2n} y_i \le \frac{2\delta}{M}$ and $x_R = \sum_{i=n+1}^{2n} y_i \le \frac{2\delta}{M}$
\end{enumerate}
If there is a strategy $i\le n$ that is a best response of the first player, i.e., $i \in S(\xx)$, then points (5) and (6) implies that there will be one played with non-zero probability that gives lower than highest payoff, which can not be the case at a Nash equilibrium. Therefore, essentially last two points imply that $S(\xx) \cap \{1,\dots,n\} =\emptyset$. This with point (1) implies that $S(\yy)=2n+1$, a contradiction to the initial assumption. 
\end{proof}

\noindent{\bf Approximation.} For $\epsilon = \frac{1}{2k^3}$ approximate well-supported equilibrium, Lemma \ref{lem:gz1} would follow. However, Lemma \ref{lem:gz2} is tricky to show. Change the game a a bit by replacing entries in the last row of matrix $R$ and last column of matrix $C$ to $1+\frac{\delta}{k} + \frac{\delta}{k^3}$. Set $\delta=\frac{1}{2}$.


\begin{lemma}\label{lem:gz2}
Given that graph $G$ does not have a clique of size $(k-1)$, if $(\xx,\yy)$ is a $\frac{1}{2k^3}$-approximate well-supported Nash equilibrium of game $(R,C)$ then either $S(\xx)=S(\yy)=\{2n+1\}$. % \in \{1,\dots,n\}$ or $S(\xx)=S(\yy) = 2n+1$. 
\end{lemma}
\begin{proof}
To the contrary suppose $S(\yy)\neq \{2n+1\}$. Recall that $m=2n+1$%neither holds for $S(\yy)\Rightarrow y_L =  \sum_{i=1}^n y_i <1$. 
This proof is based on a number of observations which I will list next with a brief justification.
\begin{enumerate}
\item $S(\yy) \cap \{1,\dots,n\} \neq \emptyset$ and $S(\xx) \cap \{1,\dots,n\} \neq \emptyset$: If $S(\yy) \subseteq\{n+1,\dots, 2n+1\}$, then $S(\xx)=\{2n+1\}$ since any strategy other than the last one gives non-positive payoff to player one, while the last one gives payoff of at least $1$. In that case, by the same argument $S(\yy)=\{2n+1\}$, a contradiction. Second part follows similarly. 

\item $\forall i \in S(\xx)$, $(Ry)_i \ge 1+\delta/k$, and similarly for player two: This follows from the fact that the last strategy always gives $(R\yy)_m = (1+\delta/k + \delta/2k^3)$ payoff regardless of what the other player is playing, and that $(R\yy)_m -\epsilon = 1+\delta/k$. 

\item $\forall i\le n, x_i > 0 \Rightarrow y_i \ge \frac{1}{k}$, and $y_i>0 \Rightarrow x_i \ge \frac{1}{k}$: This follows from the fact that player one gets at most $(1+\delta y_i)$ payoff from strategy $i\le n$. Therefore using point (2), $x_i > 0 \Rightarrow (1+\delta y_i) \ge 1+\delta/k$, and the claim follows.  

\item $\forall i \in S(\yy) \cap \{1,\dots,n\}$, $y_i < \frac{1}{k-1}$, and similary for $\xx$: Let $i^* = \argmax_{i \le n} y_i$, then payoff of player one from strategy $n+i^*$ is $ky_{i^*}-My_m=(k-1)y_{i^*} + y_{i^*} -My_m\ge 1+y_{i^*}-My_m$. While for any $i\le n$, her payoff is at most $1+\delta y_i - M y_{n+i} - M y_m<1+\frac{y_{i^*}}{2}-My_m$. Thus payoff from strategy $n+i^*$ is at least $y_{i^*}/2$ higher than any of the strategies $i \le n$. From (3) we get a lower bound of $\frac{1}{k}$ on $y_{i^*}$, which would imply $S(\xx) \cap \{1,\dots,n\}=\emptyset$ contradicting (1). 

%\item $\forall i\le n, x_{n+i}>0 \Rightarrow y_i \ge \frac{1}{k} + \frac{\delta}{k^2}$, and $y_{n+i}>0 \Rightarrow x_i \ge \frac{1}{k} + \frac{\delta}{k^2}$: Proof follows from the fact that payoff of the two players from strategy $(n+i)$ is $k*y_i$ or $k*x_i$ respectively. They need to be at least $(1+\delta/k)$ due to point (2).
%\item From point (4) it follows that $|S(\xx) \cap \{n+1,\dots,2n\}|\le (k-1)$ and $|S(\yy) \cap \{n+1,\dots,2n\} \le (k-1)$.

\item $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$ and $|S(\yy) \cap \{1,\dots,n\}| \le (k-1)$: Since $G$ does not have a clique from Lemma \ref{lem:gz1} we know that either $y_L=\sum_{i\le n} y_i<1$ or $x_L=\sum_{i\le n} x_i<1$. Suppose the first holds, then (3) implies $|S(\xx) \cap \{1,\dots,n\}| \le (k-1)$. Point (3) also implies $S(\yy) \cap \{1,\dots,n\} =S(\xx) \cap \{1,\dots,n\}$ giving us $|S(\yy) \cap \{1,\dots,n\}|\le (k-1)$ as well.
\end{enumerate}

Let $S= S(\yy) \cap \{1,\dots,n\}$ ($=S(\xx) \cap \{1,\dots,n\}$ due to (3)). 
Since $G$ does not have a clique of size $k-1$, there is some $i \in S$ that has $R(i,j)=0$ for some $j \in S$. Therefore, payoff$_1(i) = (R\yy)_i \le y_L - y_j + \delta y_i$. From (3) we know that $y_j \ge \frac{1}{k}$ and from (4) we have $y_i \le \frac{1}{k-1}$. Applying these to payoff expression we get payoff$_1(i) \le y_L - \frac{1}{k} + \frac{1}{2(k-1)}$. From (2) this value has to be at least $1+1/2k$, which would require $k \le 1/2$, a contradiction. 
\end{proof}

To allow assumption that $k$-clique does not exist in graph $G$ in the above lemma, 
%To allow graphs with $(k-1)$ sized clique, but no $k$ sized clique, 
we can make the above proof work by setting last row of $R$ and last column of $C$ to $1+\delta/(k-1)+\delta/2k^3$. This would also simplify the proof because essentially we will get lower bound of $1/(k-1)$ in point (3), and then point (4) will contradict it. 


For game constructed from graphs with $k$-clique, we want to ensure that no $\epsilon$-approximate equilibrium gives non-zero probability to the last startegy. We can do this by changing last row and last column of $R$ and $C$ respectively to $-1$. 

\noindent{\bf Question.} Now can we show that SDPs of these two games will have a common solution?

I will next try to see if the 3SAT example works as well. 


==> content/org-intro.tex <==
%!TEX root=../main.tex
\newcommand{\on}{\{-1,1\}}
\section{Introduction}
% \Pnote{Plan:
% 1. We have a new restricted model to study for equilibrium computation.\\ 
% a) Oblivious Rounding - history and why many combinatorial optimization problems have oblivious rounding based algorithms. Feige's paper on oblivious rounding. \\
% b) Oblivious Rounding with Checking Oracle\\

% 2. Why should we care about this model?\\
% We can capture the LMM algorithm a) oblivious rounding with no checking. There's a paper of Harrow et. al. which is not oblivious rounding. \\
% Might be good to check if any other algorithms for computing equilibria can be recast as oblivious rounding.\\ 

% Gaining evidence for hardness in this model?\\
% Two kinds of regimes: constant approximate equilibria and (1/n)-exact equilibria. \\

% What we have currently:

% 3. Hardness for Oblivious Rounding\\
% a) Reduction from Clique - Hazan Krauthgamer - $n^{log n}$ hardness for constant approximate equilibrium computation - not sure. \\
% b) Reduction from independent set - $2^n$ hardness for 1/poly(n) approximate equilibria - we have. \\

% 4. Hardness for Oblivious Rounding with Checking Oracle\\
% a) $n^{log n}$ hardness for constant approximate equilibria. \\
% b) $2^n$ hardness for $1/poly(n)$ approximate equilibria. \\
% }



Convex relaxations, especially the ones based on general purpose hierarchies of linear and semidefinite programs have proven to be reliable tools for an algorithm designer. Consequently, lower bounds against strong semi-definite programming hierarchies have served as unconditional evidence for hardness especially in settings such as average case complexity where the standard machinery of NP-hardness reductions is inadequate. \Pnote{cite the hell out of everything}

The principle focus of this work is the algorithmic complexity of computing equilibria in two player games. This problem has been the principle focus of algorithmic game theory since its inception. Despite more than three decades of work, efficient algorithms for the problem are known only in specialized situations. On the other hand, there are principled reasons that make the task of establishing lower bounds for NE computation via NP-hardness (and more generally, problems in the class TFNP), namely if equilibrium computation is NP-hard then NP=co-NP \cite{MP}.









% The algorithmic complexity of Nash equilibria in two-player games has been a principle focus 

 % This led to the formalization of the complexity class PPAD (within TFNP) and subsequent results that establishing PPAD-completeness of NE computation which is largely interpreted as precluding a polynomial time algorithm for computing NE in two-player games. However, a long standing goal in algorithmic game theory has been to relate hardness of computing equilibria to standard hardness assumptions in computational complexity theory. 
\Pnote{story for intro:

PPAD is not well understood. 
Multiple situations where general class of problems are ill understood.
Known, general purpose algorithms are largely "enumerative".  
On the flip side, worst-case hardness is known under strong assumptions. Mention Aviad. 



Usual recipe in other areas: lower bounds in restricted algorithmic models. Example of average case complexity. 

Can we hope to do the same here? State flurry of work on decision problem lower bounds. Talk about the issue with hardness of computing any equilibrium. 

How do we ask the question of enumerative vs non-enumerative algorithms? 

All these questions can be formalized by thinking of a oracle access to games and allowing oracle access to solutions of strong convex relaxations....we formalize...}



%Proving lower bounds


While PPAD-hardness is generally taken to imply computational intractability of the underlying problem, like many other conjectures in computational complexity, the status of PPAD-hardness remains unresolved. A grand unfulfilled goal in the field is to relate PPAD to standard complexity classes such as NP so as to put hardness of problems in PPAD on a more solid footing. Recently, stakes have been raised with the positing of a strong conjecture informally known as the ETH for PPAD \cite{BPW}, assuming which Rubinstein \cite{Rub} shower a lower bound tantalizingly close to the classical algorithm for computing constant approximate Nash equilibrium in two plyaer games due to Lipton, Markakis and Mehta. 

%Rubinstein raised the stakes in this context by positing a strong conjecture informally called as the ETH for PPAD and showed that it implies a lower bound tantalizingly close to the classical algorithm for computing approximate Nash equilibrium in two player games due to Lipton, Markakis and Mehta. 





By now, there are several generic and important settings where evidence of hardness based on standard assumptions such as P vs NP is considered hard or infeasible. In many such settings, lower bounds on restricted, but strong classes of algorithms have served as a proxy for such evidence - corroborating and often even suggesting hardness results likely to hold. Deeply intertwined with this goal is the dual task of developing a general algorithmic framework for the class of problems under scrutiny. We'd want that the framework be powerful enough to allow for most existing techniques to be captured within it and at the same time, restricted enough to be amenable to a thorough analysis, and in particular, strong lower bounds. In combinatorial optimization, convex relaxations in general and linear and semi-definite programming hierarchies in particular have played this role. 

The above discussion naturally suggests two basic and broad questions in the context of complexity of equilibria: 
Can a generic linear/semi-definite programming hierarchy capture general techniques for computing equilibria in various games? 
In particular, is there a formal way to ask for ``non-enumerative'' algorithms? \Pnote{mostly to remember that this needs to be said.} 
Could we hope to show a lower bound in such a general model and gain evidence for PPAD-hardness and the stronger versions such as ETH for PPAD?

\Pnote{this paragraph is incorrect and overattributes arrow et. al.}A recent work by Harrow et. al. \cite{HNW} addresses the first question and establishes that generic semi-definite programming hierarchies (the sum-of-squares hierarchy in particular) can capture the well-known algorithm of Lipton-Markakis-Mehta for computing approximate equilibria. Natural approaches towards the second question, however, are met with an immediate barrier - the same barrier that makes the relationship between the complexity classes PPAD and NP hard to understand \cite{MP}. In showing hardness of combinatorial optimization problems, lower bounds against linear and semi-definite programming relaxations come in one of two flavors: 1) show a family of instances of the problem that admits no "solution" but the relevant LP/SDP relaxations are feasible and, 2) \emph{integrality} gaps - for a natural certain objective function that arises in the problem (size of clique, maximum matching, max weight vertex cover etc.), establish a (multiplicative/additive) gap between the true optimum and the LP/SDP optimum for some carefully constructed family of instances. PPAD is a sub-class of TFNP ("total function NP"), i.e., every two player game has an equilibrium strategy (the ``solution'') and thus the first notion doesn't appear meaningful. 


A long line of influential works have shown integrality gaps for strong SDP/LP relaxations for finding equlibria that optimize some quality-measure such as welfare/payoffs etc \cite{Deligkas-Fearnely-Savani}. \Pnote{Add recent work by Savani etc.}. A generic hardness result of such a flavor shows the existence of a game (usually arrived at via a reduction from some hard optimization problem such as 3SAT/Clique) such that all equilibria have the given quality measure (say welfare) at most $\Delta_1$ while the LP/SDP optimum for the problem of maximizing welfare is $> \Delta_1.$ This certainly establishes the hardness of approximating an optimum (with respect to the considered quality-measure) equilibrium in games. While it can be tempting to interpret such results as suggesting hardness of finding the \emph{any equilibrium} (and not just one that maximizes some quality measure), such an intuition can be misleading. As a simple illustrative example, observe that the integrality gap of standard semi-definite programming relaxations for Max-Cut being $1/0.878$ obviously doesn't imply the hardness of finding a cut in a graph! 


While there's a lot of work establishing integrality gaps for LP/SDP relaxations that attempt to optimize various natural objectives (such as social welfare) over all (approximate or exact) equilibria - however, it is not clear whether the ``hardness'' in such a situation arises from optimizing the objective or searching over the feasible space (equilibria) itself. As a simple example illustrating this, observe that while obtaining a $0.94$ approximate Maximum Cut in a graph is NP-hard, finding a cut in a graph is of course trivial.

This leads to the principle focus of our investigation in the present paper. 
\begin{question}
Can SDP hierarchy lower bounds provide evidence for hardness of computing \emph{any} equilibrium in a two player game, both exact and approximate?
\end{question}

In what follows, we will formalize a restricted class of algorithms for computing equilibria using semi-definite programming hierarchies, show that the model is strong enough to capture general, known techniques for computing equilibria, and establish strong lower bounds for the model. 

\subsection{Games, Equilibria and Quadratic Feasibility Formulation} 
%\Pnote{will be good to shorten this...seems too verbose right now especially in the intro.}
In this paper we focus on two player games. A game $G$ with players Alice and Bob with $n$ strategies for both is described by two payoff matrices $R$ and $C$ in $[-1,1]^{n\times n}$,\footnote{Normalizing payoffs to lie in $[-1,1]$ is without loss of generality.} 
where Alice plays rows and Bob plays columns. 
%The player playing rows is called the row-player and has payoff matrix $R$, and the other player is called column-player with payoff matrix $C$. 
Players may randomize and play a mixed-strategy from $\Delta_n = \{x \in [0,1]^n \mid \sum_{i = 1}^n x_i = 1\}$. We write $\e_i  \in \Delta_n$, for the $i^{th}$ pure strategy. When Alice plays $\xx\in \Delta_n$ and Bob plays $\yy \in \Delta_n$, the expected \emph{payoffs} are $\xx^{\top} R \yy$ and $\xx^{\top} C \yy$for Alice and Bob respectively. Clearly, given an oponent's strategy, there is always a pure strategy giving the maximum payoff, {\em i.e.,} given $\yy$, there exists $i$ such that $e_i \in \argmax_{\xx \in\Delta_n} \xx^\top R \yy$, and similarly for Bob.
At Nash equilibrium (NE) no player gains by deviating unilaterally. That is,
\begin{align}
\xx^{\top} R \yy \geq \e_i^{\top} R \yy  \text{ for all } i \in [n] \notag\\
\xx^{\top} C \yy \geq \xx^{\top} C \e_j  \text{ for all } j \in [n]. \label{eq:NEchar}
\end{align} 
At an $\epsilon$-approximate NE ($\eps$-$\NE$) no player gains by more than $\eps$ by deviating unilaterally: %for the game $G$ can be similarly defined by a strategy profile $(\xx,\yy)$ satisfying:
\begin{align}
\xx^{\top} R \yy \geq \e_i^{\top} A \yy -\epsilon  \text{ for all } i \in [n]  \notag\\
\xx^{\top} C \yy \geq \xx^{\top} B \e_j -\epsilon \text{ for all } j \in [n]. \label{eq:approx-NEchar}
\end{align}

%Note that \eqref{eq:NEchar} and \eqref{eq:approx-NEchar} gives quadratic feasibility formulations for NE and $\eps$-$\NE$ respectively. 
%\eqref{eq:NEchar} (respectively, \eqref{eq:approx-NEchar}) immediately translates into a quadratic feasibility program whose feasible points are all strategy profiles that form NE ($\epsilon$-approximate NE, respectively). 
%Relaxing the feasibility program to a convex program followed by \emph{rounding} then yields a general strategy for the problem of finding NE, whether exact or approximate. \Rnote{Pravesh: I do not understand why this last sentence.}

 %Specifically, given a game $G$ as above, a convex set $\C(G)$ is a convex relaxation for NE if for every strategy profile $(\xx,\yy)$ that forms an equilibrium, there's a 
\subsection{Sum-of-Squares Method and Pseudo-equilibria}
The sum of squares method is a sequence of increasingly tight SDP relaxations for a system of polynomial inequalities. We provide a brief overview of this method specialized to computing (exact/approximate) equilibria here and point the reader to the lecture notes \cite{sos-notes} for further details on method and its applications. Central to the sum of squares method is the notion of a pseudo-distribution that generalizes probability distributions. 

\begin{definition}[Pseudo-distribution]
A degree $d$ pseudo-distribution is a finitely supported signed measure $\tilde{\mu}$ on $\R^n$  such that the associated linear functional (pseudo-expectation) $\pE$ that maps any function $f:\R^n \rightarrow \R$ to $\pE[f] = \sum_{x: \tilde{\mu}(x) \neq 0} \tilde{\mu}(x) f(x)$ satisfies the following properties:
\begin{enumerate}
\item \textbf{Normalization: } $\pE[1] = 1$ or equivalently, $\sum_{x: \tilde{\mu}(x) \neq 0} \tilde{\mu}(x) = 1,$ and
\item \textbf{Positivity: } $\pE[q^2] \geq 0$ for every degree $\leq d/2$ polynomial $q$ on $\R^n.$
\end{enumerate}
A pseudo-distribution $\tilde{\mu}$ is said to satisfy a polynomial inequality constraint $q \geq 0$ if for every polynomial $p$, $\pE[p^2 q] \geq 0$ whenever $\deg(p^2q) \leq d.$
\end{definition}


It's not hard to show that any degree $\infty$ pseudo-distribution is a probability distribution on $\R^n.$
We will now use pseudo-distributions in order to define a relaxation of the notion of equilibrium, which we call, \emph{pseudo-equilibrium}, that sum of squares algorithm can efficiently search over. Throughout this paper, we will be concerned with whether and how pseudo-equilibria be  ``rounded'' to (exact/approximate) equilibria for the underlying games. 

\begin{definition}[Degree $d$ Pseudo-equilibrium]
Given a two player game $(R,C)$, a degree $d$ pseudo-equilibrium for $(R,C)$ is a degree $d$ pseudo-distribution on strategy profiles $(\xx,\yy)$ satisfying the degree 2 polynomial inequality constraints in \eqref{eq:NEchar}. A degree $d$, $\epsilon$-approximate pseudo-equilibrium is a degree $d$ pseudo-distribution over strategy profiles $(\xx,\yy)$ satisfying the degree $2$ polynomial constraints in \eqref{eq:approx-NEchar}.
\end{definition} 


\subsection{The Model: Oblivious Rounding with Verification} 
\Rnote{Pravesh: please check this section}
In this section, we present our algorithmic framework based on restricted roundings of sum-of-squares relaxation for polynomial feasibility problems. Let $\Psi(P)$ be a system of polynomial inequalities in $x \in \R^n$ parameterized by a problem instance $P \in \R^m$. %We allow $P$ to vary in some domain and interpret each different valid value of $P$ as a new instance. 
For example, the natural quadratic programming formulation of \eqref{eq:NEchar} for finding exact NE is a system of degree 2 polynomial inequalities over $\Delta_n \times \Delta_n$ parameterized by the payoff matrices $R,C$ that encode instances of two-player games. And similarly, that of \eqref{eq:approx-NEchar} is for finding $\eps$-$\NE$.

We can now define two algorithmic models that use sum-of-squares relaxations to find solutions to polynomial feasibility program $\Psi(P).$

\begin{definition}[Oblivious Rounding]
Let $\Psi(P)$ be a polynomial feasibility problem parameterized by instances $P$. A degree $d$ oblivious rounding algorithm for $\Psi(P)$ takes input a degree $d$ pseudo-expectation satisfying the constraints in $\Psi(P)$ and outputs a point $x$ that satisfies $\Psi(P).$
\end{definition}

In particular, the rounding algorithm is a function only of the degree $d$ pseudo-expectation satisfying $\Psi(P)$, and is independent of the instance $P$ itself. 
While this notion of rounding might appear restrictive, many of the famous algorithms in combinatorial optimization happen to be oblivious roundings and examples include the Goemans-Williamson algorithm for Max-Cut, the Arora-Rao-Vazirani algorithm for Sparsest-Cut, the Barak-Raghavendra-Steurer and Guruswami-Sinop algorithm for various 2-CSPs among others. %Indeed, there are few examples of approximation algorithms that use SDP rounding and do not use oblivious rounding, \Pnote{add a couple examples} - for example, the rounding algorithms for constraint satisfaction problems due to Uri Zwick and more recently, the rounding algorithms for the sum-of-squares method due to Barak-Kelner-Steurer. 

There are also notable exceptions such as the Facility Location algorithm of \cite??, the generic rounding algorithm for Raghavendra and Steurer for constraint satisfaction and \cite??. This list in fact can be expanded as most of the recent works on roundings sum-of-squares relaxations for various polynomial optimization problems are \emph{not} oblivious. The CSP rounding algorithm of Raghavendra-Steurer and the recent algorithms based on rounding the SoS hierarchy for various polynomial optimization problem all can be seen as generating a small list of candidate solutions based on the SoS solution and then arguing that one of the candidates is a good solution to the problem at hand.

Inspired by these algorithms, we generalize our framework to allow generating a list of candidates based on the SoS solution to yield the central algorithmic model of interest in this work. This allows us to capture all known rounding algorithms mentioned above with the exception of the facility location algorithm of...and \cite??.

For every instance of the underlying problem encoded by $\Psi(P)$, we define the \emph{verification oracle} as follows. 

\begin{definition}[Verification Oracle]
\label{or1}
Let $\Psi(P)$ be a polynomial feasibility problem over $\R^n$. A verification oracle for $P$ takes input a $y \in \R^n$ and accepts if $y$ satisfies every polynomial inequality in $\Psi(P)$ and rejects otherwise.
\end{definition}

In our setting, the above oracle essentially takes a strategy profile $(\xx,\yy)$ and accepts if it is an NE ($\eps$-$NE$), otherwise rejects. 
Note that in \eqref{eq:NEchar} and \eqref{eq:approx-NEchar}, if either $\xx$ or $\yy$ are given then the problem becomes linear and can be checked for feasibility in polynomial time. Motivated from this we allow the following stronger oracle, and prove lower bounds against it.

\begin{definition}[Verification Oracle with Partial Input]
\label{or2}
Let $\Psi(P)$ be a polynomial feasibility problem over $\R^n$. A verification oracle for $P$ takes input a $y \in \R^k$ for $k \le n$ such that 
replacing $y$ in $\Psi(P)$ results in a linear system of inequalities. Then the oracle accepts if this linear system is feasible and rejects otherwise. 
\end{definition}


\begin{definition}[Oblivious Rounding with Verification Oracle]
Let $\Psi(P)$ be a polynomial feasibility problem parameterized by instances $P$. A degree $d$, $q$ query oblivious rounding with verification algorithm for $\Psi(P)$ takes input a degree $d$ pseudo-expectation satisfying the constraints in $\Psi(P)$ and outputs a list of $q$ points $x_1, x_2, \ldots, x_q$ 
is accepted by the Verification Oracle \ref{or2}. 
%\in \R^n$ such that at least one of the $x_i$s satisfies $\Psi(P).$
\end{definition}



\subsection{Our Results}
We are now ready to describe our main results.

Observe that the algorithm of Lipton-Markakis-Mehta is a degree $0$, $n^{O(\log{(n)}/\epsilon^2}$-query algorithm for finding $\epsilon$-approximate equilibria in two-player games. We show that there's an oblivious rounding algorithm for degree $O(\log{(n)}/\epsilon^2)$ SoS relaxation for finding $\NE$ that finds sparse $\epsilon$-$\NE$. This, in particular, yields a non enumerative algorithm matching the guarantees of the LMM algorithm. 


\begin{theorem}
There's a degree $O(\log{(n)}/\epsilon^2)$, oblivious rounding algorithm (with zero queries to the verification oracle) for finding $\epsilon$-approximate equilibria in two-player games with $n$ strategies.
\end{theorem}

This result shows that SoS relaxations for computing equilibria can be quite powerful and thus motivates the question of understanding whether we can round SoS solutions to good equilibria. Our next result shows a strong limitation of this approach and provides an exponential lower bound on algorithms using oblivious rounding with verification oracle for computing $\Theta(1/n)$-approximate equilibria in two-player games with $n$ strategies. 

\begin{theorem} \label{thm:main-exact}
Suppose there exists a degree $d$, $q$-query algorithm for computing $\Theta(1/n^4)$-approximate equilibria in two-player games with $n$ strategies. Then, either $d = \Omega(n)$ or $q = 2^{\Omega(n)}.$
\end{theorem}

Our second result is a similar statement for constant-approximate equilibria.
\begin{theorem} \label{thm:main-approx}
Suppose there exists a degree $d$, $q$-query algorithm for computing $\epsilon$-approximate equilibria in two-player games with $n$ strategies for some small enough $\epsilon = \Theta(1)$. Then, either $d = \Omega(\log{(n)})$ or $q = n^{\Omega(\log{(n)}}.$
\end{theorem}

\Rnote{Pravesh: should we write the following as corollaries?}
In the process of proving the above two lower bounds, we improve upon three known results. Fist, \Rnote{Pravesh: about Arrow stuff..}

Second, we prove a gap version of the result by Gilbow and Zemel.
\begin{corollary}
Given a graph $G$ and the $k$-Clique (or $k$-independent set) problem, a game $(R,C)$ can be constructed such that: $(i)$ if $G$ has a $k$-Clque then the game has a NE with payoff $\delta>0$. $(ii)$ if $G$ has no $k$-Clique then all $\eps$ approximate of $G$ has payoffs at most $(\delta - \eps)$ for $\eps \le O(1/n^2)$. 
%on reduction from $k$-Clique to checking existence of more than one NE. In essence, we construct a game such that existence of $k$-Clique implies existene of a high payoff NE, while non-existence of $k$-clique implies all $O(1/n^2)$ approximate NE having bad payoff. 
\end{corollary}

Third, we extend the result of Daskalakis and Papadimitriou on lower bounds for oblivious rounding methods. Their construction against Oracle \ref{or1}. We extend it and show lower bound against the powerful Oracle \ref{or2}. %and for a weaker notion of NE:  
\begin{corollary}
For a given game $(R,C)$ with $n$ strategies, if an algorithm queries Oracle \ref{or2} $q$ times and outputs an $O(1)$-$\NE$ of $(R,C)$, then $q=n^{\Omega(\log{(n)})}$. 
\end{corollary}



\begin{remark}
There is a stronger notion of approximation known as well-supported approximate NE (\WNE), that too has been widely studied.
%\WNE is a stronger notion of approximation that has been widely studied. 
Since every $\eps$-\WNE of a game is also its $\eps$-$\NE$, the above lower bounds holds for \WNE as well. 
Digging further into our results, it turns out that we can improve the approximation ratios significantly while keeping the lower bounds as is, {\em e.g.,} exponential lower bounds for $O(1/n^2)$ approximation. Furthermore, all results can be extended to even more powerful oracle that is only possible for \WNE, namely take supports of both players' strategies, and output if there is an $\eps$-\WNE with the given support.
To keep the exposition clean and intuitive, we stick to $\NE$. 
\end{remark}

\begin{comment}

Oblivious rounding for generic combinatorial optimization problems has received significant attention in works beginning with Feige who observed that most natural algorithms based on rounding LPs/SDPs are in fact oblivious rounding algorithms. He also observed some notable exceptions such as the Facility Location algorithm of \cite??, the generic rounding algorithm for Raghavendra and Steurer for constraint satisfaction and \cite??. This list in fact can be expanded as most of the recent works on roundings sum-of-squares relaxations for various polynomial optimization problems are \emph{not} oblivious. The CSP rounding algorithm of Raghavendra-Steurer and the recent algorithms based on rounding the SoS hierarchy for various polynomial optimization problem all can be seen as generating a small list of candidate solutions based on the SoS solution and then arguing that one of the candidates is a good solution to the problem at hand. 

Inspired by these algorithms, we generalize our framework to allow generating a list of candidates based on the SoS solution to yield the central algorithmic model of interest in this work. This allows us to capture all known rounding algorithms mentioned above with the exception of the facility location algorithm of...and \cite??.

For every instance of the underlying problem encoded by $\Psi(P)$, we define the \emph{verification oracle} as follows. 

\begin{definition}[Verification Oracle]
Let $\Psi(P)$ be a polynomial feasibility problem over $\R^n$. A verification oracle for $P$ takes input a $y \in \R^n$ and accepts if $y$ satisfies every polynomial inequality in $\Psi(P)$ and rejects otherwise.
\end{definition}


\begin{definition}[Oblivious Rounding with Verification Oracle]
Let $\Psi(P)$ be a polynomial feasibility problem parameterized by instances $P$. An degree $d$, $q$ query oblivious rounding with verification algorithm for $\Psi(P)$ takes input a degree $d$ pseudo-expectation satisfying the constraints in $\Psi(P)$ and outputs a list of $q$ points $x_1, x_2, \ldots, x_q \in \R^n$ such that at least one of the $x_i$s satisfies $\Psi(P).$
\end{definition}
\subsection{Restricted Rounding Algorithms}
Integrality gaps for convex relaxations suggest hardness because they rule out approximation ratios better than the integrality gap using any \emph{rounding} algorithm. Thus, we may hope to show that there cannot be any efficient ``rounding'' algorithms: algorithms that take a solution to the SDP/LP and outputs an equilibrium for a given game. However, as the rounding algorithm could just ignore the SDP/LP solution, this is equivalent to unconditionally showing hardness of PPAD problems. Thus, we must force the rounding algorithm to ``use'' the SDP/LP solution in order for such an unconditional result to be possible and meaningful.

The main conceptual contribution of this work is to posit a natural class of rounding algorithms and to propose showing lower bounds against this class of rounding algorithms as a means for suggesting hardness of the problem of finding an equilibrium. In this section, NE could be be replaced by approximate-NE with no change.

\begin{definition}[Oblivious Rounding, $\OR$]
Let $\cal{C}(A,B)$ be a convex relaxation for computing NE in the game $G$ described by payoff matrices $A,B$ for every $A, B \in [-1,1]^{n \times n}.$ An oblivious \emph{rounding} algorithm is a map $\cal{C}(A,B) \rightarrow \Delta_n \times \Delta_n$ that takes a point feasible for $\cal{C}(A,B)$ and outputs a strategy profile that is an NE for $G.$ In particular, the rounding algorithm is a function only of the input feasible point for $\cal{C}(A,B)$ and not the game itself. 
\end{definition}
In other words, oblivious rounding algorithms are a class of methods for finding equilibria that write a generic convex feasibility program that is a convex relaxation for NE in any game and then round a solution to the convex program to an NE without looking at the game again. While this notion of rounding might appear unnatural, many of the famous algorithms in combinatorial optimization happen to be oblivious roundings and examples include the Goemans-Williamson algorithm for Max-Cut, the Arora-Rao-Vazirani algorithm for Sparsest-Cut, the Barak-Raghavendra-Steurer and Guruswami-Sinop algorithm for various 2-CSPs among others. Indeed, there are few examples of approximation algorithms that use SDP rounding and do not use oblivious rounding, \Pnote{add a couple examples} - such exceptions include, for example, the rounding algorithms for constraint satisfaction problems due to Uri Zwick and more recently, the rounding algorithms for the sum-of-squares method due to Barak-Kelner-Steurer. 


It turns out that extending oblivious rounding a little bit allows us to capture all such algorithms as well. We call such rounding algorithms Oblivious Rounding with Verification Oracles. Indeed, we are not aware of any algorithm that uses SDP rounding and cannot be seen as an oblivious rounding with verification oracle. 

On the other hand, there are known rounding algorithms that are not quite captured in the above framework of oblivious rounding. For example, the approximation algorithms of Zwick \cite{DBLP:conf/soda/Zwick98} for CSPs involve using the ``best'' of a random assignment and a canonical rounding of the standard SDP relaxation. We thus strengthen the above framework to allow such algorithms.

\begin{definition}[Oblivious Rounding + Enumeration]

\end{definition}
\end{comment}



% \subsection{Goal}


% \begin{lemma}[Easy One]
% Fix $n \in \N.$ For every $x \in \on^n$, there exists a 3XOR formula $\psi_x$ such that $\psi_x(x) = 1$ and for every $y \in \on^n$ such that $\langle x, y \rangle \leq \delta n$, $\psi_x(y) \leq O(n) \cdot \delta^{1.5}.$
% \end{lemma}
% \begin{proof} 
% Instance: random planted instance with assignment $x$.
% Simple Chernoff + Union bound shows the lemma then. 

% \end{proof}

% \begin{lemma}[Non-trivial]
% For every satisfiable 3 SAT instance $\psi$ on $n$ variables, there's a two-player game with $m$ strategies per player, say, $G_{\psi}$ such that 
% \begin{enumerate}
% \item \text{Completeness: } For every satisfying assignment $x$ of $\psi$, there's a Nash equilibrium $p_x \in \Delta_m$ for $G_{\psi}.$
% \item \text{Soundness: } If $p \in \Delta_m$ is a $\delta$-approximate equilibrium for $G_{\psi}$, then, 
% \end{enumerate}
% \end{lemma}








% Perhaps the most famous example of this phenomenon are in average case complexity, specifically, in understanding computational vs statistical complexity trade-offs. 

% Consider the planted clique problem for example where we are interested in recovering a clique of smallest possible size added to a random graph $G(n,\frac{1}{2})$. While information theoretically, added cliques of size $\gg \log{(n)}$ are uniquely identifiable, all known polynomial time algorithms fail to recover the added clique whenever it is of size $o(\sqrt{n}).$ In the past decade, $\sqrt{n}$ has been used as a ``computational threshold'' for detection of an added clique to a random graph in order to obtain several hardness results in surprisingly diverse fields. The strongest evidence favoring the conjecture (apart from the failure to find an efficient algorithm that works below the conjectured threshold) has been strong lower bounds on restricted classes of algorithms that encapsulate all known attacks on the problem - for example, see the recent lower bound on the sum-of-squares algorithm and lower bounds on statistical algorithms. 







==> content/reduction.tex <==
%!TEX root=../main.tex
\section{The Reduction} \label{sec:reduction}
In this section, we present the reduction of Deligkas et. al. The starting point is the hardness of approximation for the 3SAT problem. While for ETH-hardness, one has to start from worst-case hard instance of 3SAT and apply the PCP theorem to get a hard-to-approximate instance, for SoS-hardness, we can simply start from the random instance of 3SAT and use Grigoriev's theorem to get exponential SoS-hardness of approximating 3SAT. Alternatively, one can view this as saying that ETH is unconditionally true when restricted to the SoS framework and in fact the hard instance is simply a random one!

\begin{fact}[Grigoriev's Theorem] \label{fact:Grigoriev}
Let $\phi$ be a random instance of 3SAT with $m =\Theta(n/\epsilon^2)$ constraints and $n$ variables. Then, with probability at least $1-1/n$, 
\begin{itemize}
\item For every $x \in \zo^n$, the fraction of clauses satisfied in $\phi$ by $x$ is at most $7/8+\epsilon$, and
\item there exists a degree $\Theta(n)$ pseudo-distribution over the satisfying assignments for the instance $\phi.$
\end{itemize}
\end{fact}

Given a hard instance of 3SAT, one transforms it into a 2 prover, \emph{free} game. 

Recall that a two prover game is defined by a distribution $\cD$ over a finite set of question pairs $(Q_1, Q_2)$ with a collection of admissible answer pairs and two players Alice and Bob. In a run of the game, the referee draws a question pair $(Q_1, Q_2)$ from $\cD$ and sends $Q_1$ to Alice and $Q_2$ to Bob and receives answers from them and accepts if the answer pair is in the list of admissible answer pairs for $(Q_1, Q_2).$ A two prover game is said to be \emph{free} if $\cD$ is a product distribution.

A \emph{strategy} for a two prover game is a  pair of functions $f_1$ and $f_2$ that maps questions to an answer. The value of the strategy is the probability that  $(f_1(Q_1),f_2(Q_2))$ belongs to an admissible answer pair for the question pair $(Q_1, Q_2)$ picked at random from $\cD.$



\begin{definition}[Free Game from 3SAT] \label{def:free-game}
Let $\phi$ be a 3SAT instance from Fact \ref{fact:Grigoriev} with $m$ clauses and $n$ variables. 
Let the clauses and variables appearing in $\phi$ each be partitioned into $\sqrt{n}$ different groups, say, $S_1, S_2, \ldots, S_{\sqrt{m}}$ and $T_1, T_2, \ldots, T_{\sqrt{n}}$, respectively. Then, $\phi$ defines a free game as follows:

Let $\cD$ be the uniform distribution on $(S_i,T_j)$ for $i \sim [\sqrt{m}], j \sim [\sqrt{n}]$ define the distribution on question pairs. For $(S_i,T_j)$, an admissible answer pair is an assignment to the variables appearing in each clause in $S_i$ and each variable in $T_j$ such that 1) every clause in $S_i$ is satisfied by the assignment chosen 2) for every variable that appears in some clause in $S_i$ and in $T_j$, the assignments given by the answer pairs match.  

Note that the number of strategies for Merlin 1 are at most $N_1 = 2^{3\sqrt{m}}$ and that for Merlin 2, at most $N_2 = 2^{\sqrt{n}}.$
\end{definition}

The free game $\cF$ can be thought of as a cooperative two player game as follows. The row player has as their strategies the set of all ordered pairs of questions to Merlin 1 and admissible answers for that question. Similarly, the column player has as strategies, all possible questions to Merlin 2 and admissible answers for those questions. Finally, a pair of ordered pairs of questions and answers receive a payoff of 1 (for both row and column player) iff the verifier accepts the two answers on those two questions and $0$ otherwise.  Observe that the size of the cooperative game produced from a free game is at most $\sqrt{m} N_1 \times \sqrt{n} N_2.$


The following completeness result holds for every free game produced from 3SAT instances from Fact \ref{fact:Grigoriev}. 
\begin{lemma}[SoS Completeness for Free Game]
Let $\phi$ be the 3SAT instance with $m = \Theta(n/\epsilon^2)$ clauses and $n$ variables from Fact \ref{fact:Grigoriev}. 
Let $\cF$ be the free game constructed in Definition \ref{def:free-game} from $\phi.$  
Then, there's a pseudo-equilibrium of degree $\Theta(n)$ for the cooperative game defined by $\cF$ with payoff for each player $=1$.
\end{lemma}
\begin{proof}
We will start from the pseudo-distribution of degree $\Theta(n)$ given to us by Fact \ref{fact:Grigoriev} that satisfies every constraint of $\phi$ and use Fact \ref{fact:reductions-within-SoS}. To do this, we need to build a low-degree map from any satisfying assignment $x$ of $\phi$ to a strategy for the Merlins in the free game $\cF$. This is very simple: for any question set $(S_i,T_j)$ - the strategy is described by a bit string of length $3 \sqrt{m}$ and $\sqrt{n}$ respectively - where the bit string corresponds to the assignment for the variables appearing in the clauses in $S_i$ and variables in $T_j$ respectively. For the strategy for the cooperative game we use the following mixed strategy: Merlin 1 chooses a question from $X$ uniformly at random and then chooses the answer corresponding to the assignment $x$ for that question. Similarly, Merlin 2 chooses a question from $Y$ uniformly at random and then chooses the answer corresponding to $x$ for that questions. Using $x_i$ as the assignment for the variable $i$ wherever it appears gives a degree 1 map into strategies of $\cF$. 

It is easy to see that since $x$ (purportedly) satisfies all constraints of $\phi$, it satisfies all clauses in $S_i$ and further, the assignments to variables appearing in both $S_i$ and $T_j$ match. Thus, we obtain a degree $1$ map from any satisfying assignment $x$ into a strategy for $\cF$ with value $1$. Further, it is easy to see (since the maximum possible payoff in the game is $1$) that the strategy constructed above satisfies all constraints of being an $\NE$. Thus, we have exhibited a degree $O(\sqrt{n})$ map from any satisfying assignment $x$ to a $\NE$ of the cooperative game associated with $\cF$. By Fact \ref{fact:reductions-within-SoS}, we immediately obtain a pseudo-distribution of degree $\Theta(n)$ on strategies with value $1$ for $\cF$. 

\end{proof}

The following soundness result holds for the partitions $S_1, S_2, \ldots, S_{\sqrt{m}}$ and $T_1, T_2, \ldots, T_{\sqrt{n}}$ chosen appropriately (we invite the reader to find the details of the reduction in Deligkas et. al...):

\begin{fact}[Soundness, \cite{?}]
There is no strategy for $\cF$ produced from $\phi$ in Fact \ref{fact:Grigoriev} with value exceeding $1-\Omega(1).$
\end{fact}


Deligkas et. al. give a construction of a game $(R',C')$ by taking the cooperative game $(R,C)$ produced from the free game as above and using it to fill the first $\sqrt{m} N_1 \times \sqrt{n} N_2$ block and then adding $H$ rows and columns for $H$ being $2^{|Y|} \approx 2^{\sqrt{n}}.$ The off diagonal blocks are filled with a carefully constructed zero sum game and its transpose. Finally, the bottom diagonal $H \times H$ block is filled with the all zero matrix. It is immediate from the simple argument of Deligkas et. al. that the pseudo-equilibrium described above for $\cF$ is in fact a $\epsilon$-approximate pseudo-equilibrium in $(R',C')$ - the only required fact in this argument is that the equilibrium strategy $\yy$ ($\xx$ respectively) satisfy $\sum_{b} \yy(y,b) = 1$ for every question $y$ to Merlin $2$. This is a linear polynomial equality constraint that carries over to the pseudo-distribution in a straightforward way. 

We omit the simple and standard argument here and summarize the result that immediately follows from Deligkas et. al. below:
\begin{fact}[Corollary of \cite{Deligkas..}]
Let $\cF$ be a free game with $\sqrt{m}$ ($\sqrt{n}$, respectively) possible questions and $N_1$ ($N_2$, respectively) possible strategies for Merlin 1 (2, respectively.)  
Then, there's a two player game with $\sqrt{m} \cdot N_1$ strategies for the row player and $\sqrt{n} \cdot N_2$ strategies for the column payer such that: 
\begin{enumerate}
\item \textbf{Completeness: } There's a $\epsilon$-approximate pseudo-equilibrium of degree $\Theta(n)$ = $\Omega(\log{(N_1 + N_2)})$ where both players receive a payoff of at least $1$. 

\item \textbf{Soundness: } For every $\epsilon$-approximate $\NE$ of the game, the payoff of either player is at most $1-1/1200.$ 
\end{enumerate}

\end{fact}



==> content/upper-bound.tex <==
%!TEX root=../main.tex

\section{Oblivious Rounding for Finding Approximate Equilibria}
\label{sec:upper-bound}




In this section, we describe our rounding algorithm for sum-of-squares that recovers the guarantees of the LMM algorithm without any enumeration. In other words, our rounding algorithm is oblivious. The following is the main theorem of this section. 

\begin{theorem}[Oblivious Rounding for Finding Sparse Approximate Equilibria] \label{thm:upper-bound-technical}
There's a randomized \emph{oblivious} rounding algorithm for the sum-of-squares relaxation of degree $O(\log{(n)}/\epsilon^2)$ for finding $\NE$ that takes input a $n$-strategy game $(A,B)$ and outputs a $O(\log{(n)}/\epsilon^2)$-sparse $\epsilon$-approximate $\NE$ for $(A,B)$ with probability at least $1-1/n.$ 
\end{theorem}

In the next subsection, we collect some preliminaries that are helpful in the analysis and description of our rounding algorithm. 

\subsection{Preliminaries}
In this section, we collect some tools for analyzing rounding algorithms for SoS relaxations.

\paragraph{Notation} Let $\U_S$ denote the uniform distribution on subset $S$ of $[n].$ Let $\cS_k(n)$ denote the set of all multi-subsets of $[n]$ of size $k$. For a multi-set $S \in \cS_k(n)$ and $z \in \R^n$, let $z^S$ be the monomial in $z$ of total degree $k$ where the degree of the $i^{th}$ variable in $z^S$ equals the number of times $i$ occurs in $S$. Let $\gamma:\cS_k(n) \rightarrow \N$ be the map that gives the coefficient of $z^S$  in the expansion of $(\sum_{i = 1}^n z_i)^k.$ Then, observe that $\sum_{S \in \cS_k(n)} \gamma(S) = 1.$



\paragraph{Basic Facts about Pseudo-Distributions} 

The first fact shows that if an inequality in a scalar random variable holds for all distributions over $\R$, then it also holds for all pseudo-distributions over $\R$ of degree $1$ higher than the degree of the polynomial appearing in the inequality.
\begin{fact} [See Corollary 6.14 in \cite{reznick2000some}, see also \cite{lasserre2015introduction}]
  Suppose $\tmu$ is a pseudo-distribution on $\R$ of degree $d$.
  Then, there's an actual distribution $\tmu'$ over $\R$ such that $\E_{\mu'}p = \pE_{\mu}p$ for every polynomial $p$ of degree at most $d-1$. \label{fact:univariate}
\end{fact}

% Next, the following fact shows a simple proof that allows moving between facts on the unit sphere and the unit simplex. We provide a simple proof because we are unaware of a reference.

% \begin{lemma}[From Sphere to the Simplex]
% Let $p$ be a polynomial over the unit simplex $\Delta_n$ in $n$ dimensions. For any $z \in \bbS^{n-1}$, let $z^{\ocircle 2} \in \R^n$ be the vector with $i^{th}$ coordinate given by $z_i^2$ for each $i$. Suppose for every pseudo-distribution $\tnu$ of degree at least $d$ over $\bbS^{n-1}$ it holds that $\pE_{\tnu}[p(z^{\ocircle 2}) \geq 0]$. Then, for every pseudo-distribution $\tmu$ over the unit simplex $\Delta_n$, it holds that $\pE_{\tmu}[p(x)] \geq 0.$  
% \end{lemma}

% \begin{proof}
% Suppose otherwise and let $\tmu$ be a pseudo-distribution over the unit simplex such that $\pE_{\tmu}p(x) < 0.$ Let $\tnu$ be the pseudo-distribution defined by  

% \end{proof}


\begin{fact}[Holder's Inequality for Pseudo-distributions] \label{fact:Holders}
Let $\tmu$ be a pseudo-distribution over $x \in \R^n$ and let $f,g$ be degree $d$ polynomials in $x$  Let $p,q$ be even integers such that $1/p + 1/q = 1.$ Then, if $\tmu$ has degree at least $2dpq$, then $\pE_{\tmu}[fg]^{pq} \leq \pE_{\tmu}[f^{p}]^q\pE_{\tmu}[g^q]^p.$
\end{fact}

\begin{fact}[Cauchy-Schwarz for Pseudo-distributions] \label{fact:Cauchy-Schwarz}
Let $\tmu$ be a pseudo-distribution over $x \in \R^n.$ Let $f,g$ be degree $d$ polynomials in $x$. Then, $\pE_{\tmu} [fg]^2 \leq \pE_{\tmu}[f^2] \pE_{\tmu}[g^2$ for any pseudo-distribution $\tmu$ of degree at least $4d.$
\end{fact}


\paragraph{Reweightings} A basic idea in rounding sum-of-squares relaxations is that of \emph{reweighting}. Given a finitely supported pseudo-distribution $\tmu$ over $\R^n$, we identify the the mass function of the pseudo-distribution with the function $\tmu$ itself. Given a polynomial $p$ in $x$ scaled so that $\pE_{\tmu}[p] = 1$, we can define the reweighting of $\tmu$ by $p$ as the pseudo-distribution $\tmu'$ with the mass function $\tmu'= \tmu \cdot p.$ 

It is easy to check that if $p$ is a sum-of-squares polynomial of degree $k$ and $\tmu$ is a pseudo-distribution of degree $d$ then $\tmu'$ is a pseudo-distribution of degree at least $d-k.$ Further, if we take two successive reweightings $\tmu \rightarrow \tmu' \rightarrow \tmu''$ of degree $k_1, k_2$ respectively, then, $\tmu''/\tmu$ is a polynomial of degree $k_1 + k_2$ and in particular, $\tmu''$ is a degree $k_1 + k_2$ reweighting of $\tmu''.$

If $\tmu$ is a pseudo-distribution that satisfies a system of polynomial constraints, then any SoS-reweighting of $\tmu$ also satisfies the same constraints so long as the degree of the reweighted pseudo-distribution exceeds the degree of every one of the constraints in the system. 

We will use the following reweighting developed in \cite{BarakKS2017} as a blackbox. 
\begin{fact}[Scalar Fixing Reweighting: Fixing a scalar around its standard deviation (See Lemma in \cite{BarakKS2017}] \label{lem:fixing-scalar}
Let $\mu$ be a distribution over $\R$ satisfying $\{x \leq 1\}$ and $\pE_{\mu}x^2 \geq \delta.$  Then, for some absolute constant $C > 0$, there exists a reweighting ("scalar fixing reweighting") $\mu'$ of $\mu$ of degree $k = Cd\log{(1/\delta)}/\epsilon^2$ satisfying $\pE_{\mu'} (x-m)^d \leq \epsilon^d m^d$ for some $m$ satisfying $|m| \geq \delta.$ Moreover, the sum of the absolute values of the coefficients of the polynomial $\tmu'/\tmu$ is at most $1/\delta^{2k}$ and the conclusions hold even for pseudo-distributions $\mu$ of degree at least $d+k.$
\end{fact}


\paragraph{Sum-of-Squares Proofs an{}d Pseudo-distributions}

\begin{definition}[Degree $d$ Derivations]
Let $\Sigma = \{ \{p_1 \geq 0 \}, \{p_2 \geq 0\}, \ldots, \{ p_r \geq 0\} \}$ be a system of polynomial constraints. For a polynomial $p$, we say that $p$ has a sum-of-squares proof of degree $d$ assuming the axioms in $\Sigma$ and write $\Sigma \vdash_d \{ p \geq 0\}$ if $p = q + \sum_{i \leq r} q_i \cdot p_i$ where $q, q_1, q_2, \ldots, q_r$ are sum-of-squares polynomials and the degree of each of $q_i \cdot p_i$ and $q$ is at most $d$. More generally, we write $\Sigma \vdash_d \{ p \geq q\}$ for polynomials $p,q$ if $\Sigma \vdash_d \{p-q \geq 0 \}.$ When a polynomial $p$ has a degree $d$ sum-of-squares proof of positivity over $\R$ (i.e. over empty $\Sigma$), we simply write $\vdash_d \{ p \geq 0\}.$
\end{definition}

An easy consequence of having a degree $d$ sum-of-squares proof is the following:
\begin{fact}[Pseudo-expectations respect sum-of-squares proofs]
Let $\Sigma$ be the system of polynomial constraints as above and suppose $\Sigma \vdash_d \{p \geq 0\}.$ Then, for any pseudo-distribution $\tmu$ of degree at least $d$ that satisfies the constraints in $\Sigma$, $\pE_{\tmu} p \geq 0.$
\end{fact}

% \subsection{Intuition for our Rounding} \Pnote{TODO:shorten this}
% As stated before, our rounding is perhaps the most natural SoSization of the sampling procedure of LMM. The observation of LMM can be stated as follows: Let $(\xx,\yy)$ be an equilibrium for the two player game under consideration. Sample $k = \Theta(\log{(n)}/\epsilon^2)$ pure strategies according to $\xx$ and $\yy$ to obtain multi-sets $S$ and $T$ of size $k$. Return uniform distribution on multi-sets $S$ and $T$, $\U_S, \U_T$ as the strategies for Alice and Bob. Then, with $1-o(1)$ probability, $(\U_S,\U_T)$ is an $\epsilon$-approximate $\NE$ for the game. 

% The probability of sampling a multi-set $S$ is easily seen as $\gamma(S) \xx^S$ where $\xx^S$ is the monomial in $\xx$ indexed by the multi-set $S$ and $\gamma(S)$ is some constant that depends on frequencies of the occurring elements in $S$. Thus, the probability of sampling $(S,T)$ is equals $\gamma(S) \gamma(T) \cdot \xx^S \yy^T$ - a monomial in $\xx$ and $\yy$ of degree $k$. 

% In order to gain intuition about how to round a pseudo-distribution over equilibria, let us start by a special illustrative case that appears interesting by itself. Suppose instead of a single equilibrium, we are given low-degree moments of a distribution $\mu$ that is supported over strategy profiles that form an equilibrium. We want to implement the sampling procedure above by accessing only low-degree moments of the distribution $\mu$. A natural choice then is to choose a multi-set $S$ with probability $\gamma(S) \gamma(T) \E_{\mu} \xx^S \yy^T$ - the average of the probabilities of sampling $S$ for each equilibrium in the support of $\mu$. This almost works with one possibly technical issue.  
%  %Note that equilibria are distributions over strategies and $\mu$ is a distribution over equilibria that we have low-degree-moment access to.


% Each equilibrium in the support of $\mu$ may yield different set of payoffs for Alice and Bob. This can be a problem - imagine that somehow, densely supported equilibria in the support of $\mu$ give large payoffs while sparsely supported equilibria give low payoffs. Then, in the sampling probability for a multi-set $S$ described above, the dominating contribution comes from sparse equilibria (since sparse equilibria will typically have large values for the monomial $\xx^S$ and $\yy^T$) and thus, we will end up getting a small payoff for the sampled strategy even though the average payoff for strategies in support of $\mu$ happened to be large. 

% A moment's reflection suggests a ``cure'' for this particular case - we should really be giving the strategies that have high payoff large weight even though $\mu$ doesn't. More generally, we would like to start with a distribution $\mu$ such almost all the probability mass in $\mu$ is on equilibria that give similar payoffs. A simple solution is to just condition $\mu$ on equilibria that give payoffs that are larger than the average payoff of the distribution $\mu$. Then our algorithm for rounding low-degree moments of $\mu$ can be described in two steps: 1) condition and obtain $\mu'$ so that the payoffs of strategy profiles in the support of $\mu$ concentrate around some quantity that is at least as large as the average payoff of $\mu$ for both Alice and Bob 2) sample $(S,T)$ with probability $\E_{\mu'} \xx^{S} \yy^{T} \gamma(S) \gamma(T).$ This is indeed our rounding for distributions.

% Further, the idea naturally generalizes to pseudo-distributions over equilibria (instead of actual distributions). We first implement an appropriate version of the conditioning step and obtain a pseudo-distribution $\tmu'$ such that the payoffs for Alice and Bob show satisfy a concentration property (which is a moment-based characterization of concentration) and then sample a multi-set pair $(S,T)$ with probability $\pE_{\tmu} \xx^{S} \yy^{T} \gamma(S) \gamma(T)$! 
% It is not hard to check that the constraints on $\tmu$ being supported on strategy profiles (i.e. elements of $\Delta_n \times \Delta_n$) makes this a valid procedure (in the sense that all probabilities are non-negative and add up to $1$ when summed up over all $k$-size multi-sets.)

% The analysis is based on generalizing the argument of LMM to work for pseudo-distributions over equilibria. \Pnote{ say more about analysis?}

\subsection{The Algorithm} 
We begin by describing the algorithm and giving an overview of its analysis here. 

\newcommand{\algnametwo}{6.2\xspace}

\begin{center}
\fbox{\begin{minipage}{6in} 
\begin{center}
\textbf{Algorithm \algnametwo} 
\end{center}

\begin{description}
\item[Input:] $d \in \N$, a pseudo-distribution $\tmu$ of degree $d$ over Nash equilibria of $n$-strategy games $(A,B)$, with payoffs $\pE_{\tmu}\xx^{\top}A\yy = \delta_1$ and $\pE_{\tmu} \xx^{\top} B\yy = \delta_2$ and parameter $\epsilon>0$. Set $\delta = \min\{\delta_1, \delta_2\}.$
\item[Output:] A $k$-support strategy profile $(\U_S,\U_T)$ for multi-sets $S,T$ of $[n]$ of size $k = \log{(n)}/\epsilon^2.$
\item[Operation:] ~
\begin{enumerate}
\item Use Lemma \ref{lem:fixing-payoffs} to obtain a reweighting $\tmu'$ of $\tmu$ of degree $C\ell \log{(1/\delta)}^2/\epsilon^2$ such that the concentration property \eqref{eq:conc-property} holds with parameters $m_A \geq \delta_1, m_B \geq \delta_2$.
\item Sample $(S, T)$, multi-sets of size $k$ with probability $\gamma(S)\cdot \gamma(T) \pE_{\tmu} \xx^S \yy^{T}$. 
\item Return $(\U_S, \U_T)$

\end{enumerate}
\end{description}
\end{minipage}}
\end{center}

\paragraph{Analysis}

We start by giving three lemmas that capture the high-level strategy of our analysis. Readers should note the similarity of the second and third high-level steps to the analysis of the LMM algorithm. 

Let $\pi_A = \xx^{\top} A \yy, \pi_B = \xx^{\top} B y$ be the respective payoffs of Alice and Bob. In the first step of the algorithm, we ``condition'' the pseudo-distribution so that the payoff is concentrated in an additive interval of $\epsilon.$ Formally, we obtain the following guarantee:

\begin{lemma}[Fixing Payoffs] \label{lem:fixing-payoffs}
Let $\tmu$ be a pseudo-distribution of degree $d$ on $\Delta_m \times \Delta_m.$ Let $\ell$ be an integer parameter. Let $\pi_A = \xx^{\top} A \yy$, $\pi_B = \xx^{\top} B \yy$ be the degree two polynomials describing the payoffs of Alice and Bob at a strategy profile $(\xx,\yy)$. Suppose $\pE_{\tmu}\pi_A = \delta_1, \pE_{\tmu} \pi_B = \delta_2$ and $\delta = \min \{ \delta_1, \delta_2\}.$

Then, there exists a polynomial $p(\xx,\yy)$ of degree $C \ell \log{(1/\delta)}^2/\epsilon^2$ for some large enough constant $C > 0$ satisfying $\pE_{\tmu}p^2 =1$ such that the reweighting $\tmu' = \tmu \cdot p^2$ satisfies: 
\begin{align}
\pE_{\tmu'} (\pi_A - m_A)^{2\ell} &\leq \epsilon^{2\ell}m^{2\ell} \notag\\
\pE_{\tmu'} (\pi_B - m_B)^{2\ell} &\leq \epsilon^{2\ell}m^{2\ell} \label{eq:conc-property}
\end{align}
for some $m_A \in [\delta_1,1]$ and $m_B \in [\delta_2, 1].$ 

\end{lemma}

Next, we argue that the payoffs of rounded strategy are close to that the payoffs of the pseudo-distribution with high probability. 

\begin{lemma}[Payoff of Rounded Strategy] \label{lem:large-payoff-of-rounding}
Let $\tmu$ be a pseudo-distribution of degree $d$ such that the payoffs satisfy the concentration property \eqref{eq:conc-property} with parameters $m_A, m_B \in [0,1].$ Fix $k = 2\log{(n)}/\epsilon^2$ and sample a pair of multisets $(S,T)$ of size $k$ with probability $\pE_{\tmu}[x^Sy^T].$ Then, with probability at least $1-1/n^2$, the payoff $\U_S^{\top}A \U_T \geq m_A - \epsilon$ and $\U_S^{\top} B \U_T \geq m_B - \epsilon.$
\end{lemma}

Finally, we show that the there's at most $\epsilon$ incentive to deviate from the rounded strategy with high probability.
\begin{lemma}[Small Incentive to Deviate from Rounded Strategy] \label{lem:incentive-to-deviate-from-rounded-strategy}
Let $\tmu$ be a pseudo-distribution of degree $d$ such that the payoffs satisfy the concentration property \eqref{eq:conc-property} with parameters $m_A, m_B \in [0,1].$ Fix $k = 2\log{(n)}/\epsilon^2$ and sample a pair of multisets $(S,T)$ of size $k$ with probability $\gamma(S) \gamma(T) \pE_{\tmu}[x^Sy^T].$ Then,with probability at least $1-1/n$, for every $i$, $e_i^{\top}A\U_T \leq m_A + \epsilon$ and $\U_S^{\top} B e_i \leq m_B + \epsilon.$
\end{lemma}

\begin{proof}[Proof of Theorem \ref{thm:upper-bound-technical}]
Our algorithm is the following: run the sum-of-squares relaxation of degree $O(\log{(n)}/\epsilon^2)$-degree and get a pseudo-distribution $\tmu$ supported over equilibria of the game. Apply the oblivious rounding above. 

We now analyze this rounding:
Combining Lemmas \ref{lem:large-payoff-of-rounding} and \ref{lem:incentive-to-deviate-from-rounded-strategy} yields that if we start with a pseudo-distribution on $\NE$ of the underlying game $(A,B)$ that satisfies the concentration property \eqref{eq:conc-property}, then with probability at least $1-1/n$, the rounded strategy satisfies all requirements of being an $\epsilon$ $\NE$ with payoff for each of the players within an additive $\epsilon$ of the payoff of the pseudo-distribution. Lemma \ref{lem:fixing-payoffs} ensures that we can make any pseudo-distribution over equilibria of the game $(A,B)$ satisfy the concentration property \eqref{eq:conc-property}. This completes the proof of correctness of the rounding algorithm.
\end{proof}

\subsection{Analysis: Key Technical Lemmas}
We now give the details of the analysis.
\begin{lemma}[Payoff of Rounded Strategy is Concentrated]
Let $\tmu$ be a pseudo-distribution of degree $d$ such that the payoffs satisfy the concentration property \eqref{eq:conc-property} with parameters $m_A, m_B \in [0,1].$ Then, for any $k$ and $q$, for any $q \in \N$,
\begin{equation} \label{eq:payoff-rounded-concentration-A}
\pE_{\tmu}  \sum_{S,T: |S|, |T| = k} \gamma(S) \gamma(T)x^S y^T (\U_S^{\top} A \U_T - m_A)^{2q} \leq \epsilon^{2q}
\end{equation}
 and
\begin{equation} \label{eq:payoff-rounded-concentration-B}
 \pE_{\tmu}  \sum_{S,T: |S|, |T|= k}\gamma(S) \gamma(T) x^S y^T (\U_S^{\top} B \U_T -m_B)^{2q} \leq \epsilon^{2q}
 \end{equation}
 whenever $d \geq q+ .$

\label{lem:payoff-of-rounded-strategy-concentrates}
\end{lemma}
\begin{remark}
Observe that the LHS of the first inequality is the centralized moment of the difference between the payoff of the rounded strategy and $m_A$ - the constant around which the payoff of Alice under the pseudo-distribution is fixed. The second inequality is a similar fact about the payoff of Bob.
\end{remark}

Finally, we show a fact about pseudo-expectation that allows us to obtain that the probability that there's an $i$ such that deviating to pure strategy $i$ increases the payoff of Alice (or Bob) by more than $\epsilon$ compared to the rounded strategy is small.






% \begin{proof}

% Fix any $x,y \in \Delta_n.$ 

% We will show the first statement. The second has the same proof with $A$ replaced by $B$. 
% Fix $(\xx,\yy) \in \Delta_n \times \Delta_n.$ Let $p(\xx,\yy)$ be the polynomial $\sum_{S,T \in \cS_k(n)} \gamma(S) \gamma(T) x^S y^T (\U_S^{\top} A \U_T - \xx^{\top} A \yy)^{2q}.$ It's easy to check that this is the expectation of $(\U_S^{\top} A \U_T - \xx^{\top} A \yy)^{2q}$ when the pair $(S,T)$ of multi-sets are sampled by taking $k$ independent singletons distributed according to $\xx$ and $\yy$ respectively. Thus, let $u_1, u_2 \ldots, u_k$ be distributed independently as $\xx$ and $v_1, v_2, \ldots, v_k$, independent pure strategies distributed as $\yy.$ Then, $p(x,y) = \E_{u_1, u_2, \ldots, u_k \sim \xx, v_1, v_2, \ldots, v_k \sim \yy} \left(\frac{1}{k^2}\sum_{i,j \leq k}  (u_i^{\top} A v_j-\xx^{\top}A\yy) \right)^{2q}.$

% We can now expand the expression for $p(\xx,\yy)$ above as $\E_{u_1, u_2, \ldots, u_k \sim \xx, v_1, v_2, \ldots, v_k \sim \yy} \frac{1}{k^{4q}} \sum_{a_1, a_2, \ldots, a_{2q}, b_1, b_2, \ldots, b_{2q}} \Pi_{i = 1}^{2q} A(a_i,b_i) \sum_{}$
% \end{proof}

The technical ingredient in the proof of Lemma \ref{lem:payoff-of-rounded-strategy-concentrates} is the sum-of-squares proof of the concentration inequality that appears in the sampling argument of Lipton-Markakis-Mehta.
\begin{lemma}[SoSizing Concentration] \label{lem:SoSizing-basic-concentration}
% Let $\tmu$ be a pseudo-distribution over $\Delta_n \times \Delta_n \times [-1,1]^n$ of degree $d$ and $(\xx,\yy,v)$, the associated (pseudo)-random variable. Then, for $k = \Omega(\log{(n)}/\epsilon^2)$, $\ell \in \N$ and $d \geq k+2\ell$,   
% \[ \pE_{\tmu(\xx,\yy,v)} \sum_{S \in \cS_k(n)} \gamma(S) \xx^{S} (\langle v, \U_S \rangle - \langle v, \xx \rangle)^{2\ell} \leq \epsilon^{2\ell}.
% \]
Let $\Sigma = \{\xx \in \Delta_n, -1 \leq w_i \leq 1 \text{ for } 1 \leq i \leq n \}$ be the system of constraints describing the space where $\xx$ is a distribution over $n$ pure strategies and $w$ is a vector in $[-1,1]^n$. Then, for any $\ell \in \N$, $k = \Omega(\ell/\epsilon^2)$ and $d = O(k)$, 
\[
\Sigma \vdash_{d} \left\{ \sum_{S \in \cS_k(n)} \gamma(S) \xx^{S} (\langle w, \U_S \rangle - \langle w, \xx \rangle)^{2\ell} \leq \epsilon^{2\ell} \right\} 
\]

\end{lemma}

\begin{proof}
Observe that for any fixed $\xx,v$, the polynomial expression $p(\xx,w)$ in the statement is the expectation of the $\langle w, \U_S \rangle - \langle v, \xx \rangle)^{2\ell} \leq \epsilon^{2\ell}$ when the strategy $\U_S$ for $S \in \cS_k(n)$ is sampled with probability $\gamma(S) \cdot \xx^{S}$. This is equivalent to sampling $k$ independent pure strategies $u_i \in \Delta_n \cap \zo^n$ where $u_i$ is distributed according to $\xx$ and then taking the strategy $u = \frac{1}{k} \sum_{i \leq k} u_i$. Thus, we can write
\[
p(\xx,w) = \E_{u_i \sim \xx \text{ for each i}} \frac{1}{k^{2\ell}} \left( \sum_{i \leq k} (\langle w, u_i \rangle - \langle w, \xx \rangle) \right)^{2\ell}.
\]
Let $z_i = \langle w, u_i - \xx \rangle$ for each $1 \leq i \leq k.$
We can expand the expression and use linearity of expectation to write:
\begin{equation} \label{eq:expanded-expectation}
p(\xx,w) = \frac{1}{k^{2\ell}} \sum_{i_1, i_2, \ldots, i_{2\ell}} \E_{u_i \sim \xx} \Pi_{j \leq 2\ell} z_{i_j}.
\end{equation}
Observe that $z_i$s are independent random variables with mean zero. Thus, the expectation of any monomial defined by $i_1, i_2, \ldots, i_{2\ell}$ above where there's some index out of $[k]$ that occurs exactly once is zero. In particular, $i_1, i_2, \ldots, i_{2\ell}$ must form a set of size at most $\ell.$  The number of such sets is at most $k^{\ell} \cdot \ell!$

Now, via elementary and standard arguments, $\{-1 \leq w \leq 1\} \vdash_4 (\langle w, u_i \rangle)^2 \leq 1$ and $\{-1 \leq w \leq 1\}, \{ \xx \in \Delta_n\} \vdash_4 (\langle w, \xx \rangle)^2 \leq 1.$ These readily imply via $O(\ell)$-degree sum-of-squares proofs, the polynomial inequalities $\{ \Pi_{i \in S} \langle w, u_i - \xx \rangle \leq 2^{2\ell}$ for any $S$, a multi-set of size $2\ell.$ 

Now, as argued above, there are at most $k^{\ell} \cdot \ell!$ non-zero terms in the expression \eqref{eq:expanded-expectation} for $p(\xx,w)$ and further, there are $O(\ell)$-degree arguments that establish that each of those terms is at most $2^{2\ell}.$ Thus, $\Sigma \vdash_d \{ p(\xx,w) \leq \frac{1}{k^{2\ell}} k^{\ell} \ell! 2^{2\ell} = k^{-\ell} \ell^{O(\ell)}.$

For any $k = \Omega( \ell/\epsilon^2)$, the upper bound above is at most $\epsilon^{2\ell}$ as required. 
\end{proof}

We can use Lemma \ref{lem:SoSizing-basic-concentration} to give sum of squares proofs that the payoffs and the incentives to deviate to any strategy for either player of the sampled strategy are concentrated around those of the unsampled strategy within $\epsilon.$

\begin{corollary}[Corollary of Lemma \ref{lem:SoSizing-basic-concentration}]
Let $\Sigma = \{\xx, \yy \in \Delta_n\}$ be the system of constraints describing the space of strategy profiles $\xx,\yy$ over $n$ pure strategies. Then, for any $\ell \in \N$, $k = \Omega(\ell/\epsilon^2)$ and $d = O(k)$, 
\begin{enumerate}
	\item  $\Sigma \vdash_d \left\{ \sum_{T \in \cS_k(n)} \gamma(T) \yy^{T} (e_i^{\top} A \U_T - e_i^{\top} A \yy)^{2\ell} \leq \epsilon^{2\ell} \right\}$ for every $1 \leq i \leq n$,
	\item $\Sigma \vdash_d \left\{ \sum_{S \in \cS_k(n)} \gamma(S) \xx^{S} (\U_S^{\top} B e_i - \xx^{\top} B e_i)^{2\ell} \leq \epsilon^{2\ell} \right\}$ for every $1 \leq i \leq n$,
	\item $\Sigma \vdash_d \left\{ \sum_{S,T \in \cS_k(n)} \gamma(S) \gamma(T) \xx^{S} \yy^{T} (\U_S^{\top} A \U_T - \xx^{\top} A \yy)^{2\ell} \leq 2(2\epsilon)^{2\ell} \right\}$
	\item $\Sigma \vdash_d \left\{ \sum_{S,T \in \cS_k(n)} \gamma(S) \gamma(T) \xx^{S} \yy^{T} (\U_S^{\top} B \U_T - \xx^{\top} B \yy)^{2\ell} \leq 2(2\epsilon)^{2\ell} \right\}$
\end{enumerate}
% \Sigma \vdash_{d} \left\{ \sum_{S \in \cS_k(n)} \gamma(S) \xx^{S} (\langle w, \U_S \rangle - \langle w, \xx \rangle)^{2\ell} \leq \epsilon^{2\ell} \right\} 
% \]
\label{cor:concentration-of-payoffs-and-incentives}
\end{corollary}

\begin{proof}

For (1), consider the vector $e_i^{\top} A$. Observe that $A$ has all of its entries bounded above by $1$ in magnitude and thus, so does the vector $w = e_i^{\top}A.$ To get the claim, apply Lemma \ref{lem:SoSizing-basic-concentration} with $w = e_i^{\top}A$. The case of $(2)$ is entirely analgous. 

For (3), we write $\sum_{S,T \in \cS_k(n)} \gamma(S) \gamma(T) \xx^{S} \yy^{T} (\U_S^{\top} A \U_T - \U_S^{\top} A \yy + \U_S^{\top} A \yy- \xx^{\top} A \yy)^{2\ell} .$

Via Cauchy-Schwarz inequality, this can be upper bounded by
\begin{multline}
2^{2\ell} \sum_{S,T \in \cS_k(n)} \gamma(S) \gamma(T) \xx^{S} \yy^{T} (\U_S^{\top} A \U_T - \U_S^{\top} A \yy)^{2\ell} \\+
2^{2\ell} \sum_{S,T \in \cS_k(n)} \gamma(S) \gamma(T) \xx^{S} \yy^{T} (\U_S^{\top} A \yy- \xx^{\top} A \yy)^{2\ell} .
\end{multline}

To upper bound the first term, we now do the following steps. First fix $S$ and then write $\U_S = \frac{1}{k} \sum_{i \in S} e_i. $ By an application of Cauchy-Schwarz inequality and using (1), we obtain an upper bound on the term (for a fixed $S$) as $2^{2\ell} \cdot \gamma(S) \xx^{S} \epsilon^{2\ell}.$ Summing over all $S$ this gives us an upper bound of $(2\epsilon)^{2\ell}$ using the fact that $\sum_{S \in \cS_{k}(n)} \gamma(S) \xx^S = 1.$ Analogously, we obtain the same upper bound for the second term above. Together, they yield (3). The proof for (4) is entirely analogous to case $(3).$

\end{proof}


Next, we analyze the probability that the incentive to deviate from the rounded strategy exceeds $\epsilon$. The key result is the following:

\begin{lemma}[Bounding Incentives to Deviate]
Let $\tmu$ be a pseudo-distribution on $\NE$ of $(A,B)$ that satisfies the concentration property of payoffs \eqref{eq:conc-property}. Then, for $k = \log{(n)}/\epsilon^2$,
\begin{equation},
\sum_{T \in \cS_k(n)} \pE_{\tmu} \gamma(T) y^T (e_i^{\top}A \U_T)^{2q} \leq (m_A +\epsilon)^{2q}, \label{eq:bounding-incentive-to-deviate-A}
\end{equation}
and
\begin{equation}
\sum_{S \in \cS_k(n)} \pE_{\tmu} \gamma(S) x^S (\U_S^{\top} A e_i)^{2q} \leq (m_B +\epsilon)^{2q}.\label{eq:bounding-incentive-to-deviate-B}
\end{equation} \label{lem:incentive-to-deviate}
\end{lemma} 

The following lemma is notes a strong consequence of payoffs and incentives being concentrated in the rounded strategy. 


\begin{lemma}
Let $\tmu$ be a pseudo-distribution on $\NE$ of $(A,B)$ that satisfies the concentration property of payoffs \eqref{eq:conc-property}. Then, for $k = \log{(n)}/\epsilon^2$, and for any $q \leq \ell/2$, 
\begin{equation},
\pE_{\tmu} (\xx^{\top}A \yy)^{2q} \leq (m_A +\epsilon)^{2q}, \label{eq:conc-payoff-A}
\end{equation}

\begin{equation},
\pE_{\tmu} (\xx^{\top}A \yy)^{2q} \leq (m_A +\epsilon)^{2q}, \label{eq:conc-payoff-B}
\end{equation}


and for every $i$, 

\begin{equation}
\sum_{T \in \cS_k(n)} \pE_{\tmu} \gamma(T) \yy^T (e_i^{\top}A \U_T)^{2q} \leq \pE (e_i^{\top} A \yy  +\epsilon)^{2q}, 
\end{equation}


\begin{equation}
\sum_{S \in \cS_k(n)} \pE_{\tmu} \gamma(S) \xx^S (\U_S^{\top}B e_i)^{2q} \leq \pE (\xx^{\top} A e_i  +\epsilon)^{2q}.
\end{equation}


\label{lem:conc-payoff}
\end{lemma}



\begin{proof}
We do the proof for the first case. The other claims are proven similarly by relying on Corollary \ref{cor:concentration-of-payoffs-and-incentives}. 
\begin{align}
\pE_{\tmu} (\xx^{\top}A \yy)^{2q} &= \pE_{\tmu} (\xx^{\top} A \yy -m_A + m_A)^{2q}\\
&= \sum_{i \leq 2q} {{2q} \choose i}  \pE[ (\xx^{\top} A \yy -m_A)^{i}] \cdot m_A^{2q-i}\\
&\leq_{\text{ Cauchy-Schwarz}}  \sum_{i \leq 2q} {{2q} \choose i} \pE[ (\xx^{\top} A \yy -m_A)^{2i}]^{1/2} \cdot m_A^{2q-i}\\
&\leq_{\eqref{eq:conc-property}} \sum_{i \leq 2q} {{2q} \choose i} \epsilon^{i} \cdot m_A^{2q-i}\\
&= (m_A + \epsilon)^{2q}.
\end{align}

\end{proof}

We can now conclude that for any $i$, with probability at least $1-1/n^2$ over the sampling of the strategy $(\U_S,\U_T)$, $e_i^{\top}A\U_T \leq m_A + \epsilon$ and $\U_S^{\top} B e_i \leq m_B + \epsilon.$

\begin{proof}[Proof of Lemma \ref{lem:incentive-to-deviate}]
We do the proof of the first claim - as usual the second has an entirely analogous proof. 

We have,
\begin{align*}
\sum_{T \in \cS_k(n)} \pE_{\tmu} \gamma(T) y^T (e_i^{\top}A \U_T)^{2q} &\leq_{\text{Lemma \ref{lem:conc-payoff}}} \pE (e_i^{\top} A \yy  +\epsilon)^{2q}\\
&\leq_{\text{ constraint in pseudo-equilibria}} \pE (\xx^{\top} A \yy + \epsilon)^{2q}\\
&\leq_{\text{ Lemma \ref{lem:conc-payoff}}} (m_A + 2\epsilon)^{2q}.
\end{align*}





\end{proof}






\subsection{Analysis: Proofs of the Three Key Claims}

% The above lemma immediately implies that the rounding outputs a strategy, that with probability at least $1-1/n^2$ has a payoff within $\epsilon$ of the payoff of the pseudo-distribution.



\begin{proof}[Proof of Lemma \ref{lem:fixing-payoffs}]
Let $k = C \ell \log{(1/\delta)}/\epsilon^2$ and $d = k \log{(1/\delta)}$ such that $\ell$ divides $d$.
Observe that $\Pi_A$ satisfies $\{\pi_A \leq 1\}$ and $\pE_{\tmu} \pi_A \geq \epsilon.$
 Apply the scalar fixing reweighting to the random variable $\pi_A$  with a degree $k' = Cd \log{(1/\epsilon)}/\epsilon^2$ degree polynomial to obtain a pseudo-distribution $\tmu'$ such that \begin{equation} \label{eq:first-payoff-fixing} \pE_{\tmu'}[ (\pi_A - m_A)^{2d}] \leq \epsilon^{2d} m_A^{2d} .\end{equation}

Now, apply the scalar fixing reweighting of degree $k$ to the random variable $\pi_B$ (under $\tmu'$) to obtain a pseudo-distribution $\tmu''$ that satisfies 
\begin{equation} \label{eq:second-payoff-fixing} \pE_{\tmu'}[ (\pi_A - m_A)^{2\ell'}] \leq \epsilon^{2\ell} m_A^{2\ell}. \end{equation}
We claim that $\tmu''$ satisfies the requirements of the lemma. It is clear that $\tmu''$ is a reweighting of $\tmu$ of degree at most $3C \ell \log{(1/\delta)}^2/\epsilon^2.$ Also, \eqref{eq:second-payoff-fixing} yields the required fixing condition for $\pi_B.$ The only remaining condition to verify is the fixing condition for $\pi_A.$ Observe that \eqref{eq:first-payoff-fixing} gives us almost the condition but holds for the pseudo-distribution $\tmu'$ and not $\tmu''$ and reweighting $\tmu'$ could have somehow killed the fixing condition from holding for $\pi_A.$ We show that this cannot happen since we fixed $\pi_A$ to a larger degree than intended ($\ell' = 2\ell$) and $\tmu''$ is a smaller degree reweighting of $\tmu.$

Let $p = \tmu''/\tmu'.$ We have:
\begin{align}
\pE_{\tmu''}[ (\pi_A-m_A)^{2\ell}]^{\frac{4d}{2\ell}} &\leq \pE_{\tmu''} [(\pi_A-m_A)^{2d}]^2\\ 
&= \pE_{\tmu'} [(\pi_A-m_A)^{2d} p(x,y)]^2\\
&\leq \pE_{\tmu'}p^2 \E_{\tmu'} [(\pi_A-m_A)^{2d}]. 
\end{align}
The first inequality follows from Holder's inequality for pseudo-distributions and the second inequality above follows from the Cauchy-Schwarz inequality for pseudo-distributions.

 Next, we observe that $\pE_{\tmu'}p^2 \leq 1/\epsilon^{4k}$ since $\pi_B \leq 1$ and $p$ has all the sum of the absolute values of all its coefficients upper bounded by $1/\delta^{2k}$ and thus, $\{\pi_B \leq 1\}$ implies that $p \leq 1/\delta^{2k}.$
Thus, $\pE_{\tmu''}[ (\pi_A-m_A)^{2\ell}]^{2 \frac{4d}{2\ell}} \leq 1/\delta^{2k} \cdot \epsilon^{2d} = (\frac{\epsilon}{\delta^{k/d}})^{2d}.$ Since $d > k\log{(1/\delta)}$, $(1/\delta)^{k/d} \leq (1/\delta)^{1/\log{1/\delta}} = 2.$ Thus,  $\pE_{\tmu''}[ (\pi_A-m_A)^{2\ell}]^{2 \frac{4d}{2\ell}} \leq 2\epsilon^{2d}$ or $\pE_{\tmu''}[ (\pi_A-m_A)^{2\ell}] \leq 2 \epsilon^{2\ell}.$ 
\end{proof} 

\begin{proof}[Proof of Lemma \ref{lem:large-payoff-of-rounding}]
Observe that \eqref{eq:payoff-rounded-concentration-A} and \eqref{eq:payoff-rounded-concentration-B} are $2q$-degree moments of the random variable $(\U_S^{\top} A \U_T - m_A)$ and $(\U_S^{\top} B \U_T -m_B)$ respectively (these are random variables arising from our ``randomized'' rounding, not ``pseudo-random variables'' associated with the pseudo-distribution.)

Then, choosing $q > 2\log{(n)}$, and applying Markov's inequality to the above random variables, we obtain that $\Pr_{(S,T) \sim \pE_{\tmu}[x^Sy^T]}[\U_S^{\top}A \U_T < m_A-2\epsilon ] \leq 2^{-q} = 1/n^2.$ A similar argument gives the analogous statement the payoff of Alice under the rounded strategy.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:incentive-to-deviate-from-rounded-strategy}]
Observe that \eqref{eq:bounding-incentive-to-deviate-A} and \eqref{eq:bounding-incentive-to-deviate-B} are $2q$-th moments of the random variable $(e_i^{\top}A \U_T)$ and $(\U_S^{\top} A e_i)$ respectively. Applying Markov's inequality to these random variables, we obtain: $\Pr_{T}[ (e_i^{\top}A \U_T) > m_A + 2\epsilon ] \leq (1+\epsilon)^{-2q}.$ Thus, choosing $q = 2\log{(n)}/\epsilon$ ensures that for each $i$, the above event has a probability of at most $1/n^2.$ Union bound over the $2n$ possible events one for each $i$ and for each of the two payoff matrices yields the Corollary.
\end{proof}



% \subsection{Commentary to be Added Elsewhere}
% The algorithm itself is simple to describe and generalizes the sampling algorithm of Lipton-Markakis-Mehta in a natural way to work with pseudo-distributions. Let us first recall what LMM showed. Their proof establishes the following:

% \begin{lemma}[Lipton-Markakis-Mehta]
% Let $(\xx,\yy)$ be a Nash equilibrium for a $n$-strategy game $(A,B).$ Sample a multi subset $S$ of size $k$ from $[n]$ by taking $k$ independent samples from the distribution $\xx$ over $[n].$ Similarly, sample a multi subset $T$ of size $k$ from $[n]$ by taking $k$ independent samples from $\yy$. Then, with probability $1-1/n$, $(\U_S, \U_T)$ is an $\epsilon$-$\NE$ whenever $k > \log{(n)}/\epsilon^2.$
% \end{lemma}

% LMM used this lemma to argue that there's a small-support approximate equilibrium for any two player game. But, the Lemma above establishes something more. Given a Nash equilibrium $(\xx,\yy)$, it can be thought of as an oblivious rounding algorithm that takes input an arbitrary equilibrium and with high probaibilty, outputs a small support approximate equilibrium. 

% Our key idea is to generalize this oblivious rounding view of the LMM algorithm to start from a pseudo-distribution (of sufficiently high degree) ove equilibria $(\xx,\yy)$ instead of a single equilibrium and produce a small support approximate equilibrium. However, an illustrative and key step is to get a version of the LMM sampling lemma that can produce an approximate equilibrium from any \emph{distribution} that is supported over strategy profiles that form $\NE$ for the underlying game. Of course, in this process, we do not want to access the game or even an oracle that can tell us if a strategy profile forms an approximate equilibrium for the underlying game. 

% So how do we ``sample'' an small-support approximate equilibrium given a distribution over actual equilibria? All we have to decide is what should be the probability of sampling any given multi-set of size $k$. In the LMM sampling, the probability of sampling a strategy profile $(\U_S, \U_T)$ for multi-sets $S$ and $T$ of size $k$ is precisely $\xx^S \cdot \yy^T$. In our sampling algorithm for pseudo-distribution, we will naturally choose this to be proportional to $\pE_{\tmu} \xx^S \yy^T.$

% Now, why should this be an approximate equilibrium with high probability? We can examine the proof of LMM for some more clues. The argument of LMM shows that if we sample $k$-size multi-sets from the distributions $\xx,\yy$ respectively, then with high probability, the payoffs for the two players are preserved within an additive bound of $\epsilon$ as are the ``incentives'' $e_i^{\top} A\yy$ and $\xx^{\top} B e_i$ for every $ 1\leq i \leq n.$ We could attempt to show that for the sampling strategy for distributions over equilibria above. But right off the start, we encounter an issue - the distribution could be supported on equilibria that give very different payoffs. In this case, we may not in general hope for the payoffs of the sampled strategy to concentrate around the average (with respect to $\mu$) of the payoffs of the distribution over the equilibria. 

% To fix this, we modify the distribution $\mu$ before applying the sampling above. Specifically, we \emph{condition} the distribution $\mu$ so that the payoffs are all constrained within some additive interval of length $\epsilon.$ As we will see later, we can implement this operation of conditioning on pseudo-distributions of degree at least $\log{(n)}/\epsilon^2.$ We then apply the sampling as described above and obtain an small-support strategy profile. 














% Let $\pE_{\tmu}$ be a degree $d$ pseudo-expectation supported over equilibria of a two-player game with $n$ strategies. We first describe a randomized algorithm that uses $\pE_{\tmu}$ to return a strategy profile that is $\epsilon$-approximate equilibrium with high probability whenever $d = \Omega(\log{(n)}/\epsilon^2).$ As discussed before, this can be seen as a Sum-of-Squares version of the sampling strategy that Lipton-Markakis-Mehta

% Let $\bbS_k$ be the set of all multi-sets of $[n]$ of size $k$. 




